Inspo: Writing with Crowds Alongside AI

The use of artificial intelligence (AI) to support creative writing has bloomed in recent years. However, it is less well understood how AI compares to on-demand human support. We explored how writers interact with both AI and crowd worker writing assistants in creative writing. We replicated the interface of the prior crowd-writing system, Heteroglossia, and developed Inspo, a text editor allowing users to request suggestions from AI models and crowd workers. In a one-week deployment study involving eight creative writers, we examined how often participants selected crowd workers when fluent AI text generators were also available. Findings showed a consistent decline in crowd worker usage, with participants favoring AI due to its faster responses and more consistent quality. We conclude with suggestions for future systems, recommending designs that account for the unique strengths and weaknesses of human versus AI assistants, strategies to address automation bias, and sociocultural views of writing.

==> sections/0-abstract.tex <==
With the rise of large language models (LLMs), research has emerged to study how writers incorporate an LLM into their writing workflows.
However, writing is more complex than receiving aid from one single assistant. 
%In practice, writers use multiple writing assistants and work with multiple humans to help them work; academics use auto-completion, ChatGPT, and Grammarly while working with co-authors, collaborators, and editors.
In practice, writers use multiple writing assistants and work with multiple people to enhance their work.
%Academics, for example, employ tools like auto-completion, ChatGPT, and Grammarly while also working with co-authors, collaborators, and editors.
This paper introduces \system, a text editor designed for creative writers to request inspiration 
%directly within the editor 
from four sources:
{\em (i)} online crowd workers, 
{\em (ii)} a story plot generation model, 
{\em (iii)} GPT-3 for predicting follow-up story plots (\gptplot), and 
{\em (iv)} GPT-3 for continuing ongoing stories (\gptc).
A week-long user study with multiple creative writers showed that participants consistently decreased their use of crowds in favor of AIs throughout the study. 
By the end, the crowd option was the least used by all the participants.
%\kenneth{TODO HCOMP: Is this true???}
\gptc was the most used by the majority, while some preferred the \plot. 
\gptc also had the greatest impact on the participants' written content, measured by text similarities. 
%Our work highlights the critical need for high-quality human involvement in creative writing support, especially as LLMs now offer instant suggestions. 
We conclude the paper by introducing a sociocultural view of writing to better understand the opportunities and risks of using LLMs in writing support. 
%These insights collectively inform the development of future creative writing assistants.

%---------------------- dead kitten ---------------------------

\begin{comment}

\kenneth{----------------KENNETH WORKING HERE--------------------}


% We built \system, and it is the best thing in the world.

With the rise of LLMs, a variety of works emerged to study how an LLM can be incorporated into writers' workflows.
However, writing is more complex than just employing one tool. 
In practice, writers use multiple writing aids and also work with multiple humans to facilitate their writing.
For example, we academics use ChatGPT, auto-completion, Grammarly, while working with co-authors, collaborators, and editors at the same time.
How writers incorporate multiple streams of assistance, some powered by AI and some by humans, in their creative workflows remains a fascinating yet underexplored research problem.
This paper presents \system, a web-based text editor that allows creative writers to request inspirations right within the editor from four sources:
{\em (i)} online crowd workers,
{\em (ii)} a story plot generation model,
{\em (iii)} GPT-3 that predicts follow-up story plots (\gptplot), and 
{\em (iv)} GPT-3 that completes the ongoing story (\gptc).
The one-week-long user study with multiple creative writers showed that participants consistently decreased their use of crowds in favor of AIs throughout the study.
By the end, the crowd option was the least used by all the participants.
%Interviews with the participants further revealed their reasons for favoring AI, including crowds' slow response times and inconsistent quality. 
%As a result, we found that participants increasingly used AI instead of crowds throughout the study. 
%Over the course of our study, we found that participants increasingly favored AI over crowds.
%By the end, Crowd was the least popular option. 
Meanwhile, %preferences for the three AI options varied:
\gptc was the most used by the majority, though some preferred the story plot generator. 
\gptc also had the greatest impact on the participants' written content, measured by text similarity. 
%similarity of texts written immediately after viewing inspirations.
Interviews with the participants show that they favor AI over the crowd because
%further revealed their reasons for favoring AI, including 
crowds' long response times and inconsistent quality. 
Our work highlights the increasingly critical requirements for the quality for human involvements to support creative writing in the era where LLM can already provide instant and decent suggestions.
We conclude the paper by introducing a socialcultrual view of writing that allow us to better understand the oppuertunies and risks of using LLMs in writing supports. 
%Our work can inform




%facilitate therie writing


\kenneth{TODO HCOMP: Need to mention more crowdsourcing}

Large Language Models (LLMs) have advanced automated writing assistance, enabling complex tasks like co-writing novels and poems.
However, real-world writing typically requires various support and collaboration across stages and scenarios.
Existing research mainly examines how writers utilize single text generators, neglecting this broader context. 
This paper introduces \system, a web-based editor that incorporates various text generators and online crowd workers.
Through a three-phase user study, we examine writers' interactions with \system for novel writing.
Quantitative analyses of writing logs highlight changes in participants' writing progress and the influence of various text-generation models.
Complementing this with qualitative insights from semi-structured interviews, we illustrate participants' perceptions of these models and the crowd.
Based on the findings, we provide design recommendations for the next generation of intelligent writing tools and discuss the potential sociocultural implications of integrating AI and human input in the writing process.

    
\end{comment}


==> sections/1-introduction.tex <==
%\kenneth{TODO HCOMP: Need to mention more crowdsourcing}

Large language models (LLMs) have recently dominated the conversations of automated writing assistants for their ability to produce fluent text and follow instructions.
In areas where providing meaningful writing assistance was challenging, such as novel or poem writing, explorations were made possible thanks to LLMs.
For example,
Wordcraft allowed users to co-write stories with a language model interactively~\cite{10.1145/3490099.3511105,ippolito2022creative};
Dramatron allowed theatre professionals to co-write screenplays interactively with LLM-powered features to generate characters, titles, story plots, location descriptions, and dialogues~\cite{mirowski2022co}; and
CoPoet was built for LLM-human collaborative poetry writing~\cite{chakrabarty2022help}.
%Sparks used a language model to generate ideas to support Twitter tutorial writing~\cite{10.1145/3532106.3533533};
%\kenneth{TODO: Add one more creative writing projects here. Maybe the one with Salesforce?}
%GPT-3.5 was also used to help emerging writers develop stories~\cite{chakrabarty2023creativity}.
% \kenneth{TODO: \cite{chakrabarty2023creativity} has been accepted at C\&C 2024. Update the citations.}
%\kenneth{TODO HCOMP: Add 1 more newer papers that just used ONE model: }
%These works offered a glimpse into how writers can incorporate a powerful text generator into their writing workflows. 
%These works provided a sneak peek into how writers might use a powerful text generator in their workflows.
These projects offered exciting peeks into how writers might incorporate an LLM into their creative workflows.
However, real-world writing is more complicated than using one single assistant. 
In reality, people work with multiple writing assistants and multiple people over a course of writing that spans days, months, or even years.
Academics use auto-completion, ChatGPT, and Grammarly while collaborating with co-authors, advisors, and editors. 
Artists employ various tools in their compositions, choosing specific ones based on their creative needs at different stages. 
%\kenneth{I feel like the argument should not just be ``because users use a lot of tools at the same time'' but rather ``we don't compare AI with human support''}\cy{Agree. But in the context, it would seem to be we want to compare AI with co-authors/editors (which is probably also interesting!) but we are doing this with workers.}
%Some poets have experimented with GPT-2 and GPT-3, recognizing distinct strengths. 
%The factors impacting writers when choosing, using, and interacting with AIs or humans remain a fascinating, unexplored problem.
%The factors affecting 
%How do writers choose, use, and interact with multiple AIs and humans in their writing processes remains a fascinating yet under-explored problem.
How writers choose, use, and interact with multiple AI assistants and humans in their writing processes remains a fascinating yet under-explored area.
%\kenneth{set up for using crowd}
%are a largely unexplored research area.




%\kenneth{TODO HCOMP: Use this \cite{bellemare2024divergent} to justify the need of crowd. Humans are still better than LLM in creative writing. Maybe also cite Steven's CHI paper: \cite{10.1145/3613904.3642834}}


This paper introduces \system, a web-based text editor that allows \textbf{creative writers to elicit inspiration from a variety of AI models as well as online crowd workers}.
\system combines AI-powered writing assistants with crowd-writing systems~\cite{feldman2021we}, offering immediate, fluent AI suggestions alongside the potentially more creative but slower responses from crowd workers.
Unlike many previous projects that relied solely on LLMs to support creative writing, \system keeps crowd workers as a viable source of inspiration because creative writing remains a domain where humans still exhibit significant advantages~\cite{bellemare2024divergent} even though LLMs have surpassed crowd workers in many tasks~\cite{10.1145/3613904.3642834,gilardi2023chatgpt}.\footnote{A study suggested many crowd workers use LLMs for writing tasks~\cite{veselovsky2023artificial}. Our user study was entirely completed before November 30, 2022, \ie, before LLMs were widely available, so these concerns do not apply to our work.}
%\kenneth{TODO HCOMP: Add one more citation here}
In this work, we define ``inspiration'' as a brief text snippet produced to enhance a story draft in development.
Writers using \system can select a portion of their draft and request inspiration from four different sources: 
\textbf{{\em (i)} crowd workers (\crowd), 
{\em (ii)} a story plot generation model (\plot), 
{\em (iii)} GPT-3 that generates follow-up story arcs (\gptplot), and 
{\em (iv)} GPT-3 that continues the given story (\gptc)}. 
%Each option allows customization, such as specifying additional instructions or choosing the number of generated inspirations. 
%\system records all user behavioral logs and writing logs for analysis.
We use the term \textit{``flock''} to characterize the ensemble of AIs and the crowd within \system, highlighting the collaborative yet independent nature of these entities. 
%Each entity contributes uniquely towards the collective goal of supporting the writing process without necessarily coordinating directly with one another.
%the coordination happens through the user though -Kenneth


To examine how writers interact with different AIs and crowd workers within \system, we conducted a three-part user study. 
In our pilot study, two creative writers used \system for three days to write 1,000-word stories, leading to system adjustments like adding undo and redo functions. 
%and setting a 50-word minimum for user-selected text. 
The main study then involved six writers using \system for a week to craft 2,000-word stories. 
Additionally, one participant used \system for a month to write stories totaling over 50,000 words. %during NaNoWriMo. 
%We conducted semi-structured interviews with all participants after each study period.
%Initially, in the pilot study, two creative writers used \system over three days to develop 1,000-word stories. 
%This phase led to final adjustments in \system, such as 
%adding undo and redo functions and 
%setting a minimum word count (50 words) for user-selected text. 
%Subsequently, the main study involved six writers using \system for one week to craft 2,000-word stories. 
%Following this, one participant extended their use of \system for an additional month to write four short stories totaling over 50,000 words during National Novel Writing Month (NaNoWriMo).
%After each study period, we conducted one-on-one semi-structured interviews with all participants. 
%to gather insights into their usage, experiences, and views on \system.
As a result, 
%Throughout our study, 
we found that participants consistently decreased their use of crowds in favor of AIs throughout the study.
By the end, the \crowd option was the least used by all the participants.
%\kenneth{TODO HCOMP: Is this true???}
Interviews with the participants further revealed their reasons for favoring AI, including crowds' slow response times and inconsistent quality. 
%As a result, we found that participants increasingly used AI instead of crowds throughout the study. 
%Over the course of our study, we found that participants increasingly favored AI over crowds.
%By the end, Crowd was the least popular option. 
Meanwhile, preferences for the three AI options varied:
\gptc was the most used by the majority, though some preferred \plot. 
\gptc also had the greatest impact on the participants' written content, measured by the similarity of texts written immediately after viewing inspirations.
We conclude the paper by discussing the necessity for extremely high-quality human involvement for creativity support in an era where AI already provides instant, decent aid. 
We also analyze our qualitative findings through a sociocultural lens, discussing the risks and implications of writers using LLM outputs to conform to the norms of their target discourse community. 
These insights, collectively, can inform the future development of writing assistants.
%in creative writing.



%-------------------- dead kitten ------------------------------

\begin{comment}

\bigskip

%We also analyzed 
%The writing and user logs were also extensively analyzed.
%We also analyzed both the writing and user logs.
As a result,
we found that participants increasingly used AI instead of crowds throughout the study. 
By the end, Crowd was the least popular option. 
Meanwhile, preferences for the three AI options varied; GPT3-Completion was the most used by the majority, though some preferred the Story Plot Generator. 
GPT3-Completion also had the greatest measurable impact on the participants' written content, measured by text similarity of texts written immediately after viewing inspirations.
Participant interviews further revealed their reasons for favoring AI, including crowds' slow response times and inconsistent quality. 


As a result, we found that, over the course of our study, participants used fewer crowds and more AIs over time. 
Toward the end of the study, \crowd was the least used option for all the participants.
Among all three AI options, preference varies across participants.
\gptc was the most frequently used option for most participants, but some participants used \plot most frequently.
The writing logs also show that \gptc has the most measurable impact on participants' written content, measured by various text similarity metrics, for the texts written right after reading the generated inspiration.
The interviews with participants further show the reasons that they decided to use less of crowd, such as long latencies and varied response quality. 
%To wrap up, we discuss a sociocultural point of view 


reduce their use of crowd options and eventually no on practically used it.
We also learn that, while GPT-3


\kenneth{--------------------------- KENNETH WORKING HERE--------------------}
\bigskip


%from CSCW draft
This paper introduces \system, a web-based text editor that allows writers to elicit inspiration from a variety of AI models as well as online crowd workers.
%An ``inspiration,'' as we defined it, is a piece of short text produced to help the writer develop an ongoing draft.
We define ``inspiration'' as a short text segment produced to help the writer develop an ongoing draft.
%\kenneth{If we ``inspiration}
%aid the writer in refining their ongoing draft. 
During the writing process, writers can send any part of the working draft to \system to request inspiration from a text-generation model of their choice (including GPT-3) or from online crowd workers. 
We then conducted a three-part user study with \system.
As a pilot study, two writers were recruited to use \system for three days to develop a story of 1,000 words.
We adjusted the system based on the pilot users' feedback and proceeded with the main study, in which six writers used \system for one week to write 2,000-word stories.
Finally, after the main study, one participant continued to use \system for an additional month to compose four short stories with more than 50,000 words for National Novel Writing Month (NaNoWriMo).
We conducted semi-structured interviews with participants to understand their use of, experience with, and perspectives toward \system.

After the user study,
we first analyzed the participants' behavior and writing logs.
This data highlighted differences in usage frequency, word count changes, and the impact of generated texts on the content participants produced across all text-generation models and the crowd.
We complemented these findings with a qualitative analysis of interview transcripts, which demonstrated participants' perceptions and comparisons between the models and the crowd.
Based on these findings, we laid out a set of design recommendations for future intelligent writing assistants.
Additionally, our analysis hinted at norm-setting behavior in some writers and potential biases in LLM's output, which we briefly explored using sociocultural theories of writing.


\kenneth{KENNETH IS WORKING HERE}

%from the old CHI/CSCW draft
We also analyzed the relationship between generated inspirations and writing logs,
aiming to provide insight into at what points in their process the writers requested inspiration and what they did once the inspiration was available.

Our work resulted in real-world feedback on how authors relate to technological assistance, informing the design of future writing assistants powered by advanced language technologies.
\kenneth{I kinda want to say something more well but let's see. The paper is quite long.}

Through qualitative analysis of interviews and user logs, we found that writers sometimes used \system's generated texts to double-check their ideas with those ``silential relations.''
Drawing on the theory of discourse community, we argue that writers learn and negotiate the conventions or ``voice''~\cite{matsuda2001voice} of their chosen discourse community by seeing what LLMs generate in various scenarios.
We further demonstrate the explanatory power of the discourse community theory by using it to interpret 
%why experienced writers found LLMs less useful than novice writers, 
what writers might expect from LLMs and the apparent risks of using LLMs to learn a community's voice.
Our core contribution is to offer a new perspective on the interactions between writers and LLMs, informing the design of future writing assistants that prioritize text generation.



Large language models (LLMs) have recently dominated the conversations of automated writing assistants for their ability to produce long, fluent text and to follow human instructions.
In the spaces where building intelligent writing assistance was considered challenging, like creative writing, several exciting recent explorations were made possible thanks to these powerful text generation models. %should we say something to hint it's ONE model?
%find papers after 2021
For example, 
Wordcraft... alllow to interact with A.... 
DeepMind Dramaton is powered by THE...
Elephant (maybe it's multiple)?
and 
Katy's creative writing work (maybe poetry).
These studies showcased how novelists and poets can incorporate a powerful generation model into their writing workflows.
However, interacting with one AI model or one writing assistant is not the whole story.

LLMs are everywhere; people think they will take over the world.
But, in reality, people work with multiple AI assistants and also people at the same time-- 
Ph.D. students write using auto-completion, ChatGPT, and Grammarly, and also with their co-authors, advisors, even editors.
People also have access to GPT-3 and GPT-4 at the same time, and they did have some quality-cost trade-offs.
What factors would impact them when choosing, using, and interacting with AIs vs. humans remains unexplored.
So here we come to help!
We built \system, a system that allows users to choose the source of inspiration.



LLMs are everywhere; people think they will take over the world.
But, in reality, people work with multiple AI assistants and also people at the same time-- 
Ph.D. students write using auto-completion, ChatGPT, and Grammarly, and also with their co-authors, advisors, even editors.
People also have access to GPT-3 and GPT-4 at the same time, and they did have some quality-cost trade-offs.
What factors would impact them when choosing, using, and interacting with AIs vs. humans remains unexplored.
So here we come to help!
We built \system, a system that allows users to choose the source of inspiration.

    
\end{comment}


==> sections/2-related-work.tex <==
%\subsection{LLM and Creative Writing Support}


%\kenneth{Crowd writing: What has been done and what underlying research questions they studied (which could potentially be studied usine LLMs?)}

%\paragraph{Crowd Writing.}
%\kenneth{Probably mention the two key writing-related motivation of crowd-writing systems: (1) is to study how text gen and understanding capability be integrated to support writing (LLM's ability), and (2) how well-scoped human involvement can be used to help writing or to create great outcome (non LLM related motivation)--- In the discussion, we will basically say (1) is gone and we should focus on (2)}

Crowd writing systems have traditionally explored two key aspects:
(\textit{i}) integrating text generation and understanding capabilities to support writing, and (\textit{ii}) leveraging well-scoped human involvement to enhance writing outcomes.
Early crowd writing systems primarily explored using collective efforts to tackle complex writing tasks~\cite{feldman2021we}, such as 
decomposing and recomposing complicated writing tasks~\cite{kittur2011crowdforge,kim2017mechanical} and 
outsourcing writing jobs to online crowds~\cite{bernstein2010soylent,hahn2016knowledge} or collaborators~\cite{teevan2016supporting}. 
In creative writing, systems like \oldSystem enabled writers to gather ideas from crowd workers~\cite{heteroglossia-huang-2020}.

The advent of LLMs has shifted this landscape. Recent research explores LLMs' integration into writing processes~\cite{coenen2021wordcraft,Yuan2022Wordcraft,Gero2022Sparks,Ippolito2022Creative}.
As the field evolves, there's growing interest in the second key aspect of crowd writing systems - effective human involvement in the writing process.

% Among the few systems focusing on creative writing assistance, Heteroglossia allowed writers to gather story ideas from crowd workers~\cite{heteroglossia-huang-2020}.
% However, \oldSystem was developed before the LLM era and did not incorporate AI into its framework.



\paragraph{Automated Creative Writing Assistants.}

%\subsection{Has prior work tried to use AI to support creative writing?}
%\kenneth{YES. A lot of them! Google's study and DeepMind's study were all focusing on single AI.}
%\kenneth{Given ALL these, why do we still need to study THIS? Because (1) literature hole (weak argument) and (2) we need to understand how people use LLMs in reality so that we can improve and iterate!}
%\cy{This is from the CSCW review. \say{The References list 95 works, however, the Related Work section is rather short. A structured Related Work section would have been nice, that informs about the discourse community theory, and the importance of the sociocultural point of view, but also technical work, and work that investigated interactions with LLMs but with different goals, e.g. by authors such as Elena Glassman, Qian Yang, Kenneth Arnold, Daniel Buschek.}}

%\kenneth{----------------------- KENNETH IS WORKING HERE: BEGINS -----------------}

%Researchers created prototype systems that advanced technological support for writing.
Before the recent rise of LLMs, writing assistant research typically centered on the technical and business domain~\cite{greer2016introduction} or language learners, with a few exceptions dedicated to creative writing.
For example,
CreativeHelp generated follow-up sentences %as a suggestion 
for creative writing~\cite{roemmele2015creative};
%InkWell imitated the writer’s personality traits and revised the draft to provide stylistic variations~\cite{gabriel2015inkwell};
Metaphoria helped writers create metaphors by connecting concepts automatically~\cite{10.1145/3290605.3300526};
%Heteroglossia allowed creative writers to elicit story plot ideas from online crowd workers via a text editor~\cite{heteroglossia-huang-2020};
and 
\citeauthor{Clark:2018:CWM:3172944.3172983} had machines take turns coauthoring stories with users.
%\kenneth{TODO CY: Add a few more famous recent LLM+creative writing studies.}
The recent rise of LLMs has led to numerous studies investigating 
%The recent rise of LLMs has spurred numerous studies on 
how people interact with systems capable of 
generating fluent and lengthy texts~\cite{lee2022coauthor}, 
offering high-quality suggestions and feedback for writing~\cite{10.1145/3490099.3511105,Wan2023It,AlexHow,mirowski2022co,Ippolito2022Creative}, and
generating interesting inspirations~\cite{roemmele2021inspiration,10.1145/3532106.3533533}. %and
%providing non-diegetic prompting~\cite{Dang2023Choice}. 
%and introducing new forms of support~\cite{arnold2021generative}.
Moreover, recent research has also started to explore how writers and creators perceive AI co-creation~\cite{rezwana2023user,feuston2021putting,lawton2023tool}. 
For example, \citet{gero2023social} investigated the circumstances under which creative writers might opt for AI-powered assistants over peers or mentors.
While previous research often focused on writers using a single assistant, our study examined scenarios where writers choose from multiple sources of assistance.
%While most of these research focused on how a single writing assistant can aid users, our system provided multiple types of support.








%\kenneth{This following part is about 150 words. Maybe we could remove it.}

%\kenneth{TODO HCOMP: mention crowd writing + crowdsourced FAQ-gen (UCSD)}


\begin{comment}

One key challenge in studying creative writing assistants is assessing these systems' impact on users' workflows.
Highly controlled studies with short timespans and assigned writing tasks make recording writing processes easier.\kenneth{TODO CY: Add a few citations that use in-lab studies. Including Elena's study (CHI)}
However, how people write in these studies differs significantly from how they engage in their own writing.
A user study session could range from 10 to 75 minutes, but composing an article or story in reality might take days or weeks.
On the other hand, an open-ended, loosely controlled deployment study could span over days, weeks, even months, making participants' writing processes more realistic.\kenneth{TODO CY: Add a few citations that use deployment studies. Dramatron. WordCraft. Heteroglossia. WearWrite}
However, in such studies, user intent can only be inferred from the writing log or by asking participants to recall long after it happened, so some data will not be captured with good resolution, as in-lab study methods, such as think-aloud studies, can do.
In our study, we took the latter approach and conducted a 7-day-long deployment study, acknowledging potential tradeoffs.
    
\end{comment}



















% \cite{feuston2021putting}
% \say{there are key differences between how AI and human analysts practice induction and interpret phenomena [43]. Within this context, the focus of our study is to address how qualitative scholars understand the use of machine learning techniques in qualitative research, exploring their existing practices and openness to working with AI.}
% \say{Lubars and Tan propose a framework of task delegability for human-AI collaboration [30], arguing that we need to consider what AI should do, rather than what it can do, and proposing four factors for evaluating task delegation to AI: motivation, difficulty, risk, and trust.}
% \say{examining how the use of AI impacts different stages of qualitative analysis, including data exploration and coding.}

% Researchers have analyzed different writing capabilities among writers themselves, the crowd, and automatic systems \cite{greer2016introduction}.
% "The self has access to context and can handle a wide range of tasks well, but is subject to cognitive blocks. The crowd has limited access to context and can handle a narrower range of tasks, but can do so at scale. Automation is even better at handling volume, but provides the most narrow and rigid task support and is error-prone.”

% \textbf{Researchers also conducted studies to understand users' perspectives on ethical challenges in human-AI co-creativity \cite{rezwana2023user}.} 
% % 
% The ethical issues they found included ownership, leadership, AI feedback and evaluation, accountability, data collection and usage, personified communicative AI, and AI access to public data.

\begin{comment}

\subsection{Just Avon's notes}
\subsubsection{Irrelevant}
\cite{gmeiner2023exploring} %3D CAD, no AI v.s AI or AI v.s. human
\say{how engineering designers learn to work with AI-based design tools.} 
\say{We find that designers face many challenges in learning to effectively co-create with current systems, including challenges in understanding and adjusting AI outputs and in communicating their design goals.}

\subsubsection{Belong to Related work part 1}
[already cited] CoAuthor: Designing a Human-AI Collaborative Writing Dataset for Exploring Language Model Capabilities (CHI'22)

\subsubsection{Maybe useful somehow}


% May be useful for discussion about discourse community
\textbf{Researchers found that writers refer to their target readers and their publishing venues to seek alignment. \cite{yang2019sketching}.} %Sketching NLP
% 
They found that writers \say{often picked those who are close to their target readers as their “beta-readers." Participants worked to translate their often egocentric writing into a style that meets the expectations and needs of their target readers. Many read other documents from their target venue to infer the expected length, lexical complexity, or level of detail that they should write in} \cite{yang2019sketching}
%
They \say{see this as an excellent opportunity for NLP technologies to help authors, as algorithms are good at rapidly summarizing or characterizing a sizable collection of documents. We therefore designed an “ask your reader" function. It mines documents from an author-identifed venue. The author can request insights about these documents or make comparisons between their own writing against it. For instance, “Am I writing too formally?"} 


\end{comment}

% \subsubsection{Finding summary of gero2023}
% \paragraph{without quotes}
% [Planning] human and AI
% --human: brainstorming
% --AI: research assistant

% [Translation] AI
% --human:
% --AI: see some possibilities laid out

% [Reviewing] human
% --human: different perspectives; if people can understand
% --AI: concerned about explanation or implicit value judgment

% [Motivation/Affirmation]
% --general: need affirmation; what she had created was legible to others.

% [Availability] AI:
% --human: writers would be mindful of reading request
% --AI: non-implosive; mundane; different from peers’ response

% [Individuality (details of the actor)] human
% --human: writers know an individual’s personality
% --AI: the impossibility of a “universal” reader

% [Trust/Vulnerability] AI
% --general: understood the writer’s unique characteristic
% --human: required to be trustworthy people
% --AI: good for critical response

% [Intention] human
% --human: writers need to explain their intention of the writing contents
% --AI: can’t understand writers’ intentions

% [Authenticity] human
% --human: more me(writer) in them
% --AI: what if readers recognize that it’s not the writer’s voice?; ownership;

% [Creativity] mixed opinions about AI
% AI: AI is the past; trigger an idea

% \paragraph{with quotes}
% [Planning] human and AI
% --human: brainstorming
% "working on a science fiction novel, described having a great brainstorming relationship with her teenage son, who also loves science fiction and enjoyed swapping plot ideas."
% --AI: research assistant
% "While some writers were hesitant to use a computer for fact-checking, others were open to a computer program that was “kind of like having a research assistant”"

% [Translation] AI
% --human:
% N/A
% --AI:
% "turn to thesauruses (W8 said “sometimes I’m really frustrated because I feel like the words I’m using don’t have the right texture or sound”), or turn to a computer program.
% Several writers, both those who used SudoWrite and those who didn’t, discussed using a computer program to help them with writer’s block. W14 described a hypothetical situation, “where I’m not sure how to proceed, but [could use the computer] to see some possibilities laid out.” S16 talked about how “it’s a lot easier to react to something and make modifications than to come up with something from nothing.” S20 talked about how SudoWrite brought ease to her writing, saying she could “pound her head against the wall” and “open up other books and flip through for inspiration”, but SudoWrite eliminates this struggle for her when she feels stuck."

% [Reviewing] human
% --human: different perspectives; if people can understand
% "Almost all discussed the importance of needing other people’s perspectives, whether on a poem (W10 said “people can see things in my poems that I don’t necessarily see”) or a newspaper article (W2 said “I was mostly interested in how it was working structurally, and the clarity of the analysis”)."
% --AI: concerned about explanation or implicit value juegement
% "In this way, writers expected an explanation for feedback, especially if it came from a computer. W5 said, “I would want to be able to interface with the program to understand why it thinks it needs revision.”"
% "Feedback is often laden with implicit value judgments. W1 discussed the situation of a computer giving her feedback that a certain passage is boring, saying “I would be so angry!” because, for example, sometimes the point of a book may be to explore plotlessness. Specificity or being able to question feedback is a way to move past value judgements into more concrete territory."

% [Motivation/Affirmation]
% --general
% "When writers talked about how they were influenced by other people, or the kind of support they tended to seek out, they often talked about motivation or affirmation as an important part of the writing process. The writers talked about how writing, especially writing a large project like a novel, was a vulnerable, ambitious, and often lonely activity. W4, who was working on the script for a TV show pilot, said, “If I don’t periodically get validation? The operation is a bust.”
% The importance of affirmation ran across most of the writers we interviewed. Writers talked about having no idea how their writing would come across, or wanting something “to confirm it’s not trash”. S20 described the first time someone else talked about the characters in her novel as if they were real people, and the importance of this indication that what she had created (i.e. the fictional world) was legible to others.
% Writers described this as being distinct from feedback used for reviewing or revision. Writers described that when they’re looking for support, it can be useful to know or be explicit about if they are looking for help with revision or motivation. As W7 explained, “A loRteovifewtiimnges you want validation, but you asked for feedback, or you want feedback, but you’re asking for validation.”"


% [Availability] AI: 
% --human:
% "Many writers noted that requesting help with their writing was an imposition. By asking for support, they are asking a friend or acquaintance for time, and were always mindful of such a request."
% --AI: non-implosive; mundane; different from peers' response 
% "Several writers noted that a computer program wouldn’t have these issues. S19 said, “The advantage that SudoWrite has is availability, because you can’t just walk up to a person at any time of the day or middle of the night and go, Hey, I have this idea. How about this?” Even non-SudoWrite users noted that making use of a computer program wouldn’t be an imposition on the computer. W14 said, “I’m imagining things [to request from a computer] that feel too mundane somehow to ask someone for their time.”"
% "While computers were understood as being always available, writers didn’t necessarily want replicas of their not-always-available peers. W2 said that because he does have access to peers, a program that replicated his peers’ response would thus be uninteresting. Instead, he would want a computer program to give him something different, something that wasn’t currently available to him."


% [Individuality (details of the actor)] human
% --human: writers know an individual's personality
% "Writers would come to learn specific characteristics of people that would modulate when they’d turn to these people for support. For instance, W8 discussed how the life experience or writing interests of a peer would dictate who she would send it to, saying
% “Since my brother is also Indian, if I want to know how something reads to another Indian person, I will show him. But then if I’m writing a story about girlhood, I’ll send it to my friend Jen, who also writes about girlhood.” S19 even described situations where negative feedback may indicate he’s on the right track, saying “I can kind of place their feedback into preference categories. . . there’s certain aspects where I know if a certain person doesn’t like that, then it’s exactly what I want to achieve in that part of the story.""
% --AI: the impossibility of a “universal” reader
% "When discussing a computer support actor, several writers talked about the impossibility of a “universal” reader. W10 worried that computers would represent only a dominant perspective, saying,
% “The ‘universal’ perspective has been the perspective of cis straight white men and any other perspective is just not considered univer- sal.” Others noted that, based on their understanding of how such a computer program might work, it would reflect generalizations of its training data, and lose the individuality that people provide. W6 described the uniqueness of humans in this way: “Let’s just say there’s a 1\%, that is unpredictable, a response they’ll have that does not fit the pattern . . . I’m interested in that 1%, too. I like the inherent unpredictability of a person.”
% SudoWrite users were able to articulate the unique characteristics of SudoWrite. S20 describes their sense of SudoWrite:
% A peer is someone who is grounded in a very specific point of view, and culture and identity and preference, you know, their own reading habits and a peer can be a very valuable partner . . . when I turn to SudoWrite, I know that I’m getting feedback and interactions with my work that is not personal at all . . . The amount of information on hand that SudoWrite is pulling from is this vast trove. And that’s something that a human could never, even if they’re well read, could really never achieve."

% [Trust/Vulnerability] AI
% --general
% "At other times trust was about how well the support actor under- stood the writer’s unique characteristics. Someone who had read their work before, who understood their writing ‘crutches’ and where they tend to be strong, would give better feedback than someone who didn’t know anything about them."
% --human: required to be trustworthy people
% N/A
% --AI: good for critical response
% "Sometimes trust had to do with privacy. W7 talked about how sharing her work with someone meant she’s “going to show them a very deep inner part of [her] mind”, and mentioned that there may be times when you don’t want to share something “extremely sensitive” with a person yet. In this situation, a computer may be a useful intermediary step as a kind of anonymous support actor."
% "Relatedly, trust also had to do with vulnerability. Many writers talked about the emotional difficulty of getting feedback on their work, and that sometimes they were looking for affirmation, while other times they wanted a more critical response. W10 says, “If it’s a poem that is really close to my heart, sometimes if I get feedback on it, I don’t even look at the feedback for a couple of days until I’m ready to receive it.” W14 talked about the fear of not being good enough, and noted that a computer seemed to not trigger this kind of vulnerability. Her comments about this articulate in general the kind of fears writers have when getting support"

% [Intention] human
% --human: writers need to explain their intention of the writing contents
% "Support actors wouldn’t always understand their intention. Writ- ers talked about the difficulty of finding good readers who understood or respected their personal vision for a piece. Sometimes they’d have to discuss with a reader what they were trying to do in the writing, in order for the reader to know if they achieved that."
% --AI: can't understand writers' intentions
% "When it came to computers, this idea of sharing the intention was often a roadblock. W1 talked about how “it’s not like the computer can understand what you want to say; they can only see what you have written.”"

% [Authenticity] human
% --human: more me(writer) in them
% some writers had existing close relationships with other writers, and these writers often left strong marks on their writing. In describing what was different between her brother influencing her writing and a computer, W8 said, “it somehow feels like there’s more of me in it, maybe because we have a relationship with each other.” W5 discussed how he gives trust to his fiancé in a multitude of ways, and he can’t imagine giving that same trust to a computer.
% --AI: what if readers recognize that it's not the writer's voice?; ownership;
% "First, some writers worried not about their own sense of authenticity, but the sense of their reader. Would the reader notice that the writing was not always in the writer’s own voice?"
% "writers worried not just about ownership of words on the page, but how even viewing suggestions might derail them. W1 commented that, “once something is on the page it becomes just a bit harder to imagine what else it can be.”"

% [Creativity] mixed opinions about AI
% AI: AI is the past; trigger an idea
% "Writers disagreed on the subject. W1 proposed that what computers produce comes out of what they have seen (i.e. training data) and thus computers “help us understand or generalize what is a well-trodden path”. W11 thought a computer would be better at historical novels than science fiction ones for this same reason; he trusted the computer to understand the past but not predict the future. W6 said, "I sort of hold the line in believing that there is something irreducibly human" that a computer could never replicate. Similarly W10 said, “I think very highly of all my friends’ creative brains. But I don’t think that way about a computer.”"
% "Others, especially SudoWrite users, were more positive about the creative potential of a computer. W10 even said she may feel bad compared to the computer’s abilities, saying “I feel like it would bruise my ego if I couldn’t figure out how to end one of my poems, but a computer came up with this really great idea.” S19 related Su- doWrite to role playing games that used dice rolls to trigger an idea for world building, saying SudoWrite is essentially a more evocative version of that. S20 discussed a moment when she had SudoWrite complete a scene she had started writing, and it “introduced a completely new character, and gave him two stanzas of a song that he was singing... I was floored.” Even still, S20 said her creativity is her
% “humanity” and was not worried about a computer replacing that. She thought writers should be open to new technology, and make use of whatever was available to them."

%-------------------- dead kitten --------------------------
\begin{comment}



%\kenneth{-------------------- KENNETH IS WORKING HERE: BEGIN ------------------------}

\paragraph{How Do Creators Choose Assistance for Creative Work?}
%\subsection{How do users select who or what to get help from when doing creative work?}

HCI researchers have studied how creators choose support providers for their creative work between humans and AI. 
%
For example, \citet{rezwana2023user} found that
%conducted a study to understand users' perspectives on ethical challenges in human-AI co-%creativity. They found that
when co-creating with AI, creators were concerned about ownership, leadership, AI feedback and evaluation, accountability, data collection and usage, personified communicative AI, and AI access to public data.
% 
In the field of human-AI collaboration, researchers have studied creators' perceptions and practices about the complementary of AI and humans~\cite{feuston2021putting,lawton2023tool}.
\citet{lubars2019ask} argued that designers need to consider what AI \textit{should} do rather than what it \textit{can} do and developed a framework on human perception of task delegation to AI.
%which included four factors for assessing task delegation to AI (motivation, difficulty, risk, and trust).
Along this line, prior work has studied the differences between AI and humans, specifically for writing support.
%Prior work has researched writers' trust in feedback created by humans and machines. 
%\avon{Not sure if we could add this. This is more like professional writing than creative writing. But I think it's okay because writing itself is creative.}
For example, \citet{liaqat2021collaborating} found that English learners significantly preferred machine feedback over peer feedback, but peers' feedback excelled in identifying errors due to shared challenges.
%For example, \citet{liaqat2021collaborating} studied the confidence of English learners in the feedback to English essay writing provided by instructors, peers, and machines.
%They found that English learners accepted machine feedback significantly more than peer feedback.
%Yet, the advantage of peers' feedback is that peers could better identify errors as they have similar challenges.
% 
Researchers have also analyzed different writing capabilities among writers themselves, the crowd, and automatic systems~\cite{greer2016introduction,gero2023social}. 
For example, \citet{gero2023social} has investigated when and why creative writers might choose AI-supportive systems rather than peer or mentor for support.
They interviewed creative writers about their experiences and what kinds of support they want from whom, when, and why.
They identified that writers select support based on their desires, perceptions of potential support actors, and their own values related to the writing process.
For example, human assistance is approached with social consideration, to avoid overburdening others and such concern is lifted when seeking support from AI;
whereas, writers also doubt AI's ability to align with their creative intentions and values. 
% They also asked questions about supports they (don't) want from hypothetical computational tools that could act ``at the level of a peer.''\kenneth{TODO CY: What does this sentence mean? We should probably say one or two sentences here about their conclusion?}
% Question template: If a computer program could _____ like a teacher or peer could, would you use it? Why or why not?
% suggest places to revise; rewrite sections; write in a gap; finish a piece; continue something when you felt stuck; something about reader perspective; where a reader might get stuck or bored or confused; write into something out of domain (explanation or science fiction details); do research for you or describe a city or summarize a new technology
\citet{mckee2020ethics} pointed out one important difference between human and AI writing is that AI lacks the sense of implicit ethics codes.
\kenneth{TODO CY: Well Dramatran is a deployment study. Maybe just say prior work did not have their requests to human built in their systems?}
While researchers have discussed how creators and writers choose support providers for their creative work between humans and AIs, few studies built systems that come with a feature allowing for direct requests for human support.
% deployed an in-the-wild study. 
%Although prior research has deployed systems that combined AI and human support~\cite{huang2018evorus}, few aimed to understand writers' support-seeking behaviors between humans and AIs.
%\kenneth{TODO Kenneth: Add}



%\kenneth{-------------------- KENNETH IS WORKING HERE: END ------------------------}



%\subsection{Human-AI Collaboration}
\subsubsection{What has prior work studied on how humans select from a group of AIs?}
%begin with general things e.g., algorithm audit, bot market, etc
\kenneth{There are some prior work that studies how people interact with multiple AI agents-- Cite Amos' famous pirate game paper-- and how to audit multiple AI models, BUT not really in the context of writing or content creation. Writing is a complex series of decision-making process.}

Following recent developments in AI-supportive systems for creative work, such as creative writing, HCI researchers have studied the differences in strengths and use cases among various AI-based creativity-supportive systems~\cite{hwang2022too, gmeiner2023dimensions}. 
% 
\citet{hwang2022too} reviewed current products that support creative processes and separated AI co-creative tools into categories that support various levels of each of the three co-creative dimensions: introducing "surprises" and uncertainty, yielding new ideas and\/or outputs, and human leadership in co-creativity.
% 
Researchers also analyzed how different AI functions could support different writing tasks. For example, \citet{gmeiner2023dimensions} analyzed LLM capabilities in writing support in terms of writing task complexity and output quality.




% \textbf{A review paper about current products that support creative processes \cite{hwang2022too}.} 
% % 
% This paper separates AI co-creative tools into four categories: the editors, the transformers, the blenders, and the generators. Each of the categories supports various levels of each of the three co-creative dimensions: introducing "surprises" and uncertainty, yielding new ideas and\/or outputs, and human leadership in co-creativity.
% The author thinks that the merit of AI creativity-supportive tools is providing surprising, non-human outcomes. The downsides include (1) auto-generation reduces the opportunities for humans to spend time on and get inspired by boring tasks, (2) the lack of explainability and clues for optimization of its outcomes, (3) it does not support multi-human collaborative creative processes, and (4) users lack agency.




\subsubsection{What has prior work studied on how humans select when to use AI and when to use humans?}
% \paragraph{begin with general study}
\kenneth{Cite Evorus/Chorus maybe. Also some papers on complementary of AI and human.}

% (PENDING, because this belongs to the first part of the related work)
% HCI researchers also studied creators' perspectives regarding seeking support from AI.
% Creators find AI has several advantages, including a, b, and c. Yet, when e, d, and f, people have concerns seeking support from AI.
% For example, ...


% For example, in X field, Y found that X creators prefer to choose AI when a, b, c, while they prefer to seek help from humans when d, e, f.
% Human-AI collaborative system papers might mention something related to human vs. AI support.
% If no relevant papers, then we discuss when AI and no AI.

% Previous research has studied how AI co-creates with creators vs. participatory design or co-create/co-design.



% \paragraph{say more about writing specifically}
\kenneth{Also probably cite jeff bigham yash paper to say it's not that easy? Also cite the machine translation paper.}
\kenneth{Again, basically saying those are }
Similarly, HCI researchers have studied how creators choose support providers for their creative work between humans and AI. 
% 
\citet{rezwana2023user} conducted a study to understand users' perspectives on ethical challenges in human-AI co-creativity. They found that, when co-creating with AI, creators were concerned about ownership, leadership, AI feedback and evaluation, accountability, data collection and usage, personified communicative AI, and AI access to public data. 
% 
In the field of human-AI collaboration, researchers have studied creators' perceptions and practices about the complementary of AI and humans~\cite{feuston2021putting, lawton2023tool}. \citet{lubars2019ask} argued that designers need to consider what AI \textit{should} do rather than what it \textit{can} do. They developed a framework on human perception of task delegation to AI, which included four factors for assessing task delegation to AI (motivation, difficulty, risk, and trust).

Along this line of work, prior work has also studied the differences between AI and humans for writing support. Prior work has researched writers' trust in feedback created by humans and machines. 
\avon{Not sure if we could add this. This is more like professional writing than creative writing. But I think it's okay because writing itself is creative.}
For example, \citet{liaqat2021collaborating} studied the confidence of English language learners in the feedback to English essay writing provided by instructors, peers, and machines. They found that English language learners accept machine feedback significantly more than peer feedback. Yet, the advantage of peers' feedback is that peers could better identify errors as they have similar challenges.
% 
Researchers have analyzed different writing capabilities among writers themselves, the crowd, and automatic systems \cite{greer2016introduction, gero2023social}. 
For example, \citet{gero2023social} has investigated when and why creative writers might choose AI-supportive systems rather than peer or mentor for support. They interviewed creative writers about their experiences and what kinds of support they want from whom, when, and why. They also asked questions about supports they (don't) want from hypothetical computational tools that could act ``at the level of a peer.''
% Question template: If a computer program could _____ like a teacher or peer could, would you use it? Why or why not?
% suggest places to revise; rewrite sections; write in a gap; finish a piece; continue something when you felt stuck; something about reader perspective; where a reader might get stuck or bored or confused; write into something out of domain (explanation or science fiction details); do research for you or describe a city or summarize a new technology
\citet{mckee2020ethics} pointed out one important difference between human and AI writing is that AI lacks the sense of implicit ethics codes.

While researchers have discussed how creators and writers choose support providers for their creative work between humans and AIs, few studies deployed an in-the-wild study. Although prior research has deployed systems that combined AI and human support (e.g., ~\cite{huang2018evorus}), few aim to understand writers' support-seeking behaviors between humans and AIs.



\kenneth{----------------------- KENNETH IS WORKING HERE: ENDS -----------------}


%then be specific, cite Evorus/Chorus

%edited by CK
%Over the years, improvements to writing assistants have made the writing process easier~\cite{greer2016introduction}. 
Researchers developed prototype systems that pushed the envelope of technological support for writing.
%, such as decomposing and recomposing complicated writing tasks~\cite{kittur2011crowdforge}; outsourcing writing jobs to online crowds~\cite{bernstein2010soylent,hahn2016knowledge}, collaborators~\cite{teevan2016supporting}, or the writers themselves~\cite{teevan2014selfsourcing}; or even allowing users to write papers using smartwatches~\cite{nebeling2016wearwrite}.
%edited by CK
In the earlier era, 
while research into writing assistants often focuses on the technical and business domain~\cite{greer2016introduction} or to language learners~\cite{tay2018skipflow,wang2018automatic,muangkammuen-fukumoto-2020-multi,schmaltz2016sentence,chollampatt2018multilayer,bryant2019bea,omelianchuk2020gector,kaneko2020encoder,grundkiewicz2019neural,homma2020non},
%with features such as essay scoring~\cite{tay2018skipflow,wang2018automatic,muangkammuen-fukumoto-2020-multi} or grammar correction~\cite{schmaltz2016sentence,chollampatt2018multilayer,bryant2019bea,omelianchuk2020gector,kaneko2020encoder,grundkiewicz2019neural,homma2020non}, 
a few exceptions aimed to support creative writing.
CreativeHelp generated a follow-up sentence as a suggestion for creative writing~\cite{roemmele2015creative}.
InkWell imitated the writer’s personality traits and revised the draft to provide stylistic variations~\cite{gabriel2015inkwell}.
Metaphoria helped writers create metaphors by connecting concepts automatically~\cite{10.1145/3290605.3300526}.
Heteroglossia allowed creative writers to elicit story plot ideas from online crowd workers via a text editor~\cite{huang2020heteroglossia}.
\citeauthor{Clark:2018:CWM:3172944.3172983} had machines take turns coauthoring stories with users~\cite{Clark:2018:CWM:3172944.3172983}.
With the advent of large language models (LLMs),
many recent works studied how people would interact with systems that can
produce fluent and long texts (CoAuthor~\cite{lee2022coauthor}),
give high-quality and general suggestions for writing (WordCraft~\cite{10.1145/3490099.3511105,ippolito2022creative}, \citeauthor{Wan2023It}'s work~\cite{Wan2023It}, and \citeauthor{AlexHow}'s work~\cite{AlexHow}, Dramatron~\cite{mirowski2022co}),
produce interesting inspirations (\citeauthor{roemmele2021inspiration}'s work~\cite{roemmele2021inspiration} and Sparks~\cite{10.1145/3532106.3533533}),
personalize models (LMCanvas~\cite{Kim2023LMCanvas}),
provide non-diegetic prompting~\cite{Dang2023Choice},
or even new forms of supports~\cite{KennethGenerative}.

A common challenge in studying creative support tools is measuring their impact on users' workflows and outcomes.
Highly controlled studies with short timespans and assigned writing tasks make it easier to record writing processes and compare writing outcomes.
However, how people write in these studies differs significantly from how people engage in their own writing.
A user study session could range from 10 to 75 minutes, but composing an article or a story, in reality, might take days or weeks.
%These studies' assigned writing tasks, such as the essay section of Standardized American Tests (SATs)~\cite{dang2022beyond}, or using 10 to 20 minutes to write a short story for a given prompt~\cite{lee2022coauthor,10.1145/3511599}, are also artificial.
Only a few prior works focusing on creative writing conducted user studies beyond minutes-long user sessions.
For example, Heteroglossia conducted a three-day-long study with two creative writers~\cite{huang2020heteroglossia}, and WearWrite was deployed to seven participants for one week~\cite{nebeling2016wearwrite}.


% Other works needed to cite:
% - Choice Over Control: How Users Write with Large Language Models using Diegetic and Non-Diegetic Prompting~\cite{Dang2023Choice}
% - LMCanvas: Object-Oriented Interaction to Personalize Large Language Model-Powered Writing Environments~\cite{Kim2023LMCanvas}
% “It Felt Like Having a Second Mind”: Investigating Human-AI Co-creativity in Prewriting with Large Language Models~\cite{Wan2023It}
% Generative Models can Help Writers without Writing for Them~\cite{KennethGenerative}
% How Novelists Use Generative Language Models: An Exploratory User Study~\cite{AlexHow}




%However, despite the exciting technological progress, we still know little about the real-world impact of these writing-assistant tools and how authors would incorporate them into their writing practices.
%The user studies of these newly-emerged writing assistants have often focused on the writing assistants' capabilities rather than unveiling how people would use them.
%They were short-term studies that assigned tasks rather than engaging with the subject's own writing. 



%edited by CK
A common challenge in studying creative support tools is measuring their impact on users' workflows and outcomes.
Highly controlled studies with short timespans and assigned writing tasks make it easier to record writing processes and compare writing outcomes.
However, how people write in these studies differs significantly from how people engage in their own writing.
A user study session could range from 10 to 75 minutes, but composing an article or a story, in reality, might take days or weeks.
%These studies' assigned writing tasks, such as the essay section of Standardized American Tests (SATs)~\cite{dang2022beyond}, or using 10 to 20 minutes to write a short story for a given prompt~\cite{lee2022coauthor,10.1145/3511599}, are also artificial.
Only a few prior works focusing on creative writing conducted user studies beyond minutes-long user sessions.
For example, Heteroglossia conducted a three-day-long study with two creative writers~\cite{huang2020heteroglossia}, and WearWrite was deployed to seven participants for one week~\cite{nebeling2016wearwrite}.

\end{comment}

==> sections/3-1-user-interface.tex <==
%\kenneth{What is this you want to do?}\cy{Want to say \system is built as an website. But I think the interface kind of show that.}





%In this work, we define ``suggestion'' as a short text snippet produced to help story development.
%edited by CK
Figure~\ref{fig:interface} overviews \system's user workflow and interface components,
%Our design goals for \system are discussed in Appendix~\ref{subsec:design-principles}.
%\kenneth{TODO HCOMP: Add a few sentences about design goals.}
%\system 
%designed with a set of design goals in mind, and we believe it is useful to make these design goals explicit to our readers.
%These goals were extensively discussed internally among our authors.
%As shown in Figure~\ref{fig:interface}, 
%The \system interface 
which we describe as follows.
%\oldSystem is a system that allows users to request asynchronous support; 
We followed \oldSystem's design and presented writing suggestions in a sidebar.

%contains three main components: the {\em (i)} Text Editor, {\em (ii)} suggestion Panel, and {\em (iii)} Sidebar.

%\subsubsection{Text Editor: Write Story and Send suggestion Requests (\Cref{fig:interface}A)}



%\begin{itemize}
% \kenneth{Need to say we followed \oldSystem}


%edited by CK
%\item
%\textbf{Text Editor: Writing the Story and Sending suggestion Requests (\Cref{fig:interface}A).}
\paragraph{Text Editor (\Cref{fig:interface}A): Writing the Story and Sending Suggestion Requests.}
Users write stories inside the text editor, which was implemented using \texttt{Quill.js} (quilljs.com),
%\footnote{Quill.js: \url{https://quilljs.com/}} 
like many other online text editors.
%\kenneth{TODO HCOMP: Convert the footnote to citation.}
To request a new suggestion, the user first selects a snippet of text from the current draft and clicks the ``Get Inspired'' button on the editor's toolbar.
After clicking the button, the Task Creation Panel (Step 2 in \Cref{fig:interface})
%(\Cref{fig:interface-create-task}) 
pops up to let the user select the generation model and set task-specific parameters, such as instructions or number of ideas.
When finished, the user clicks the ``Create'' button, and \system starts the suggestion generation process in the backend and displays the result in the Sidebar and Suggestion Panel when it is ready.

%The Task Creation Panel includes several components: \textit{Content}, which is the selected story snippet used to generate suggestion; \textit{Task Type}, where users specify one of the four suggestion functions provided; and \textit{Task-Specific Parameters}, which vary for each task, such as ``Number of Ideas'' and ``Instruction'' for the \crowd task.
%After clicking the ``Create'' button, \system starts the suggestion generation process in the backend and displays the result in the Sidebar and Suggestion Panel when it is ready.












%(see the Task Creation Panel paragraph below).
%The following subsection details the steps of requesting a new suggestion.
In the text editor, the text spans that have been used for producing suggestions will be highlighted in light blue (\Cref{fig:interface}A).
When the user's mouse cursor focuses on a particular suggestion in the Sidebar (\Cref{fig:interface}C), the corresponding text snippet will be highlighted in yellow (Step 1 in \Cref{fig:interface}).
%Users can toggle the highlighting by clicking the ``No-Highlight'' button in the top right corner to avoid distraction when writing in the text editor.
The editor monitors the user's editing logs; it automatically saves the document and the editing logs if there is no activity for five seconds.



%edited by CK
%\item
\paragraph{Suggestion Panel (\Cref{fig:interface}B): Displaying the Generated Suggestions and Enabling Requests for More Suggestions.}
Once the suggestion is produced, the Suggestion Panel displays the meta information and generated text of a suggestion.
%If the user wants to obtain more suggestion with the same setting (\ie, a selected text snippet, generation model, etc.), the user can click the ``Get Another Plot'' button.
To get more suggestion with the same setting (\ie, using the same selected text snippet and generation method), the user can click the ``Get Another Plot'' button.
Within a suggestion, each generation outcome is displayed in different tabs (\eg, the ``Plot-1'' and ``Plot-2'' tabs in \Cref{fig:interface}B). 
%so that 
\system can record which suggestion (tab) is being read.




%edited by CK

\paragraph{Sidebar (\Cref{fig:interface}C): Navigating All the Suggestions.}
We name a suggestion requested by the user a ``suggestion task.''
The Sidebar lists all the suggestion tasks. %of the current document.
For each suggestion task listed in the Sidebar, \system shows the task type and a brief snippet of the corresponding draft.
When the user clicks a suggestion task, \system displays the suggestion's content in the Suggestion Panel (\Cref{fig:interface}B) and brings users to the corresponding text snippet.



%\end{itemize}

%--------------- dead kitten ------------

\begin{comment}

\item
\textbf{Sidebar: Navigate All the Suggestions (\Cref{fig:interface}C).}
We name a suggestion requested by the user a ``suggestion task''.
The Sidebar lists all the suggestion tasks of the current document.
For each suggestion task listed in the Sidebar, \system shows the task type and a brief snippet of the corresponding draft.
When the user clicks a suggestion task, \system displays the suggestion's content in the Suggestion Panel (\Cref{fig:interface}B) and brings users 
to the corresponding text snippet.
%The spinning circle and the thumbs-up icon indicate the task is under process and ready, respectively.
%The ``NEW'' badge tells users that a new inspiring plot is coming and ready to read.
%Clicking the suggestion task, \system will show the suggestion result and bring users
%to the corresponding story snippet.


\item
\textbf{Suggestion Panel: Display the Generated Suggestions and Request More Ideas. (\Cref{fig:interface}B).}
Once the suggestion is produced, the Suggestion Panel displays the meta information and generated text of a suggestion.
If the user wants to obtain more suggestion with the same setting ({\em i.e.} selected text snippet, generation model, etc.), the user can click the \textbf{``Get Another Plot''} button.
Within one suggestion, each generation outcome will be displayed in different tabs (\eg, Plot-1, Plot-2. See \Cref{fig:interface}B) so that \system can explicitly capture which suggestion is being read.

\item 
\textbf{Text Editor: Write Story and Send Suggestion Requests (\Cref{fig:interface}A).}
Users write stories inside the text editor, which was implemented using \texttt{Quill.js},\footnote{Quill.js: \url{https://quilljs.com/}} similar to many other online text editors~\cite{lee2022coauthor}.\kenneth{Maybe add a citation to other editor?}
The editor monitors the user's editing logs; it automatically saves the document and the editing logs if there are no activities for five seconds.
%\paragraph{Send Suggestion Requests.}
To request a new suggestion, the user first selects a snippet of text from the current draft and clicks the \textbf{``Get Inspired''} button on the editor's toolbar.
After clicking the ``Get Inspired'' button, the task creation panel (\Cref{fig:interface-create-task}) will pop up to let the user select the generation model and add instructions when needed. 
The following subsection details the steps of requesting a new suggestion (Section~\ref{subsec:generation-model}).
In the text editor, the text spans that have been used for producing suggestions will be highlighted in light blue (see \Cref{fig:interface}A).
When the user's mouse cursor focuses on one particular suggestion in the Sidebar (\Cref{fig:interface}C), the corresponding text snippet will be highlighted in yellow (see Step 1 in \Cref{fig:interface}).
The users can toggle the highlighting by clicking the ``No-Hightlight'' button on the top right corner to avoid distraction when writing in the text editor.

As shown in \Cref{fig:interface}, the \system interface contains three main components:
{\em (i)} text editor, 
{\em (ii)} suggestion panel and
{\em (iii)} sidebar.
\cy{Make sure to mention that the overall design rational is for ``story plot ideas''}
\kenneth{What does this mean?}\cy{Want to emphasize we try to provide ``suggestions'' even though we have an auto-complete function.}

\paragraph{Text Editor}
The text editor, as shown in \Cref{fig:interface} (A), is implemented using \texttt{Quill.js}\footnote{Quill.js: \url{https://quilljs.com/}}.
Users can write their stories directly in the text editor.
We use Delta provided by Quill.js to monitor all the editing logs from users.
The text editor will automatically save the document along with the editing logs if there is no activities for five seconds.
In the text editor, texts that have been used for suggestion tasks will be highlighted 
in light blue.
Texts highlighted in yellow are the suggestion task users' mouse are focusing on.
Clicking a highlighted text, the corresponding suggestion task will pop out in the sidebar.
Users can also toggle the highlighting by clicking the ``No-Hightlight'' button on the top right corner.

\paragraph{Sidebar}
The sidebar, \Cref{fig:interface} (B), shows the suggestion task list.
For each of the suggestion task, we show the type of the suggestion task 
and the briefing of the selected story draft.
The spinning circle and the thumbs-up icon indicate the task is under process and ready, respectively.
The ``NEW'' badge tells users that a new inspiring plot is coming and ready to read.
Clicking the suggestion task, \system will show the suggestion result and bring users 
to the corresponding story snippet.

\paragraph{Suggestion Panel}
As shown in \Cref{fig:interface} (B),
the suggestion panel shows the task parameters and settings on the top;
and the generated suggestions on the bottom.
Suggestions are placed in different tabs (\eg, Plot-1, Plot-2, and so on) 
so that \system can explicitly capture which suggestion is being read.
For most of the task (except the crowd ideation task),
users can retrieve more suggestions with the same setting by clicking the 
``Get Another Plot'' button.




\end{comment}

==> sections/3-2-request-task.tex <==
%\input{tables/inspiration-tasks}

%^\kenneth{HCOMP TODO: I suggest we use the following terms to describe the four options (1) \crowd, (2) \plot, (3) \gptplot, and (4) \gptc}

Writers using \system can select a portion of their draft and request suggestions from one of the following four different sources: 
\textbf{{\em (i)} crowd workers (\crowd), 
{\em (ii)} a story plot generation model (\plot), 
{\em (iii)} GPT-3 that generates follow-up story arcs (\gptplot), and 
{\em (iv)} GPT-3 that completes the given story (\gptc).}
These are called suggestion ``task types'', which we detail below:
\textbf{1) \crowd:}
The \crowd task allows the user to create human intelligence tasks on Amazon Mechanical Turk to ask crowd workers to provide plot ideas that continue the selected story snippet.
Users can specify the number of story ideas they want (the default is three) and write additional instructions for the workers.
We obtained the code and interface from Heteroglossia~\cite{heteroglossia-huang-2020} and adapted them for this function.


%\begin{enumerate}


%edited by CK
%\item
\paragraph{\crowd: Asking Online Crowd Workers to Provide Plot Ideas.}
The \crowd task allows the user to create human intelligence tasks on Amazon Mechanical Turk to ask crowd workers to provide plot ideas that continue the selected story snippet.
Users can specify the number of story ideas they want (the default is three) and write additional instructions for the workers.
We obtained the code and interface from Heteroglossia~\cite{heteroglossia-huang-2020} and adapted them for this function.
%, which can include character descriptions, story summaries, or creative guidance. 
%While crowd workers can provide high-quality ideas, this method has higher response latency compared to other AI-based options.




%edited by CK
%\item
\paragraph{\plot: AI Forecasting What Would Happen in the Next 20 or 100 Sentences.}
The \plot option generates a few sentences describing possible next events in the story based on the selected snippet.
This method, developed by~\citet{plotp2023huang}, builds on the Semantic Frame Forecast model~\cite{huang-huang-2021-semantic}, which predicts likely future events in a story based on its past.
We obtained their data, code, and model to implement this component.
\system offered two models for this function:
%\begin{itemize}
%\item 
(1) One generates a \textbf{near future} plot, summarizing what would happen in the next 20 sentences.
(2)
%\item
The other generates a \textbf{far future} plot, summarizing what would happen in the next 100 sentences.
%\end{itemize}
%One generates a story plot for the \textit{near future} (about 20 sentences),
%and the other generates a story plot for the \textit{far future} (about 100 sentences).
Users can specify which model to use when creating a suggestion task.
This method, based on GPT-2, is expected to yield more divergent outputs than more powerful LLMs~\cite{zhu_luo_2022,10.1115/1.4056220}.







%This method is built on top of GPT-2 and is expected to provide more divergent outputs compared to more powerful LLMs~\cite{zhu_luo_2022,10.1115/1.4056220}.
%\kenneth{TODO HCOMP: Why so? What's the intuition?}\cy{GPT2 is less accurate and thus more divergent and random.}




%edited by CK
%\item
\paragraph{\gptplot: GPT-3 Producing a Follow-Up Story Arc.}
%LLMs have shown their power in zero-shot learning and language generation~\cite{NEURIPS2020_1457c0d6,chowdhery2022palm,smith2022using,thoppilan2022lamda}.
% In this task, 
%we take advantage of GPT-3~\cite{NEURIPS2020_1457c0d6}, a publicly available LLM,
%to generate possible plot ideas to continue the story.
%Users can also provide instructions to the model to generate suitable plot ideas.
%The instructions can be constraints for the desired direction, contextual information about the characters, and more.
We asked GPT-3~\cite{NEURIPS2020_1457c0d6} to produce a follow-up story arc using the prompt:
\textit{
    Given the previous story: \texttt{\small[story-snippet]}.
    Follow the instruction: \texttt{\small[instruction]} to describe the follow-up story arc using 50 words.
}
\texttt{\small[story-snippet]} and \texttt{\small[instruction]} are the placeholder for the selected snippet and the instruction.
% \vspace{.5pc}
% \texttt{
%   {\list{}{\leftmargin=0.3in\rightmargin=0.3in}
%     Given the previous story: [story-snippet] \newline
%     Follow the instruction: [instruction] to describe the follow-up story arc using 50 words:
%   }%
%   {\endlist}
% }
% \begin{quote}
% \small
% Given the previous story: [story-snippet] \newline
% Follow the instruction: [instruction] to describe the follow-up story arc using 50 words:
% \end{quote} \vspace{.5pc}
% } 








%edited by CK
%\item 
\paragraph{\gptc: GPT-3 Continuing the Story.}
The \gptc task continues the story based on the selected content by running the text completion function using GPT-3 model (\texttt{text-davanci-003}).
% \kenneth{This needs to be more specific. What does it mean to tell GPT3 to do so? Is it an API call function without needing to give it any promopt?}
%\kenneth{I mean, we kinda need to remind people GPT-3 has this option via API (right?) and it's kinda different than using a prompt (for today's ChatGPT) saying ``continue the story''}
%\cy{How about this?}
This is the only function that generates ready-to-use content; the other three provide plot ideas for users to develop.












%---------------------- dead kitten ----------------

\begin{comment}






\subsection{Task Creation Panel.}


%TC:ignore
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{figures/create-task-large.png}
    \caption{Task creation panel shows the remaining credits and the selected story snippet along with the inspiration task configuration fields. \cy{Could we have a higher-quality figure?}}
    \label{fig:interface-create-task}
\end{figure}
%TC:endignore    



%edited by CK
To request a new inspiration, the user first selects a snippet of text from the current draft and clicks the ``Get Inspired'' button, which causes the Task Creation Panel to pop up (Step 2 in \Cref{fig:interface}).
%\Cref{fig:interface-create-task} shows 
The Task Creation Panel contains the following components:\kenneth{TODO HCOMP: This needs to rewrite to be a paragraph. Also remove all the Appendix pointers.}

\begin{itemize}


%edited by CK
\item 
\textbf{Credits.}
The user's remaining credit to create tasks.
Since the four inspiration task types have different costs, \system uses a credit system to indicate the cost to users.
We describe the credit system in \Cref{subsec:credit-system}.

%edited by CK
\item
\textbf{Content.}
The selected story snippet that will be used to generate inspiration.


%eidted by CK
\item 
\textbf{Task Type.}
\system provides four inspiration functions, as described above.
Users can specify the task type here.


%edited by CK
\item 
\textbf{Task-Specific Parameters.}
Different inspiration tasks take different parameters.
For example, ``Number of Ideas'' and ``Instruction'' are parameters for the Crowd Plot Generation task.

%edited by CK
\item
\textbf{Cost.}
The cost of each task is determined by the task type, the length of the selected text snippet, and some task-specific parameters.
\system computes and shows the cost on the fly (see \Cref{subsec:credit-system}.) 

%$(We describe the credit system in \Cref{subsec:implementation}.)



\end{itemize}

%After clicking the ``Create'' button, \system starts the inspiration generation process in the backend and displays the result in the Sidebar and Inspiration Panel when it is ready.

%edited by CK
After clicking the ``Create'' button, \system starts the inspiration generation process in the backend and displays the result in the Sidebar and Inspiration Panel when it is ready.

More details, including the credit systems and the implementations of the four text generation models and the crowd tasks, can be found in \Cref{subsec:implementation}.

generating ready-to-use content.
In contrast, the other three functions provide plot ideas that users need to develop further.










%\end{enumerate}



The \gptc task asks GPT-3 to simply continue the story.
%We used GPT-3 without any prompt designs, \ie, input of the selected story snippet as the prompt, and asked GPT-3 to continue the story.
Note that this function is the only one that generates ready-to-use contents; whereas the above three functions are expected to generate plot ideas and users should develop the contents by themselves.


The \plot option produces a few sentences that describe what could happen next in the story given the selected story snippet.
This technique was proposed and developed by~\citet{plotp2023huang}, who expanded the concepts of Semantic Frame Forecast~\cite{huang-huang-2021-semantic}, a predicting model that forecasts likely events that would occur in the forthcoming story based on the past story.
We obtained their data, code, and model to implement this component.
\system provides two models for this function.
One generates a story plot for the \textit{near future} (about 20 sentences),
and the other generates a story plot for the \textit{far future} (about 100 sentences).
Users can specify which model to use when creating a suggestion task.
This method is built on top of GPT-2 and is expected to provide more divergent outputs compared to powerful LLMs~\cite{zhu_luo_2022,10.1115/1.4056220}.
%\avon{If you can find the quotes, maybe "writers want more interesting and divergent plot" could be a good finding?}

The users can specify how many story ideas they want to obtain and also write instructions to guide workers.
The instructions to crowd workers could be descriptions of particular characters in the story, summaries of the previous story, or creative guidance.
It is worth noting that, although crowd workers can fully understand the instruction and provide higher-quality ideas, Crowd Plot Generation is financially more expensive than other task types.
It also has a high response latency, especially compared with other AI-based approaches.








These are referred to as different inspiration \textit{task types}, 
which we detail in the following.

The following details each type.











We refer to these different approaches as different inspiration {\em task types}.
This subsection details the four types of inspiration tasks.\kenneth{TODO HCOMP: Change the word ``subsection''}


%edited by CK
\system supports four different approaches for generating inspirations: 
{\em (i)} \crowd, 
{\em (ii)} \plot, 
{\em (iii)} \gptplot, and 
{\em (iv)} \gptc. 
We refer to these different approaches as different inspiration {\em task types}.
Users can freely select their preferred task types and manually supplement additional instructions when needed.
This subsection details the four types of inspiration tasks.\kenneth{TODO HCOMP: Change the word ``subsection''}



\item \textbf{Cost.}
The cost of each task is decided by the task type, the length of the selected text snippet, and some task-specific parameters. 
\system computes and shows the cost on the fly. 
We will discuss the credit system in the next subsection.


\item \textbf{Task-Specific Parameters.}
Different inspiration tasks take different parameters. 
For example, ``Number of Ideas'' and ``Instruction'' are parameters for the Crowd Plot Generation task. 

\item \textbf{Task Type.}
\system provides four inspiration functions:
{\em (i)} Crowd Plot Generation,
{\em (ii)} AI Plot Generation, 
{\em (iii)} AI Plot Generation with Guidance, and
{\em (iv)} Auto-Completion.
Users can specify the task type here.

\item \textbf{Content.}
The selected story snippet that will be used to generate inspiration.

\item \textbf{Credits.}
The user's remaining credit to create tasks. Since the four inspiration task types cost differently, \system used a credit system to signify the cost to users. We will discuss the credit system in the next subsection.

To request a new inspiration, the user first selects a snippet of text from the current draft and clicks the ``Get Inspired'' button, and the Task Creation Panel will pop up.
\Cref{fig:interface-create-task} shows the Task Creation Panel, which contains the following components:

\item \textbf{Auto-Completion: GPT-3 Continues the Story.}
The Auto-Completion task asks an LLM to simply continue the story, meaning that the output is ready to use. 
We used GPT-3 without any prompt designs, {\em i.e.,} input the selected story snippet as the prompt and ask GPT-3 to continue the story.

\item \textbf{AI Plot Generation with Guidance: GPT-3 Produces the Follow-Up story Arc.}
Large language models (LLMs) have shown their power in zero-shot learning and language generation~\cite{NEURIPS2020_1457c0d6,chowdhery2022palm,smith2022using,thoppilan2022lamda}.
In this task, we take the advantage of GPT-3~\cite{NEURIPS2020_1457c0d6}, a publicly available PLM.
In particular, instead of asking the model to simply continue the story snippet, we ask GPT-3 to produce the follow-up story arc using the following prompt:


\item \textbf{AI Plot Generation: AI Forecasts What Would Happen in the Next 20 or 100 Sentences.}
AI Plot Generation produces a few sentences that describe what would happen next in the story, given the selected story snippet.
This technique was proposed and developed by Huang \etal~\cite{plotp2023huang}, which expanded the concepts of Semantic Frame Forecast~\cite{huang-huang-2021-semantic}, a predicting model that forecasts likely events that would occur in the forthcoming story based on the past story.
We obtained their data, code, and model to implement this component.
\system provides two models: one generates a story plot for the near future (about 20 sentences), and the other generates a story plot for the far future (about 100 sentences).
Users can specify which model to use when creating a suggestion task.


\item \textbf{Crowd Plot Generation: Ask Online Crowd Workers to Provide Plot Ideas.}
The crowd plot generation task allows the user to create Human Intelligence Tasks (HITs) on Amazon Mechanical Turk (MTurk) to ask crowd workers to provide plot ideas to continue the select story snippet.
The users can specify how many story ideas they want to obtain and also write a piece of instruction to guide workers.
The instruction to crowd workers could be descriptions of particular characters in the story, summaries of the previous story, or any creative guidance.
It is noteworthy that, although crowd workers could fully understand the instruction and provide higher-quality ideas, Crowd Plot Generation is financially more expensive than other task types.
It also has a high response latency, especially compared with other AI-based approaches.


\system supports four different approaches to generate inspiration:
{\em (i)} Crowd Plot Generation,
{\em (ii)} AI Plot Generation, 
{\em (iii)} AI Plot Generation with Guidance, and
{\em (iv)} Auto-Completion.
We refer to these different approaches as different inspiration {\em task types}.
Users can freely select their preferred task type and manually supplement additional instructions when needed. This subsection details the four types of inspiration tasks.

\kenneth{Say we will discuss technical details in later sections.}




To create a new task, users need to first select a snippet from the draft and then
click the ``Get Inspired'' button.
\system will generate inspirations based on the selected story snippet.
After clicking the ``Get Inspired'' button, the task creation panel will pop out.
The task creation panel, as shown in \Cref{fig:interface-create-task}, contains a few components:
\begin{itemize}[]
    \item \textbf{Credits}. The user's remaining credit to create tasks. Since the four provided inspiration functions cost differently, we implemented a credit system to balance among them.
    \item \textbf{Content}. The selected story snippet for generating inspirations.
    \item \textbf{Task Type}. \system provides four inspiration functions: (\textit{i}) Crowd Plot Generation, (\textit{ii}) AI plot generation, (\textit{iii}) AI plot generation with guidance, and (\textit{iv}) auto-completion. Users can specify the type of inspiration task here.
    \item \textbf{Task-specific Parameters}. Different inspiration tasks take different parameters. For example, ``Number of Ideas'' and ``Instruction'' are parameters for the crowd plot generation task. 
    \item \textbf{Cost}. The cost of task depends on the task type, the length of the selected story snippet and some of the task-specific parameters. \system computes and reports the cost on-the-fly. Note that when the remaining credit is lower than the cost, users will not be able to create the task.
\end{itemize}

After clicking the ``Create'' button, \system starts the inspiration generation process in the back-end and displays the result in the Sidebar and Inspiration Panel when it is ready.


After clicking the ``Create'' button, \system will start working on the inspiration generation task in the backend and display the result when it is ready.
Next, we will describe the four inspiration tasks in detail.
\todo[inline]{Say more about Table 1}





\bigskip

%\subsection{Inspiration Task}
\system allows users to retrieve ideas via four different inspiration tasks:
\begin{enumerate*}[label=(\roman*)]
    \item Crowd Plot Generation;
    \item AI Plot Generation;
    \item AI Plot Generation with Guidance;
    \item Auto-completion;
\end{enumerate*}
\Cref{tab:inspiration-task} shows the basic difference between tasks. 
We will detail how each task works in the following sections.


\subsubsection{Crowd Plot Generation}
The crowd plot generation task allow users to 
create Human Intelligence Task (HIT) on Amazon Mechanical Turk (AMT)
and ask crowd workers to provide plot ideas to continue the select story snippet.
In this task, \system allows users to specify 
(\textit{i}) how many story plot ideas they would like to retrieve;
and (\textit{ii}) an instruction to guide workers.
The instruction can be character settings, summaries of the previous story, potential future direction, and so on.
\Cref{fig:interface-crowd-ideation} shows the interface for workers when collecting story plot ideas.
The instruction specified by users are shown as a note (\Cref{fig:interface-create-task} (A));
the selected story snippet is shown in the story panel (\Cref{fig:interface-create-task} (B)); 
users are required to write down a 50-word story plot idea to continue the provided story in the idea panel (\Cref{fig:interface-create-task} (C)).
We added three locks, a 30-second submission lock, a reach-to-the-bottom lock in the story panel, and a 50-words lock, to prevent workers from performing undesired works.
Aiming at paying hourly wage of \$10 dollars, for each of the task, we set up the payment according to:
\begin{align}
\begin{split}
    Cost(HIT) & = Cost(Reading) + Cost(Writing) \\
              & = [Time(Reading) + Time(Writing)] \times \$10 (dollars / hours) \\
              & = [ \#words / 200 (Minutes) + 6 (Minutes)] \times \$ 1/6 (dollars / minutes) \\
              & \simeq  \$ \ \#words / 1000 + \$1.0 \ (dollars)
\end{split}  
\end{align}
where the reading time is estimated by the average reading time (200 - 300 words per minutes on LCD monitors) for English native speaker~\cite{siegenthaler2012reading}, the writing time is estimated empirically, and \#words is the user selected story snippet.

From user side, the cost of the task is computed by:
\begin{equation}
    Cost(Crowd\_Plot\_Generation\_Task) = \#ideas * Cost(HIT) * 1.2
\end{equation}
where $1.2$ refers to the 20\% AMT processing fee\footnote{Amazon Mechanical Turk - Pricing: \url{https://www.mturk.com/pricing}}. 

Although, the crowd plot generation are relatively expensive, 
workers are able to fully understand the instruction and provide high quality ideas.
Another limitation is the high latency especially when compared to AI-based approaches.
We will investigate the effect in the user study section.

% We generally believe that crowd can provide ideas in a much better quality and clearly follow the insturction. However, the latency will be higher meaning that it would take more time to get the inspirations.

\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{figures/Story-block-formulation.pdf}
    \hfill
    \includegraphics[width=0.59\linewidth]{figures/story-block-example.pdf}
    \caption{The AI plot generation task is built on top of the story block formulation~\cite{huang-huang-2021-semantic}. Given the selected story snippet (story block n), we first (A) summarize the story snippet (story block n) with three sentences~\cite{zheng-lapata-2019-sentence} and (B) predict what would happen next (story block n+1) in terms of semantic frame representation~\cite{huang-huang-2021-semantic}. Combining the information together, a sequence-to-sequence model is used to generate the future three sentence summary (story block n+1).\kenneth{This figure is not easy to understand. Send me the original files.}}
    \label{fig:pipeline-ai-plot-generation}
\end{figure}

\subsubsection{AI Plot Generation}
\cy{Probably mention story block formulation here. It will make the following content easier to understand (?)}
The AI plot generation function allows users to 
call our language models to generate a few sentence about what would happen next 
given the selected story snippet.
\system provides two models: one generates story plot for a near future (about 20 sentences);
and one for a far future (about 100 sentences). 
Users can specify which model to use when creating a suggestion task.

\Cref{fig:pipeline-ai-plot-generation} shows the whole pipeline of our AI plot generation model.
Given a selected story snippet, our model will 
(\textit{i}) generate a three-sentence summary using PacSum~\cite{zheng-lapata-2019-sentence}; 
and (\textit{ii}) extract and predict the future semantic frame representation~\cite{huang-huang-2021-semantic}.
The concatenated information then goes into our future plot generation model to generate a three-sentence follow-up story plot. 
Next, we will describe each component in detail:

\textbf{Summarizing Story Snippet.}
We summarize the story snippet using Pacsum~\cite{zheng-lapata-2019-sentence}, an extractive summarization model.
The Pacsum's score weightings are finetuned for the story domain using the Shmoop corpus~\cite{chaudhury2019shmoop}.
We notice that including nonconsecutive conversations leads to confusing summaries and hurts the summary quality.
As a result, we identify conversations by matching double quotation marks with regular expressions and penalize sentences in conversations to prioritize descriptive sentences.
For each of the story snippet, we extract a three-sentence summary.

\textbf{Semantic Frame Forecasting.}
Huang \etal~\cite{huang-huang-2021-semantic} formulated a long story as a sequence of story blocks, where each story block contains a fixed number of sentences (\eg, 20-sentence story block, 100-sentence story block, and so on). 
They, then, introduced the semantic frame representation to 
encode high-level semantic information from a story block into a fixed-length vector.
The semantic frame representation tells us the how important a corresponding 
semantic frame (\eg, \texttt{Prohibiting\_or\_licensing}, \texttt{Size}, and so on)
in FrameNet~\cite{baker1998berkeley} is. 
Thus, forecasting a future semantic frame representation essentially means predicting 
what would happen next. 
We followed Huang \etal's work~\cite{huang-huang-2021-semantic} to train LGBM models~\cite{ke2017lightgbm} on Bookcorpus~\cite{Zhu_2015_ICCV}.
However, instead of training models on the same size of story blocks 
(\eg, using information 20-sentence story block to predict the semantic frame representation in the following 20-sentence story block), 
we varied the size of the source story block with the size of 10, 20, 50, and 100 sentences. 
Given the two target models, near future model (20-sentence) and distant future model (100-sentence), 
a total of eight (four source sizes $\times$ two target sizes) are trained.

\textbf{Future Plot Generation.}
We take advantage of the semantic frame representation to encode 
longer contextual information and Huang \etal's semantic frame forecast model~\cite{huang-huang-2021-semantic} 
to generate the guidance of the follow-up story block. 
Note that the predicted frame representation contains semantic units that are expected to happen 
in the next story block which serves as a \textbf{goal-setting} function in the writing process theory~\cite{flower1981cognitive}.
We build a sequence-to-sequence model using the pre-trained GPT-2 model 
where two GPT-2 models are used for encoder and decoder respectively. 
The frame representation of story block \textit{n} and 
the predicted frame representation of story block \textit{n+1} are passed 
through a linear layer to fit the GPT-2's word embedding dimension 
and fed into the GPT-2 encoder as two words.
The encoder input can be described as:
$
    \mathbf{X} = [ \mathbf{x}_1, \mathbf{x}_2, \cdots, \mathbf{x}_n, \mathbf{f}_{n}, \hat{\mathbf{f}}_{n+1} ]
$
where $\mathbf{x}_i$ is the $i$-th word in the story plot of story block \textit{n},
$\mathbf{f}_{n}$ is the adapted frame representation of story block \textit{n},
and $\hat{\mathbf{f}}_{n+1}$ is the LGBM's prediction of the frame representation for story block \textit{n+1}.
We added the \texttt{<START>} and \texttt{<PAD>} token to the model to enable the sequence-to-sequence training framework.
The sequence $[ \texttt{<START>}, y_1, y_2, \cdots, y_n, \texttt{<|endoftext|>} ]$, 
where $y_i$ is the $i$-th word in the story plot of story block \textit{n+1}, 
is used as the target to train the decoder.

We trained the future plot generation models on Bookcorpus~\cite{Zhu_2015_ICCV}.
The near future model and the far future model are trained 
on story blocks with 20 sentences and 100 sentences, respectively.
All the required information, (i) summary for story block \textit{n}, 
(ii) semantic frame representation $\mathbf{f}_{n}$, 
and (iii) predicted semantic frame representation $\hat{\mathbf{f}}_{n+1}$,
were obtained by running the above mentioned methods.
The models were built using HuggingFace's GPT-2 implementation~\cite{wolf2019huggingface} 
where \texttt{gpt2-large} is used for initialization.
We trained the models using AdamW optimizer~\cite{loshchilov2017decoupled} 
with learning rate = $1e-5$, weight decay factor = $1e-4$, and batch size = 32 for 200 epochs.
The models were validated every 10k epochs, the ones with the highest ROUGE-2 F1 scores were kept.
For decoding, we used Top-k sampling with top-k = 100, temperature = 0.8, and repetition penalty = 3.0.

Since we own the AI plot generation model, we simply set the cost to 0 for users.


\subsubsection{AI Plot Generation with Guidance}
Large pre-trained language models (PLM) has shown their power in zero-shot learning and language generation~\cite{}. 
In this task, we take the advantage of GPT-3~\cite{}, a publicly available PLM.
Different from asking the model to simply continue the story snippet, 
we ask the model to provide the follow-up story arc to continue the story.
\begin{quote}
Given the previous story: \newline
\space    [story-snippet] \newline
Follow the instruction: \newline
    [instruction] \newline
to describe the follow-up story arc using 50 words: \newline
\end{quote}
where \texttt{[story-snippet]} and \texttt{[instruction]} are the placeholder for the user selected story snippet and the specified instruction. 
We use temperature sampling method for decoding, 
where temperature = 0.8, max\_tokens = 100, top\_p = 0.95,
frequency\_penalty = 0.5, and presence\_penalty = 0.5. 
Given that GPT-3 is a mature product where a plenty of GPUs are used to accelerate the computing, we manually add a five-second delay to reduce the latency difference this and the AI plot generation model. 
The price is computed according to the following formula and the OpenAI pricing page~\footnote{OpenAI: \url{https://openai.com/api/pricing/}}:
\begin{align}\label{eq:gpt-3}
\begin{split}
    Cost(GPT3) &= (\#tokens + max\_tokens) \times base\_rate \\
               &= (\#tokens + 100) \times 0.02 \div 1000
\end{split}    
\end{align}
where the base rate for Davinci is \$0.0200 per 1,000 tokens and the \#tokens refers to the number of sub-word tokens by GPT-3 tokenizer (for the entired prompt).
We also use this formula to calculate the required credits for users.

\subsubsection{Auto-completion}
Auto-completion asks a large PLM to continue the story directly, 
meaning that the output is ready to use. 
This is the use case most of the other works used.
\todo[inline]{citation needed}
We use GPT-3 again in this task but no prompt design is involved. 
We simply input the selected story snippet as the prompt and ask GPT-3 to continue the story.
The temperature sampling method is used for decoding, 
where temperature = 0.8, max\_tokens = 100, top\_p = 0.95,
frequency\_penalty = 0.5, and presence\_penalty = 0.5. 
The cost is estimated using \Cref{eq:gpt-3}, where \#tokens calculated for the selected story snippet. 
Note that we also added a five-second delay to this task to make it a fare comparison among AI approaches.

% 5 seconds delay
% GPT-3 
% Decoding method
% Cost












\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/create-task.pdf}
    \caption{Task creation panel. }
    \label{fig:interface-create-task}
\end{figure*}

To create a new task, users need to first select a snippet from the draft and then
click the ``Get Inspired'' button.
\system will generate inspirations based on the selected story snippet.
After clicking the ``Get Inspired'' button, the task creation panel will pop out.
The task creation panel, as shown in \Cref{fig:interface-create-task}, contains a few components:
\begin{itemize}[]
    \item \textbf{Credits}. The user's remaining credit to create tasks. Since the four provided inspiration functions cost differently, we implemented a credit system to balance among them.
    \item \textbf{Content}. The selected story snippet for generating inspirations.
    \item \textbf{Task Type}. \system provides four inspiration functions: (\textit{i}) Crowd Plot Generation, (\textit{ii}) AI plot generation, (\textit{iii}) AI plot generation with guidance, and (\textit{iv}) auto-completion. Users can specify the type of inspiration task here.
    \item \textbf{Task-specific Parameters}. Different inspiration tasks take different parameters. For example, ``Number of Ideas'' and ``Instruction'' are parameters for the crowd plot generation task. 
    \item \textbf{Cost}. The cost of task depends on the task type, the length of the selected story snippet and some of the task-specific parameters. \system computes and reports the cost on-the-fly. Note that when the remaining credit is lower than the cost, users will not be able to create the task.
\end{itemize}

After clicking the ``Create'' button, \system will start working on the inspiration generation task in the backend and display the result when it is ready.
Next, we will describe the four inspiration tasks in detail.
\todo[inline]{Say more about Table 1}

\end{comment}

==> sections/4-1-pilot-study.tex <==
The pilot study was 3-day-long, where the participants were encouraged to write 1,000 words.
The compensation for each participant was a \$100-dollar Amazon gift card.
All other setups of the pilot study were identical to the main study.
%, including the post-study interview.
The pilot study led to final adjustments in \system. %, such as 
%adding undo and redo functions and 
%setting a minimum word count (50 words) for user-selected text to ensure sufficient context is provided. 


%We used the pilot study to spot potential issues in the \system system before the main user study.
%Appendix~\ref{app:pilot-study} lists all the changes we made based on the pilot study.
%We used the pilot study to spot potential issues in the \system system and to finalize our user study 

%--------------- dead kitten ------------

\begin{comment}

protocol. 
Based on the two participants' feedback, we made the some changes to \system 
before the main study:

\begin{itemize}

\item \textbf{Remove the formatting information when copying and pasting texts.}
The participants reported some issues in text formatting when they copied and pasted texts. We learned that these were caused by Quill.js parsing the HTML tag for formatting in an undesired way. We thus configured the editor to automatically remove the formatting information while copying and pasting.

\item \textbf{Add the undo and redo functions.}
As \participant{1} accidentally deleted all her content once in the pilot study, we added an undo and redo function to the editor.



\item \textbf{Set a minimum word count (50 words) for the selected text.}
We noticed that when the user selected a very short text snippet when requesting an inspiration, the AI models sometimes performed poorly, and the crowd would also get frustrated.
So we added a minimum word count (50 words) requirement to the selected text snippet.


\item \textbf{Record more user activities.}
We also improved the event logging components to record more events, \eg, focusing on the Inspiring Panel.


\end{itemize}

    
\end{comment}


==> sections/5-analysis-methods.tex <==
% \cy{P002's nanowrimo logs are not included. We should mention this but where?}
%In this section, we describe how we conducted the writing log analysis, and the qualitative coding and analysis.

\subsection{Analysing Writing Logs}

To perform a comprehensive analysis of writing logs, our approach involved several key steps:
\begin{enumerate*}
    \item \textbf{document reconstruction}, where we implemented a function to reconstruct the state of a document at any specified timestamp, T, based on the writing logs.

    \item \textbf{working session analysis}, where we carried out an analysis to determine appropriate boundaries for working sessions. This enabled us to identify whether a certain period of inactivity meant participants were thinking or leaving.

    % \item \textbf{simulation of normal behavior}, where we simulate ``baseline'' writing behavior that occurs in the working sessions.

    \item \textbf{comparative analysis}, where we compared the baseline behavior-- simulated writing behavior without supports-- with behaviors influenced by four different types of inspiration. This comparison was performed along two dimensions, \textbf{progress} and \textbf{influence level}.
    For progress, we measured the word count produced. For the influence level, we adopted three different methods, including edit-distance, semantic similarity, and paraphrasing detection, as measurements.
\end{enumerate*}
Appendix~\ref{app:writing-log-analysis} discusses each of these steps in detail.
Note that this analysis incorporates writing logs from both the pilot study and the main study, but excludes those from the NaNoWriMo one.

%In the following sections, each of these steps will be discussed in detail.
%\kenneth{I moved the writing log analysis method to Appendix~\ref{app:writing-log-analysis}}

%\input{sections/5-1-writing-analysis-method-details}




\subsection{Qualitative Coding and Analysis}
%\section{Thematic Analysis}
%\kenneth{I moved Sanjana's method section to here.}

The interviews of all the participants were recorded and transcribed by the authors using a mix of automated software and manual checking.
The transcribed interviews and textual data records were analyzed using \textit{analytic induction}, a mixture of deductive and inductive approaches \cite{robinson1951logical,znaniecki1934method}. 
Upon the first round of analysis of the interviews, we identified 287 unique quotes or phrases from the participants. We created a codebook using these unique quotes and then distributed it across 67 excerpts. Upon finalization of the 67 excerpts, they were finally grouped together into nine themes as discussed below. 

==> sections/6-findings-writing-log.tex <==
We analyzed user behavioral and writing logs to answer three research questions (RQs):
{\em (i)} RQ1: What is the usage frequency of each method for generating inspiration?
{\em (ii)} RQ2: How does the inspiration generated by each method affect the number of words produced?
{\em (iii)} RQ3: How does the inspiration from each method influence the content of the writing?
This section outlines the methods and results.



\input{tables/inspiration-stastistic}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\linewidth]{figures/request_trend.png}
    \vspace{-2mm}
    \caption{Usage distribution of four functions across study phases, highlighting a decline in the \crowd function from 28.6\% initially to 11\%-13\% in subsequent phases (RQ1).}
    \label{fig:request-trend}
    \vspace{-2mm}
\end{figure}

\subsection{RQ1: How frequently is each inspiration generation method used?}
\Cref{tab:inspiration-stastistic} shows the usage statistics of our study.
%for all inspiration tasks and the writing tasks.
%\avon{means \#tasks and \#ideas? writing task(x) tasks(o)?}
\participant{5} incorporated their original works into the writing task, resulting in an extensive final draft of 10,287 words.
In contrast, \participant{15} produced three shorter drafts, with word counts of 1,198, 1,288, and 272, respectively.
Since the NaNoWriMo study did not require the participant to write within the \system's editor, we excluded the word counts for \participant{2}$_{na}$.

\paragraph{GPT3-Continuation was the most popular, while Crowd usage declined after the initial phase.}
\Cref{tab:inspiration-stastistic} shows that
the \gptc function was the most popular, with 74 tasks created and 95 inspirations generated. 
Six participants used \gptc most frequently. 
Meanwhile, \plot was the second most popular option, primarily used by two participants (\participant{4} and \participant{2}$_{na}$).
%\paragraph{Participants reduced their use of the \crowd option after the initial phase.}
% \kenneth{TODO HCOMP: Name the two participants.}
We further analyzed the percentage of each function's use within the first, second, third, and last 25\% of participants' requests to \system.
Figure~\ref{fig:request-trend} shows that participants reduced their use of the \crowd option after the initial phase of the study. 
Initially, the crowd function accounted for 28.6\% of requests, but this dropped to 11\%-13\% in subsequent quarters.
% \kenneth{TODO HCOMP: I added this. Please check.}








\input{tables/latency-table}



%\paragraph{Latency of Each Function.}
\paragraph{\crowd had a much longer system and reading latency, with one-third of responses going unread.}
From interviews with participants, we learned that latency significantly influences their choices. 
To analyze this, we calculated two types of latency for each function in \system: {\em (i)} system latency and {\em (ii)} reading latency. 
System latency is the time from when a user creates a request to when the system first responds. %(either from AI or Crowd). 
Reading latency measures the time from receiving the first response to when the user reads it. 
Table~\ref{tab:latency-distribution} shows the results.
Most AI functions deliver responses within 10 seconds; users typically read these inspirations immediately. 
In contrast, the \crowd function can take up to an hour for an initial response, and users often delay reading these for several hours. 
%This latency pattern, also noted in prior studies of crowd ideation~\cite{heteroglossia-huang-2020}, likely increases the chances that users will skip reading crowd-generated inspirations. 
Moreover,
%Table~\ref{tab:latency-distribution} also shows that 
participants did not read 36.67\% of the inspirations produced by the \crowd function.
% \kenneth{TODO HCOMP: I rewrite this part. Please check.}




\subsection{RQ2: How does each method of inspiration affect word count?}
%To perform a comprehensive analysis of writing logs, our approach involved several key steps:
To perform a comprehensive analysis of writing logs, we pre-processed the data with the following steps:
\input{sections/5-1-writing-analysis-method-details}





\subsection{RQ3: How does each inspiration method influence writing content?}
RQ3 evaluates how much the inspirations influenced the content of participants' writing.
We compared sentences in the inspirations to the ``newly-edited content'' in the drafts. 
``Newly-edited content'' includes {\em (i)} sentences that were not in the draft when the inspiration was accessed but appeared five minutes later, and  {\em (ii)} sentences that were edited within these five minutes.
For each inspiration-reading event (see RQ2), we first calculated sentence-level similarities pairwisely.
For example, with a 3-sentence inspiration and a draft having 5-sentence newly-edited content, we calculated 15 ($3\times5$) similarities. 
Following prior work~\cite{roemmele2021inspiration}, we then took the highest value among the 15 as the final similarity score.
%Following prior work~\cite{roemmele2021inspiration}, we chose the highest score, considering that even one closely matching sentence in the newly edited content indicates a strong influence from the inspiration.
We chose the highest score because if even one sentence in the newly edited content closely matches a sentence in the inspiration, we consider the inspiration to have had a strong impact on the writing.
%Focusing on sentence-level similarity strikes a balance between granularity and noise: full paragraphs are rarely copied, while individual words would be too noisy.
%\kenneth{Can we cite something here to justify some of these decisions?}
%\paragraph{Three Text Similarity Metrics.}
We used three sentence-level similarity metrics for this comparison:

\begin{itemize}


\item \textbf{Normalized Edit Similarity:}
% We first calculated the normalized edit distance~\cite{4160958,python-string-similarity}
% \footnote{\url{https://github.com/luozhouyang/python-string-similarity\#normalized-levenshtein}}.
We used $1 - Normalized Edit Distance$~\cite{4160958,python-string-similarity}, meaning higher scores indicate higher similarity.
%This metric identifies instances where users have copied text verbatim from the inspiration.

\item \textbf{Semantic Similarity:}
We calculated the cosine similarity on semantic representations obtained from Sentence BERT~\cite{reimers-2019-sentence-bert}.
%(\texttt{sentence-t5-base})
% We turned sentences into semantic representations using Sentence BERT (\texttt{sentence-t5-base})~\cite{reimers-2019-sentence-bert}
% \footnote{\texttt{sentence-transformers/sentence-t5-base}}
% and calculated cosine similarity as the metric.
%This metric aims to capture instances where users have been inspired by the content but have formed their own sentences.
%This metric captures instances where users were inspired by the content but formed their own sentences.

\item \textbf{Paraphrasing Detection Score:}
A paraphrasing detection model~\cite{nighojkar-licato-2021-improving} was used to classify whether a written sentence is a paraphrase of a sentence in the inspiration.
The output probability was treated as the similarity score.
%This metric captures instances where users paraphrased the inspiration.
%Because this model is a classifier, it is the strictest one of our three metrics.
%We include it to provide a different dimension to our measurements.

\end{itemize}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/similarity-240sec-5min-edit-distance-best-random.png}
    \includegraphics[width=0.7\linewidth]{figures/similarity-240sec-5min-sentence-embedding-best-random.png}
    \includegraphics[width=\linewidth]{figures/similarity-240sec-5min-paraphrasing-best-random.png}
    \vspace{-2mm}
    \caption{Distribution of the similarity metrics (RQ3). A 1.0 similarity means that the whole sentence is adopted. Overall, \gptc has a higher rate of being adopted.}
    \label{fig:similarity-behavior}
    \vspace{-2mm}
\end{figure}


%\paragraph{Comparing with a Simulated Baseline.}
We simulated a baseline condition by comparing a random working draft and a random inspiration. 
We randomly selected a time from a working session and observed changes in the document five minutes later.
%\kenneth{Does this also done 1000 times like in RQ2?}\cy{Yes. Added this to the following draft.}
We also randomly sampled one inspiration from the same document and then applied the three similarity metrics to these sentences. 
The simulation was run 1,000 times.
%Note that the similarity between two random text pieces from the same document will not be zero due to potential general overlap.
Finally, similar to RD2, we used KDE plots to visualize the distribution of these influence levels across the four inspiration methods and the baseline condition.
Figure~\ref{fig:similarity-behavior} shows the results, in which
%In Figure~\ref{fig:similarity-behavior}, 
a 1.0 similarity indicates complete integration of the ``inspiration sentence'' into the user's draft, while a 0.0 similarity means no integration occurred.
In each chart of Figure~\ref{fig:similarity-behavior}, the prominent peak in the Baseline curve represents cases where users did not adopt any parts of the generated inspiration.
%These Baseline's peaks were not always near 0.0 because both the inspiration and the user's writing came from the same document, leading to some inherent conceptual overlap.

\paragraph{\gptc influenced the written content the most, with full-sentence adoption across all methods.}
Across all three charts in Figure~\ref{fig:similarity-behavior}, \gptc's curves are notably flatter and skewed to the right, indicating a higher likelihood of users producing texts similar to those generated by \gptc.
Additionally, at the high-similarity end (close to 1.0), \gptc exhibits a greater probability density compared to other options. 
This indicates a higher tendency for \gptc sentences to be directly copied into participants' drafts. 
Overall, \gptc influences the participants' writing the most.
Note that, at the high-similarity ends, all options exhibit a probability density greater than zero, indicating that full-sentence adoption occurs across all inspiration generation methods in \system.
%Some inspiration sentences still made their way into the draft.
%Meanwhile, \plot's curve aligns closely with the Baseline, suggesting that within a five-minute window, it may have the least impact on the written content.









%------------------- dead kitten -----------------

\begin{comment}







Across all three charts in Figure~\ref{fig:similarity-behavior}, \gptc's distribution curves are the flattest and also skewed to the right, suggesting it has a higher probability of having users produce texts similar to its generation.
Furthermore, on the right end of all three charts in Figure~\ref{fig:similarity-behavior}, i.e., when similarity is close to 1.0, \gptc has a higher probability density than all other options.
This means sentences in \gptc's inspiration also had a higher chance to be completely copied and pasted into participants' drafts.
These, collectively, suggest \gptc shows the strongest influence on participants' writing content. 

In Figure~\ref{fig:similarity-behavior}, \gptc shows the strongest influence on participants' writing content. as evidenced by its highest values at a similarity of 1.0 (the right end of Figure~\ref{fig:similarity-behavior}), indicating complete incorporation, across all three metrics compared to other options and the baseline.
Additionally, \gptc's distribution curves are the flattest and skewed to the right in all metrics, further supporting its significant impact.





















%Pure zero values are uncommon.



\bigskip


%RQ3 evaluates how much the inspirations influenced the content of participants' writing.
We compared sentences in the inspirations to the newly edited or added sentences in the drafts. 



%``Newly edited content'' is defined as sentences that were not in the draft when the inspiration was accessed but appeared five minutes later (\ie, Document$_{T+5}$ - Document$_{T}$).





\kenneth{-----------------KENNETH IS WORKING HERE----------}




%\paragraph{Assessing the Level of Influence}
We aim to evaluate how much the inspirations actually influenced the writing generated by participants.
To achieve this, we compare the sentences in the inspirations to the newly edited or added sentences in the document pair-wisely.
Specifically, we define ``newly edited content'' as sentences that were not in the document at the time of accessing the inspiration but appeared in the version five minutes later (\ie, Document$_{T+5}$ - Document$_{T}$).
%
To make this comparison, we use three different types of similarity metrics:



%
For each inspiration-reading event, we calculate the similarities on the sentence level pair-wisely\footnote{For example, with a 3-sentence inspiration and a document with 5-sentence modification, we would get 15 similarities.} and then take the highest value among them.
We chose the highest score because if even one sentence in the new edit is closely related to the inspiration,
we consider the inspiration to be effective. \avon{I can't understand, the highest score among what? The three similarity methods? If yes, how do you align their scores? I assume the similarity scores of different methods represent different things and are not comparable.}
We focus on sentence-level similarity, as it strikes a balance between granularity and noise:
full paragraphs are rarely copied, while individual words would be too noisy.

For better comparison, we also simulate a baseline condition
by comparing the similarity between a random working draft and a random inspiration.
Namely, we randomly select a time from a previously identified working session
and then observe what changes occur in the document five minutes later.
One inspiration from the same document is also sampled randomly.
We apply the three similarity metrics to these sentences, aiming to capture the influence level in a scenario where inspiration is not helpful\footnote{Note that the similarity between two random pieces of text from the same documents will not be simply zero as there might still be some general overlap}.
\avon{Can't understand this part.}
%
Finally, we use Kernel Density Estimation (KDE) plots to visualize the distribution of these influence levels across the four inspiration methods and the baseline condition.
Again, the common-norm is set to false so that we can focus on the distribution itself.


\kenneth{------------------ KENNETH IS WORKING HERE--------------------------}
\bigskip



\subsection{Analysis Methods}
%To perform a comprehensive analysis of writing logs, our approach involved several key steps:


\subsection{Basic Statistics and Use Frequency}

\Cref{tab:inspiration-stastistic} shows statistics for all inspiration tasks and the writing tasks.\avon{means \#tasks and \#ideas? writing task(x) tasks(o)?}
\participant{5} incorporated her original works into the writing task, resulting in an extensive final draft of 10,287 words.
In contrast, \participant{15} produced three shorter drafts, with word counts of 1,198, 1,288, and 272, respectively.
Since the NaNoWriMo study did not require the participant to write within the \system's editor, we excluded the word counts for \participant{2}$_{na}$.
Notably, the Auto-Completion function was the most popular, with 74 tasks created and 95 inspirations retrieved.
%
\Cref{tab:latency-distribution} shows the distribution of the time-related statistics. \avon{What are samples? Why don't you use all ideas? Better to say it's the unit is second.}
As illustrated, most AI functions deliver a response in under 10 seconds, and users typically engage with these inspirations soon after.
In contrast, the Crowd Plot function might require up to an hour for an initial response.
Furthermore, users often defer reading these inspirations, waiting several hours -- a pattern consistent with findings by \citeauthor{heteroglossia-huang-2020} in their study on crowd ideation functions~\cite{heteroglossia-huang-2020}.
Such delays naturally lead to a higher probability of users skipping the reading of crowd plot inspirations.
%In the following section, 
%Appendix describe how we analyze the writing logs in detail.

% \kenneth{We can probably say more about frequency, especially when writing logs didn't give us anything...}

% \kenneth{ALSO if we want to mention writing logs, we can add a few words to say other people didn't mention it hehe.}

% \cy{I also include the latency table. We need to describe it here.}



%TC:ignore
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.80\linewidth]{figures/writing-behavior-240sec-3min-all.png}
%     \caption{Distribution of the Writing Progress with 3-minute writing. The Crowd Plot's small peak at 70 words in \Cref{fig:progress-distribution} reduces and shifts left, indicating that users might need time to catch up with the prior information.\kenneth{TODO HCOMP: Maybe merge Fig 4 and 5 into one figure. Make it take less space.}}
%     \label{fig:progress-distribution-3-min}
% \end{figure*}
%TC:endignore

\subsection{What can we learn from observing each participant's accumulated word counts?}

\subsection{How did the generated texts influence users' writing?}
\label{subsec:similarity-analysis}
%TC:ignore

%TC:endignore

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/similarity-240sec-5min-edit-distance-best-inspiration-random.png}
%     \includegraphics[width=0.8\linewidth]{figures/similarity-240sec-5min-sentence-embedding-best-inspiration-random.png}
%     \includegraphics[width=0.8\linewidth]{figures/similarity-240sec-5min-paraphrasing-best-inspiration-random.png}
%     \caption{Distribution of the three similarity metrics. Aggregated by taking the max value per inspiration sentences.}
%     \label{fig:similarity-behavior}
% \end{figure}

\Cref{fig:similarity-behavior} displays the distribution of how generated texts impacted users' writing,
measured using metrics, edit similarity, semantic similarity, and paraphrasing probability.
A 1.0 similarity suggests the entire ``inspiration sentence''
from the generated text was integrated into the user's draft.
Conversely, a 0.0 similarity indicates none of the inspiration was integrated.
These pure zero values are rare.
The prominent peak in the Baseline likely represents cases
where users did not adopt any of the generated suggestions.
The peak is not located at 0.0 because both the suggestion and the user's writing are from the same document and a certain level of overlap is expected.
Values that fall between the baseline peak and 1.0 indicate various degrees of influence from the generated text.
%
Here are the key observations:

\paragraph{Auto-Completion influenced writing the most.}
Auto-Completion consistently shows the highest frequency of users adopting entire sentences,
evidenced across all three metrics.
The distribution also skews to the right, indicating that, apart from high full-sentence adoption rates, it also has a higher rate of mirroring or impacting user writing.

\paragraph{Each of the four functions was utilized at some point.}
Observing the 1.0 similarity side, AI Plot with Guidance follows Auto-Completion
in terms of full-sentence adoption rates.
AI Plot and Crowd Plot, while having lower rates, are not zero,
which suggests that on rare occasions, some inspiration sentences still made their way into the draft.
For context, the Baseline has almost no density at a 1.0 similarity score.

\paragraph{AI Plot may lack efficacy.}
The distribution for the AI Plot aligns closely with the Baseline,
hinting that within a five-minute window, it might not effectively guide users.

\paragraph{Crowd Plot often demands modification before use.}
The distribution for Crowd Plot presents an interesting pattern
with a slight peak to the right in both edit and semantic similarity metrics
(recorded at 0.70 and 0.86, respectively).
This suggests that users while incorporating Crowd Plot's suggestions,
frequently modify them to match their narrative or
only select certain portions of the inspiration.

% \cy{The difference of All is very little. Is there another aggregation method?}
% \cy{How about selecting the best for every inspiration sentence?}
%
\Cref{tab:latency-distribution} shows the distribution of the time-related statistics. \avon{What are samples? Why don't you use all ideas? Better to say it's the unit is second.}
As illustrated, most AI functions deliver a response in under 10 seconds, and users typically engage with these inspirations soon after.
In contrast, the Crowd Plot function might require up to an hour for an initial response.
Furthermore, users often defer reading these inspirations, waiting several hours -- a pattern consistent with findings by \citeauthor{heteroglossia-huang-2020} in their study on crowd ideation functions~\cite{heteroglossia-huang-2020}.
Such delays naturally lead to a higher probability of users skipping the reading of crowd plot inspirations.
%In the following section, 
%Appendix describe how we analyze the writing logs in detail.

% \kenneth{We can probably say more about frequency, especially when writing logs didn't give us anything...}

% \kenneth{ALSO if we want to mention writing logs, we can add a few words to say other people didn't mention it hehe.}

% \cy{I also include the latency table. We need to describe it here.}
    
\end{comment}



==> sections/7-findings-qualitative.tex <==
%%% Remove most of the quotes and keep only essentials%%%%


%The interviews of all the participants were recorded and transcribed by the authors using a mix of automated software and manual checking. 
The transcribed interviews %and textual data records 
were analyzed using analytic induction, a mixture of deductive and inductive approaches~\cite{robinson1951logical,znaniecki1934method}.
Upon the first round of analysis of the interviews, we identified 287 unique quotes or phrases from the participants. 
We created a codebook using these unique quotes and then distributed it across 67 excerpts.
Upon finalization of the 67 excerpts, 
they were finally grouped together into themes as discussed below. 


\subsection{Thoughts on Writing with Crowd Workers} 

\paragraph{Charm of Human Input.}
Participants recognized the value of \crowd inputs despite their infrequent use, expressing appreciation for the human touch and originality these responses provided over AI-generated text. 
Feedback highlighted the personal touch and shared understanding humans brought to the writing, with participants particularly impressed by the ability to ask directed questions and explore different writing alternatives. 
%For example:
%This sentiment is best described by participants' accounts:
%\myquote{\participant{14}}{Everything was barely off topic. There wasn't anything that seemed really off-topic from what I was writing. \textbf{And it made sense, like it made logical sense any of the ideas or the continued story that was given. I think it was the most helpful overall.}}
%\myquote{\participant{4}}{...they always came through with some \textbf{interesting directions} and it felt like \textbf{being in a writer's workshop}, but it did take longer.}
Additionally, there was curiosity about the demographics of the human responders, and while preferences varied, there was a consensus on the need for a more defined audience.



%We observed the participants saw the potential value of the \crowd inputs.
%There was positive and constructive feedback that surrounded the feature where the participant could use the system to ask questions to the MTurkers about the writing and the directions it can take.

%We found that participants preferred the \textbf{human touch} over the text generated by AI. The \textit{perceived} originality of human responses was often preferred over AI. This can be seen more as a personal touch that humans brought to the writing as well as the shared understanding of the writing really impressed the participants. They liked that they could ask more directed questions and explore different alternatives for their writing. 


%Furthermore, we saw that the participants were curious about the demographics of the \textit{human responder} (MTurker). Though the participants differed in their preferences for the \textit{optimal} background (of the MTurker), there was consensus around a need for a more defined audience. 


\paragraph{Pitfalls with the \crowd Feature.}
Participants valued the human touch in the \crowd feature but faced significant issues with \textbf{inconsistent and delayed responses}.
%, contrasting with the near-instantaneous replies from AI. 
They suggested recruiting responders across diverse time zones to ensure continuous availability and improve timeliness.
Additionally, \crowd sometimes produced incoherent responses due to unclear instructions. 
Participants recommended filtering mechanisms to verify the qualifications of human assistants, who should ideally be writers or avid readers with the option to choose their preferred type of writing. 
%This could enhance their engagement and improve the quality of responses. 
%Cost was also a concern; participants indicated that the affordability of the feature could influence their decision to continue using it.\kenneth{We should probably mention the cost/credit part somewhere hmmm}




%Participants appreciated the human touch but encountered obstacles in effectively using the feature.
%The main issue was inconsistent and delayed responses. Comparing this with the near-instantaneous AI responses, the delay was a significant drawback.
%Participants preferred more timely responses and suggested recruiting responders from diverse time zones to ensure round-the-clock availability. 


%MTurkers sometimes struggled with instructions, resulting in incoherent responses. Participants feedback was helpful in addressing these pitfalls. Recommendations included implementing filtering mechanisms to determine the qualification of human assistants. Preferably, assistants should be writers or enthusiastic readers, able to select the type of writing they want to assist with, ensuring their interest and improving response quality. Lastly, an additional consideration is the cost for human feedback. Some participants felt their decision for the continued use of the function would depend on the upkeep cost that it would incur. 

 %%\textit{\say{No I didn't like it at all because it is time-consuming and still, the response that the human brings is not according to what you are trying to write.} - \participant{10}} \textit{\say{The points that it costs would maybe lead me to not use it because of the time and the points} - \participant{4}}

\subsection{Comparing the Different AI Features}

\subsubsection{\plot.}
\plot generated significant interest, with participants generally preferring the near future option because it better maintained the flow of their writing without introducing unwanted elements like new characters.
%For example, \participant{4} mentioned:
%\textit{\say{There was like a higher quality of ideas coming from the near future one just because it had more logic or it made more sense than sometimes the far ones.} - \participant{4}}
However, %under specific conditions, 
a few participants found the far future function more useful, particularly when they wanted to advance the story or gain an overview of their world.
%\textit{\say{I stopped using the near after a couple of days because I wasn’t getting anything helpful from it. So after I learned that the distant was usually more helpful for me. The distant future one was less random. And usually incorporated more of my story into it.} - \participant{14}}
Participants also often explored and compared both the near and far future functions. 
Some used them as a way to bounce ideas off another mind.

%\textit{\say{Sometimes I chose both [far and near future options] because I just kind of wanted to see the ideas. ... 
%but, I know 
%If it's something as simple as ``how's he going to react to this'', that's near future. 
%If I wanted to know ``what do you [system] think his reaction should be?'', it would be for the far future, ...} - \participant{5}}








%AI plot generation produces potential story developments based on the selected story snippet. This feature garnered significant interest, with participants showing varied preferences between the near and far future options.
%However, 
%Our impression is that there was a slight inclination toward the near future feature. Participants believed it better captured the flow of their writing, whereas the far future functionality sometimes introduced unwanted elements, such as new characters. 
%\textit{\say{There was like a higher quality of ideas coming from the near future one just because it had, like, it had more logic or it like made more sense than sometimes the far ones.} - \participant{4}}

%Under contrasting conditions, we saw that for some participants the distant future prediction function worked better. It helped them in scenarios where they wanted to take the story forward or wanted to an overview of situating their world. 
%\textit{\say{I stopped using the near after a couple of days because I wasn’t getting anything helpful from it. So after I learned that the distant was usually more helpful for me. The distant future one was less random. And usually incorporated more of my story into it.} - \participant{14}}

%As with other participants, they explored both functions and compared the results of near and future predictions. Interestingly, they approached it with a perspective of bouncing ideas off like another mind. 





\subsubsection{\gptplot.}
Participants had mixed feelings about using \gptplot. 
Some used it to validate their storylines, while others explored alternative perspectives. 
They appreciated \gptplot's quick response time %, particularly in comparison to the \crowd feature, 
and its utility in mapping out structural outlines. 
\gptplot also helped them overcome writer's block by allowing repetitive actions until the desired response was achieved. 
However, there were challenges. 
\gptplot sometimes 
did not consistently provide plot predictions aligned with authors' expectations.
It also fell short in offering refined guidance in specific scenarios.
%did not align with authors' expectations for plot predictions and sometimes lacked refined guidance in specific scenarios. 

%\textit{\say{I use the plot [\gptplot] next, the second plot idea as it worked a lot when you plot something and it doesn't appeal to you and generate another plot, it gives you a good plot that you can definitely put it.} - \participant{10}}


%There were mixed feelings about the use of \gptplot.
%Some participants used it for validation of their story-line while others to explore alternative perspectives.
%The participants felt that the function was useful in mapping the outline structures. %\textit{\say{So the function was helpful for figuring out how to map out a plot. I didn't really start with a plot in mind when I was writing this story.} - \participant{4}}
%\cy{\participant{4} is a discovery writers. We can probably mention this?}



%Upon closer examination of this function, we noted participant complaints about the system. The primary challenge was that the feature did not consistently provide plot predictions aligned with authors' expectations.
%While helpful in overcoming writer's block, the feature often fell short in offering refined guidance in specific scenarios. %\textit{\say{I use the plot next, the second plot idea as it worked a lot when you plot something and it doesn't appeal to you and generate another plot, it gives you a good plot that you can definitely put it.} - \participant{10}}


%Participants valued the quick response time of this feature, especially when compared to the MTurk feature.
%It allowed them to repeat actions until they achieved the desired response.
%They frequently incorporated specific elements into their own work, as evidenced in 
% \Cref{subsec:similarity-analysis}
%RQ3 and \Cref{fig:similarity-behavior}, where AI Plot with Guidance was the second most adopted option. %\textit{\say{There was sometimes pieces of information that I could pull from it. It was also a little bit more points, but not necessarily a lot. So a lot of times, I would just sit there and I'll just be like, get another plot, get another plot.} - \participant{15}}



\subsubsection{\gptc.}
In the interview, 
\textbf{all the participants unanimously preferred \gptc}.
%Highlighting the common sentiment, participants said:
%\textit{\say{\textbf{I liked the auto-complete (\gptc) function the most} because it was \textbf{instant gratification}.} - \participant{2}}
%\textit{\say{... (\gptc) was a function that you can select a paragraph that you want it to be completed. \textbf{And actually it worked and worked very perfectly.}} - \participant{10}}
In some instances, 
\gptc sparked fresh ideas and alleviated writer's block by proposing alternative story leads. 
Interestingly, some participants found \system's unintentional feature of leaving sentences unfinished---due to a 100-word constraint on GPT-3 that we implemented---encouraging them to think more creatively.
However, \gptc sometimes disrupted their natural workflow, as they felt compelled to edit the AI-generated text, leading to interruptions in their thought process.
%Despite these interruptions, many users still preferred \gptc over \crowd for its immediate results. 
%Yet, some participants reported that the auto-completion feature occasionally caused them to lose their train of thought, leading them to favor maintaining their own line of thinking and opting out of using this feature.




%as indicated by its higher request rate (\Cref{tab:inspiration-stastistic}) and adoption rate (\Cref{fig:similarity-behavior}). 
%In some instances, \gptc sparked fresh ideas and alleviated writer's block.
%Regarding generating new ideas, a participant suggested \gptc sometimes proposed alternative leads for completion. 
%\kenneth{TODO CY: I didn't see any quotes about idea dump...? So I removed the description.}
%\kenneth{TODO CY: I modified this to make it more clear. Take a look.}
%Some participants found it intriguing when the system intentionally left sentences unfinished, encouraging authors to think creatively.\footnote{This ``feature'' is not intentional; however, we implemented a 100-word constraint for GPT-3 to motivate users to engage in more extensive writing.} In comparison to the human feature, users favored the auto-complete for its immediate results. 

%within a 100-word constraint set for GPT-3. 

%\textit{{I liked the auto-complete function the most because it was instant gratification.} - \participant{2}}

%In terms of how it fits in their process, some participants felt that because they felt like they had to go in and edit the AI-generated text, it interrupted their natural flow of work.
%In line with interruptions, some participants had strong feelings about how they prefer sticking to their chain of thought and would, therefore, not use this feature. 
%In some cases, with the auto-complete, the participants lost their chain of thought.

\subsection{Challenges in Interacting with \system}

\paragraph{Steep Learning Curve.}
Participants highlighted the need for better training on formulating prompts. 
They suggested providing clear guidance on selecting an optimal text, offering detailed instructions for human assistants, and explaining the differences between AI features. 
Some noted that the initial learning curve impacted their early use of \system and could influence their overall experience.

%\subsection{The Challenges with Learning Curve}

%Many participants expressed a need for improved training in formulating instructional prompts.
%Suggestions included providing guidance on optimal text selection, detailed instructions for humans, and distinctions between AI features.
%Some participants noted a learning curve impact on their initial use of the tool, potentially influencing their overall experience. 

%\myquote{\participant{10}}{I didn't understand what the features were actually and I just wrote the story first thinking about the story alone. And then all of a sudden I got interested in these features. I was willing and I was very interested with these features, and I tried the first the human, but the human didn't respond.} 

%\cy{I guess this can also link to some issues related to voice assistants - people don't really know what they can do with the model as the input is ``natural language'' and there is no clear ``boundary'' for this. And the trust can not really be built when the system ``sometime'' fail you (which is very hard to predict).}
%\cy{Do we have papers relevant to this but on chatgpt?}
%\cy{One possible solution is to allow people to share their ``prompt'' with others.} \sanjana{Maybe we can add that in the discussion}

\paragraph{Lost Context while Interacting with AI.}
Participants noted that \plot and \gptplot sometimes produced irrelevant inspirations due to a poor grasp of context. 
They also noted that the AI struggled with complex prompts and failed to comprehend detailed instructions. 
This limitation left those seeking interactive AI experiences, including the ability to ask follow-up questions and receive meaningful responses, dissatisfied. 
Additionally, there were instances where the AI inaccurately captured the genre.
%of the participants' work.









%Participants raised concerns about losing context with \plot and \gptplot, resulting in AI-generated inspiration that sometimes seemed irrelevant due to poor contextual understanding. 
%They also noted that the AI struggled with complex prompts and failed to comprehend detailed instructions. 
%This limitation left those seeking interactive AI experiences, including the ability to ask follow-up questions and receive meaningful responses, dissatisfied. 
%Furthermore, there were instances where the AI did not accurately capture the genre of the participants' work.




%\subsection{Lost Context while Using the Different Features}
%Finally, we saw that participants highlighted concerns about lost context when using plot prediction and future prediction functions.
%This resulted in issues where AI-produced results became irrelevant due to the lack of contextual understanding. 
%Another problem was the AI's limited response to complex prompts, leading participants to believe it struggled to comprehend instructions.
%Participants seeking more interaction with AI, including the ability to ask questions and receive meaningful responses, were left unsatisfied.
%Additionally, there were instances where the AI's writing failed to capture the genre of the participants' work.
%\kenneth{This doesn't even mention MTurk I think? Maybe just remove MTurk.}


%One of the most important concerns that came from the participants was the lost context while using plot prediction as well as future prediction functions. This created multiple issues where the results produced by AI were useless considering they lost the context of the work and story. Another issue was that AI did not respond well to complex prompts. In some cases, the impression the participant had was that AI did not understand the instructions well. The participants when they tried more complex queries did not get satisfactory results. They also expected more interaction with AI, where they can ask questions and respond and expect responses back. In some cases, they felt that AI writing did not capture the genre of their writing. 
%\cy{This one also related to the previous one. I guess there would be questions like, how about chatGPT, which is more powerful in following the instruction.}

%\myquote{\participant{1}}{I say it could be very wild because I don't know who this Jumbie is.}
% \textit{\say{But so, yeah, cause I say it could be very wild because I don't know who this Jumbie is. But like the other, for my own story, I actually think that AI works better on my own story than on the [inaudible one that's something we can talk about later. Let me see the completion. Yes. This part, this one is where I feel like it's. Oh, I see. Okay.} - P001}

%\myquote{\participant{4}}{I would only do a small chunk to see what it would give. But when I did a small chunk, I had a main character who was not a human, the main character was a chicken and the machine would just like always turn her back into a human. So, I would have to go through, like, if I did use it in the writing.}
% \textit{\say{I would only, you know, do a small chunk to see what it would give. But when I did a small chunk, I had a main character who was not a human, the main character was a chicken and the machine would just like always turn her back into a human. So, I would have to go through like, if I did use it in the writing,} - P004}


%\kenneth{I moved the qualitative results to here.}
%In this section, we present the findings we observed from our qualitative analysis.
%Additionally, participants also make some design recommendations for \system, which we list in Appendix~\ref{app:qual-additional-feature}.

%\section{Qualitative Results}

%\subsection{Author Processes}

%Each participant had a different process for writing as well as challenges they face while writing. As this tool is designed to support writers in their writing, we work towards understanding their process and how we fit in it. From the varied perspectives of the participants, some come up with a plot idea first and then develop the characters, while others are inspired by paintings. 

%\textit{\say{I would think is, probably how to keep the story going and keeping the conflict there without having it become too much and too dramatic.} - P005}

%While they struggle with different things during the writing process, there are different ways they manage them. For some, the deadline pressure helps while others find strolls as means of new inspiration when they are stuck.

%Through all this they do turn to technology at times for support. It may be in the form of grammar check, spell check, productivity support and fact checking through simple Google searches. 

%\textit{\say{Like, I'll come up with a plot idea and then some of the characters and I'll kind of like work through the plot a bit, like in my head. And then I'll like, go work through the characters a bit sort of like, what are their personalities? - P015}}

%As discussed in the previous section, we provided the participants with features like crowd plot generation that allows the user to create human intelligence tasks (HITs) on Amazon Mechanical Turk (MTurk) to ask crowd workers to provide plot ideas to continue the selected story snippet. The users can specify how many story ideas they want to obtain and also write instructions to guide workers. The instructions to crowd workers could be descriptions of particular characters in the story,

%\myquote{\participant{14}}{Everything was barely off topic. There wasn't anything that seemed really off-topic from what I was writing. And it made sense, like it made logical sense any of the ideas or the continued story that was given. I think it was the most helpful overall.}

%\myquote{\participant{5}}{I love, I love the idea of it. I love that you can go and there's going to be someone there that kind of talks it out with you.}

% \textit{\say{Everything was barely off topic. There wasn't anything that seemed really off topic from what I was writing. And it made sense, like it made logical sense any of the ideas or the continued story that was given. I think it was the most helpful overall.} - P014}

% \textit{\say{I love, I love the idea of it. I love that you can go and there's going to be someone there that kind of talks it out with you.} - P005}
% %\textit{\say{Not, not a lot. I think usually I prefer other people.} - P014}

% \textit{\say{I'm not sure who was giving the ideas, but they always, you know, came through with some interesting directions and it felt like being in a writer's workshop, but it did take longer.} - P004}

%\textit{\say{I would highlight from text and then ask a person either some questions about it or how to keep going with it, or any ideas branching off the text that was highlighted.} - P014}
%how they used the feature??

%The participants used the feature to study other people's perspectives on it, or if they expanded a concept into a paragraph, or any new ideas branching off what they had already written. 
%In a comparison with AI, we saw that a participant was of the opinion that asking MTurkers ensures they use their \textbf{own words}, rather than referring to other sources. 

%Interesting to see assumptions about AI play a role in how MTurk work is perceived
%\myquote{\participant{14}}{As sometimes I needed to see how, what I'd written had come across before I moved on to the next part, and I was able to get a response back from an actual person. Like an actual reader, essentially to see if what I was saying made sense to them or what they were thinking was happening.}
% \textit{\say{As sometimes I needed to see how, what I'd written had come across before I moved on to the next part, and I was able to get a response back from an actual person. Like an actual reader, essentially to see if what I was saying made sense to them or what they were thinking was happening.} - P014}

%\myquote{\participant{10}}{They can quote books, but they can virtually use their own words, not like AI can just refer and take maybe some words that are at the same, as the one, the referred book.}
% \textit{\say{They can quote books, but they can virtually use their own words, not like AI can just refer and take maybe some words that are at the same, as the one, the referred book.} - P010}

%Although the participants loved the human touch, there were a lot of deterrents when it came to successfully using the feature. Firstly, the responses were not always on time and varied delays in the responses (see latency distribution in \Cref{tab:latency-distribution}). One of the most notable considerations was the comparison with AI responses when it came to the timing of it. AI responses were almost immediate and it was seen as the biggest deterrent in using this function. The participants felt if the responders were more timely in their responses they would reach out to them more often. One of the recommendations was to recruit people across time zones so that there are responses round the clock. 

%\myquote{\participant{2}}{I highlighted sections and I clicked to ask a human, but I checked back the next day I still hadn't gotten a human to respond to that prompt}
% \textit{\say{Well, I highlighted sections and I clicked to ask a human, but I checked back the next day I still hadn't gotten a human to respond to that prompt} - P002}

% \textit{\say{I think the timeframe was just some like, it's hard to not compare it to the other ones, the other ones were just so much faster. And so that was like the big drawback.} - P004}

%At times it felt like the MTurkers were not reading the instructions well and so the responses were not making a lot of sense. We received a lot of feedback from the participants when it came to improving the pitfalls of this function. There were recommendations about how there should be filtering mechanisms about \textit{"who"} are the humans that help with the process. They should either be writers or enthusiastic readers. They should be allowed to pick and choose what kind of writing they want to assist with to ensure their interest when it comes to responses.

% \textit{\say{So in my use of the ask human function, it was awesome to get ideas from people. there was definitely a difference when the person understood the assignment it was more personal and it was more, you knew that they were kind of going, that they understood what you were asking and you could trust them more if that made sense} - P005}

% \textit{\say{No I didn't like it at all because it is time consuming and still, the response that the human brings is not according to what you are trying to write.} - P010}

 
%Some people expected more conversational interaction with humans so consistency with the same human would have been helpful. 

% \textit{\say{And one thing that I noticed was like the points that it costs or whatever were different that like the thing that would maybe lead me to not use it because the time and the points} - P004}

%There were three different AI features that the system came with:
%(\textit{i}) AI Plot Generation: AI forecasting what might happen in the next 20 or 100 sentences,
%(\textit{ii}) AI Plot Generation with Guidance: GPT-3 producing a follow-up story arc,
%and (\textit{iii}) Auto-Completion: GPT-3 continuing the Story. 

%AI plot generation produces a few sentences that describe what could happen next in the story given the selected story snippet. This feature received a lot of interest from the participants and there was little consensus on which of the two options (near or far) they preferred. 
%However, there was a slight inclination towards the near future feature over the far future functionality. The participants felt that the near future prediction captured the flow of their writing better, while the far future drifted in other directions.
%In some cases, it would even end up producing new characters that the authors did not want to see. 

%\myquote{\participant{10}}{I hate the far future when you have quoted some maybe few paragraphs and it produces out-of-topic future paragraph, which doesn't even connect with the paragraph that you have written.}
% \textit{\say{I hate the far future when you have quoted some maybe few paragraphs and it produces out of topic future paragraph, which doesn't even connect with the paragraph that you have written.} - P010}

%\myquote{\participant{5}}{The (latest) one seemed to pick up right. From what I was writing for near future. So I think it definitely got the concept and did near future, the far future seemed to go out even further where it was off the rails.}
% \textit{\say{I'm looking at the latest one I did. I mean, the one seemed to pick up right. Where, from what I was writing for near future. So I think it definitely got the concept and did near future, the far future seemed to go out even further where it was off the rails.} - P005}

% \textit{\say{I think that there was like a higher quality of ideas coming from the near future one just because it had like, it had more logic or it like made more sense and sometimes the far ones} - P004}

% \textit{\say{I stopped using the near after a couple of days because I wasn’t getting anything helpful from it. So after I learned that the distant was usually more helpful for me. The distant future one was less random. And usually incorporated more of my story into it.} - P014}

% \myquote{\participant{1}}{Yeah, I think this one is probably my favorite one. Yeah. This one is not bad. It's quite good. Yeah. For example, if I ask for, I need world, so this is why, I need world building for a loud planet. What are the aliens like? What do they do?}
% \cy{This one is not for far future? I think this one is for GPT-plot (AI Plot with Guidance)?}
% \textit{\say{Yeah, I think this one is probably my favorite one. Yeah. This one is not bad. It's quite good. Yeah. For example, if I ask for, I need world, so this is why, I need world building for a loud planet. What are the aliens like? What do they do?} - P001}

% \textit{\say{You know, sometimes I chose both because I just kind of wanted to see the ideas, but , I know if it's something as simple as how's he going to react to this that's near future if I wanted to know, like, what do you think, what do you think his reaction should be? It would and for the far future, it's like, how do you think this is?} - P005}

%This feature was used to produce a follow-up story arc using GPT-3.

% \textit{\say{So the function was helpful for figuring out how to map out a plot. I didn't really start with a plot in mind when I was writing this story.} - P004}

%However, as we started to take a deeper look at the use of this function, we saw that our participants had some complaints with regard to the system. The major challenge with this feature was that it did not always offer plot predictions in the direction that the authors were expecting. This was helpful in the cases where the authors were stuck. However, when it came to scenarios where they were looking for more refined guidance the feature lost its way.
% \cy{This system and study were done last year right before ChatGPT. With ChatGPT/GPT-4, the instruction-following capability largely improved. I feel like we should describe this somewhere. Maybe limitation?}


% \textit{\say{I use the plot next, the second plot idea as it worked a lot when you plot something and it doesn't appeal to you and generate another plot, it gives you a good plot that you can definitely put it} - P010}

%The participants did appreciate the turn-around time for this feature. In comparison to the MTurk feature, this provided them with the desired response so they could repeat the action as often as required till they got the desired response. There were always certain pieces they could adopt into their own work (in \Cref{subsec:similarity-analysis} and \Cref{fig:similarity-behavior}, we also found that AI Plot with Guidance was adopted second frequently).
% \cy{Connected to \Cref{fig:similarity-behavior} where AI Plot+Guidance can be considered second useful (adopted the second frequently).}


% \textit{\say{And this one felt like there was some, like, there was sometimes sort of pieces of information that I could sort of like pull from it. It was also like, it was a little bit more points, but not necessarily a lot. So a lot of times, like, I would just like sit there and I'll just be like, get another plot, get another plot.} - P015}

%They primarily utilized auto-complete for text dumps, avoiding the need to articulate precise thoughts on the story or novel.
%The function allowed them to insert generic ideas for later revision.

%In other cases, it gave them a lot of new ideas and helped with writer's block. Following up with generating new ideas, one participant recommended that the auto-complete feature suggest alternate leads when it comes to completion. They were, in some cases, fascinated by how the system would leave some sentences undone which helped the author think more along the lines of the story (this ``feature'' is not entirely on purpose but we set a 100-word constraint for GPT-3 to encourage users to write).
%Compared to the human feature, we saw people preferred the auto-complete in terms of the immediacy of results.


% \textit{\say{I think I liked the auto complete function the most because it was instant gratification. Because the scope was only like a thousand to 1500 words. Generating later plot points, like distant future plot points or generating the story ideas. I couldn't necessarily use them within this scope.} - P002}

%There was a strong sentiment among participants that they could have used better training in terms of formulating the instructional prompts. A lot of participants remarked that maybe better wording of instructions to AI as well as humans would have led to improved results. For example, guidance about how much text is optimal to select for which task, how detailed the instructions to humans need to be, and how is each AI feature different would have helped participants use the system. As with any tool, some participants felt that the learning curve for the tool affected their use of the tool initially. Both these factors may have affected the outcome of their experience with using the tool. 



% \textit{\say{I didn't understand what the features were actually and I just wrote the story first thinking about the story alone. And then all of a sudden I got interested in these features. I was willing and I was very interested with these features, and I tried the first the human, but the human didn't respond} - P010}

%\myquote{\participant{15}}{So I think maybe more clear instructions of what instructions you can give. That like they're trained for}
% \textit{\say{So I think maybe more clear instructions of what instructions you can give. That like they're trained for} - P015}

%\subsection{Lost Context while Using the Different Features: Both AI and MTurk}

%%:\textit{\say{... they always came through with some interesting directions and it felt like being in a writer's workshop, but it did take longer.} - \participant{4}}

%%\textit{\say{It was awesome to get ideas from people. There was definitely a difference when the person understood the assignment it was more personal and it was more ... that they understood what you were asking and you could trust them more if that made sense} - \participant{5}}

%%\textit{\say{I think the timeframe was like, it's hard to not compare it to the other ones, the other ones were just so much faster. And so that was like the big drawback.} - \participant{4}}

==> sections/8-design-recommendations.tex <==
%\section{Design Recommendation}

\kenneth{We should have at least a few DRs from the writing log analysis I guess?}
\cy{This one is probably worth reading: Mapping the Design Space of Human-AI Interaction in Text
Summarization\url{https://arxiv.org/ftp/arxiv/papers/2206/2206.14863.pdf}}

Based on the user study results, we provided design recommendations for creative writing assistants:

%\kenneth{------------------------ KENNETH IS WORKING HERE: BEGINS -------------------------------}

\begin{itemize}

\item 
\textbf{Improved Human-Matching Feature:}
While the ``ask human'' feature garnered positive feedback, the study identified delays in responses as a significant challenge. 
%Participants suggested finding human helpers motivated by interests rather than just monetary compensation.
Recruiting individuals from writer and reader groups based on the genre of writing could enhance matching. 
Ensuring consistency in human responses, possibly by having the same person provide perspectives on follow-up questions, was also recommended.

\item 
\textbf{Conveying AI's Understanding to Users:}
%The study emphasized the importance of empowering users with control over AI-generated content.
Beyond selecting the context, prompting the AI to generate summaries and pose questions about characters and plot offered users a snapshot of the AI's interpretation.
This reflective tool helps identify potential misalignments between user expectations and AI responses, improving clarity and enhancing the user's understanding of how the AI interprets their inputs.

\item 
\textbf{Allowing Genre or Style Selection:}
%Maintaining consistency in a story, including writing style and character introductions, was deemed crucial.
Participants highlighted issues with the suggested text deviating from the context of their writing. 
Allowing users to specify the genre or writing style could provide the system with additional information, resulting in more refined and accurate auto-complete and plot recommendations.

\item 
\textbf{Visual Changes in Highlighting Text Aid the Writing Process:}
Several participants found it helpful to highlight and categorize different texts with different colors, allowing them to track the status of individual sections and focus on specific areas.
The recommendation included highlighting human-recommended and AI-generated text separately, serving as a productivity tool for future revisions.

\kenneth{I removed Autocomplete as an Idea Placeholder to save some space as we didn't mention this in the qual results.}

%\item 
%\textbf{Autocomplete as an Idea Placeholder:}
%Participants appreciated the autocomplete feature's popularity. 
%While discussions mainly focused on its current capabilities, some users were intrigued by the autocomplete function's potential to generate non-detailed text as a temporary placeholder.
%This feature could enable writers to quickly sketch out ideas for later revision, preventing the loss of creative insights during breaks.

\end{itemize}

%----------------- dead kitten ------------------
\begin{comment}
    



\kenneth{------------------------ KENNETH IS WORKING HERE: ENDS -------------------------------}

%\begin{enumerate}



\item
\textbf{Conveying AI's understanding to users.}
The primary purpose of asking users to select the ``context'' is to empower them with control,
ensuring they have a clear idea of what the AI perceives (see our design principle in \Cref{sec:design-principle-control}).
Yet, a further step can be taken.
By prompting the AI to generate summaries of the selected text and pose questions
about the characters and plot, we can offer users a snapshot of the AI's interpretation
or assumptions based on the provided input (the selected texts and the given prompt).
This function can reveal potential misalignment between user expectations and AI responses,
which can be especially enlightening when the AI behaves unpredictably.
%
The concept of summarization as a tool for reflection is echoed
in the work of \citeauthor{dang2022beyond}.
While their research employed it to assist writers in self-reflecting on their work,
the core principle remains consistent.
Providing users with a summarized perspective -- an AI's interpretation --
serves as a reflective mirror.
Even when users are familiar with their selected text,
this external viewpoint, described as ``AI annotation'', can deliver invaluable insights~\cite{dang2022beyond}.
It acts as a pair of ``fresh eyes,'' which can improve clarity~\cite{tully2019reverse}.
Significantly, this approach can enhance the user's grasp of how the AI interprets their inputs and allows them to check if the conveyed information is comprehensive.


\item 
\textbf{Allowing genre or style selection.}
%When building a story, it is essential that certain consistency is maintained. This extends from the style of writing to character introductions. Multiple participants reported that the recommended text lost the context of their writing (for example, introduced new characters or changed the genre of writing). Having a selection criteria for the genre and style of writing might help with better auto-complete as well as plot recommendations. This would provide the system with additional information for more improved and accurate results.
%\cy{What kind of selection criteria? }
Maintaining consistency in a story is crucial, encompassing writing style and character introductions.
Several participants noted that the suggested text often deviated from the context of their writing, introducing new characters or altering the genre.
Allowing users to specify genre or writing style could give the system additional information, leading to more refined and accurate auto-complete and plot recommendations.

\item
\textbf{Improved human-matching feature.}
While there was a lot of positive feedback and excitement around the ``ask the human'' feature, it did have a lot of pitfalls. Among those, the highest priority is the delay in responses. Most participants felt that an unreliable timeline of the human response creates mismatched expectations of human responses. It might be useful to find human helpers who are more motivated to help based on their interests than just monetary compensation. So, scouting in writer groups as well as reader groups based on genre of writing might be helpful. This would allow the right people to be matched with the right authors. Another suggestion was consistency in human responses, which means having the same person's perspective on follow-up things. If the same set of people are responding to different parts of the prompts and questions it helps in better context establishment. 
\sanjana{Do we want to add more on the comparison between MTurk and recruitment through Facebook groups? Or would that be too much deviation from our current goals?}
\cy{I actually think Facebook groups is a good idea but there are a lot of trade-offs/decisions to make. Should we briefly discuss them?}
\cy{For a community-based solution (Facebook groups), I would expect the response quality would improve but the latency can be even longer as they don't have responsibility for replying to it in time and the number of available people is definitely fewer than workers.}
\cy{I also remember one person (\participant{5} maybe?) mentioned that she feels more comfortable sharing the draft with workers. She is more protective when facing other writers.}
\cy{The feature for having the same person probably works better for Mturk. And that essentially means we give users more control about the recruiting process (ban people, recruit same people, etc)}


\item 
\textbf{Autocomplete as an idea place-holder.}
Participants were drawn to the popularity of the autocomplete feature.
While most of the discussion focused on its current capabilities, some were intrigued by its potential to generate non-detailed text for use as a temporary placeholder.
For instance, a writer could quickly sketch out the next paragraph and, instead of losing the idea during a break, use autocomplete as a placeholder to revisit and edit later.
%The popularity of the autocomplete feature won it attention of the participants. While the majority of the conversation was centered around the current goals that autocomplete was able to meet and achieve, some participants were interested in autocomplete generating non-detailed text to be used as a placeholder for when they return back to the text after further analysis. For example, let us consider a scenario in which a writer has thought through a rough sketch of how the next paragraph looks; they would like to take a break before they resume writing. In such a case, so as to not lose the idea, they would instead use the autocomplete feature as a place-holder that they can later come back to and edit. \sanjana{Might have to further fix the language here.}

\item
\textbf{Visual changes in highlighting text aid the writing process.}
For a number of participants, it was really helpful to highlight and brand different texts with different colors denoting different things. This helped them keep track of the status of individual sections and also redirect their attention to what they were working on. It might also be useful, to highlight human-recommended as well as AI-generated text separately so they might return to it in the future in case they want to make revisions to the same. This helps as a productivity tool.

\kenneth{I removed the prompt sharing idea for now. I didn't see participants suggest this?}

\end{comment}

\begin{comment}


\item
\textbf{Enabling collective intelligence for prompt and experience sharing.}
Participants using our tool primarily faced two prominent challenges:
(\textit{i}) not being able to understand the nuances of usage and differences in functionality, and
(\textit{ii}) encountering difficulties when formulating prompts for the AI.
Although a comprehensive FAQ section can mitigate some of these challenges
by providing the proper use of each feature and outlining expected response times,
it may not be sufficient due to the dynamic nature of LLMs.
As LLMs continue to advance rapidly, their capabilities expand and some existing challenges,
such as LLMs not following instructions in this study,
might be addressed in subsequent versions (\eg, ChatGPT or GPT-4).
%
Although better prompting strategies could also help~\cite{Dang2023Choice,arora2022ask},
we believe the integration of collective intelligence can resolve the problem fundamentally given its fluid nature.
%
% Given this fluid nature, we propose the integration of collective intelligence as a solution.
By facilitating users to share their experiences and effective prompts within \system,
we can create a dynamic knowledge-sharing ecosystem.
We envision a proactive system that, based on the user's selected text,
suggests: ``Based on similar contexts, other users have found success with the following prompts...''.
Furthermore, a mechanism allowing users to rate and share their configurations and outcomes,
when satisfactory, could be invaluable.
Nevertheless, implementing such features requires careful consideration of associated challenges such as privacy concerns where users might want to keep their draft secret while sharing the experience.

    


\cy{I want to merge the following two points with this one and emphasize the importance that LLMs are new and involving, and we are not sure about its capability so we should probably rely on collective intelligence to help.}

% \item 
% \textbf{Nudging the participants in the right direction.}
% One of the biggest challenges that participants faced while using our tool was not being able to understand the nuances of usage and differences in functionality. This leads to a steeper learning curve. We can reduce that by having a more detailed FAQ section that shares with them the correct usage of each individual feature. The FAQ section can further include an estimated response time for human helpers to set more realistic expectations about the turnaround time as well as help them plan their writing process better. 
% \cy{I do have some FAQs and estimated response time (probably not accurate enough and the std is probably high). So I think another way is to use collective intelligence (similar to the following one) again - enabling people to share their experiences/notes with others.}


% \item
% \textbf{Prompt examples for different features.}
% This ties into DR5 with regards to helping participants use the tool better. But having example prompts and their results might help the participants better frame their queries to the AI features for improved and accurate results. A lot of participants seemed to be at a loss when it came to formulating the question prompts.
% \sanjana{Should we link it to prompt engineering as an emerging field?}
% \cy{I don't think prompt engineering can solve the issue. I take prompt engineering as a term to describe the process where we modify the prompts back and forth with or without a certain smart algorithm to improve the overall performance.}
% \cy{I think a better way is to build something for people to share their prompts as templates. There are several platforms out there (team-gpt, prompt pal, etc.) We don't fully understand what LLM can and cannot do so the better way is probably to allow people to share their experiences when they succeed.}




% \item
% \textbf{Creating a discourse community.}
% \kenneth{We do not have to do this.}



%\end{enumerate}


%\end{itemize}
\end{comment}


==> sections/9-1-soc-view.tex <==
Our third suggestion is to view writing through the lens of \soc theories



%---------------- dead kitten ----------------------

In this subsection, we explore users' discourse-aligning behavior when engaging with \system through the lens of \soc theories of writing. 
While this behavior was not a main theme in our analysis, we believe it provides key insights into writers' interactions with LLMs.
During our study, we observed that participants, despite knowing their intent, sometimes used \system to validate their thoughts:
%The following are two examples:

%After having an idea about how readers thoughts, the writers would then consider whether they wanted to adopt the readers opinions or not. When the feedback is not appealing enough, the writers might not buy in the ideas.
\myquote{\participant{5}}{I asked, should she confess the lie to her brother? Or should she insist that there is a boyfriend? 
And \textbf{it (\system) actually got right on what I was going to do} anyhow...
%So I liked the thought that yeah, 
Sometimes this could be either \textbf{confirmation of what I was going to do} or kind of lead me in another direction.%What I didn't like was it lacked the detail to tell me why I would go in another direction, because it was just very vague.
}
%
\myquote{\participant{15}}{I want to see what things, like \textbf{where they (\system) think this story is going and then see whether or not that validates where I have it going in mind.} Or if there's a shift, or if, this is not yet enough content to get an understanding of these characters and where things are happening.}

The discourse community theory used by \soc writing study researchers provides a valuable lens for understanding this behavior~\cite{bizzell2003cognition}.
%With this lens, we can recognize how users' writing behaviors are part of a broader pattern of regular interaction with \system and their intended audiences~\cite{bizzell2003cognition}.
%This perspective also proved useful in interpreting another observation from our study (regarding \participant{1}), which we will describe shortly.

\paragraph{Listening to the Voice of a Discourse Community via LLMs.}
Discourse Community (DC) is a \soc concept that views a genre of writing as a constantly evolving and shared form of communication for a group of individuals who share personal or professional values, interests, or goals~\cite{killingsworth1992}. 
These groups or communities can be defined according to different metrics, such as physical proximity~\cite{swales2017concept} or larger ``landscapes of practice''~\cite{Wenger2000}. 
Professional writers align their work to the implicit and explicit expectations of their discourse community of readers, which give a genre its recognizable features. 
For example, a science fiction discourse community is recognizable because of its expected elements of technology and the future.
Discourse community members have an understanding of unspoken rules and expectations, referred to as ``silential relations''~\cite{becker2000beyond}, which need not be explicitly stated or written down and can explain professional writers' motivations.
Our findings can be understood as that the writers sometimes used \system's generated texts for double-checking their ideas with those ``silential relations.''
Given that LLMs now allow for rich and nuanced interaction, we suggest that \textbf{writers may familiarize and adapt to the conventions or ``voice''~\cite{matsuda2001voice} of their chosen discourse community by observing what LLMs produce in different contexts.}
In the cases of \participant{5} and \participant{15} above, both note an expectation of either validation of their thinking about a story's next steps or a ``direction'' change.
Because both participants explained the possibility of a ``shift'' or change in ``direction'' for the story prompting their use of \system in these moments, we can understand how participants already have some conceptual understanding of an appropriate style or voice for their intended discourse community participation. 
%Participants' recognition of a possible need to change the direction of their stories exemplifies how both writers and audiences participate in adaptations to a discourse community convention or norm.

\paragraph{Risks of Using LLMs as Voice.}
The \soc lens explicates the risks of using LLMs' outputs to learn and negotiate the convention of a community.
First, the most obvious issue is the social-technical gap~\cite{ackerman2000intellectual} between what writers want LLMs to provide and what LLMs can provide.
LLMs' outputs, at their best, can only be described as a rough representation of the community's convention captured in the LLMs' training data.
Due to the technical limitations of LLMs, the authenticity and level of detail in such representations are likely distant from what the community convention actually is because genre is constantly negotiated and updated by all discourse community members~\cite{Wenger2000}. 
Such fluidity contrasts with the static, frozen data used to train LLMs. 
Second, the deeper issue is that LLMs could reinforce the outdated voice of a discourse community and suppress the newly emerged voice.
For example, \participant{1} was writing a queer story, but the ideas suggested by the AI-based functions were always about heterosexual relationships.
There were also gender biases in the suggestions:

\myquote{\participant{1}}{I could imagine some people if they're writing like \textbf{queer story}. I think \textbf{all the suggestion that gave me was heterosexual relationship}.}
\myquote{\participant{1}}{... (\plot) gave me something like `she blushed when she realized people were looking at her naked body.' It's a bit like what I just described previously, like women are dispensable.}
%\kenneth{TODO: Update ``[AI Plot Generation]'' with the new name.}

%Such bias could convey problematic values to users and require more attention. 
%Participants in Dramatron~\cite{mirowski2022co} also found that LLMs sometimes generated predictable outputs and occasionally gave responses with problematic stereotypes.

One could argue that writers, with their unique agency, would not easily succumb to biases present in machine-generated texts. 
However, a well-documented phenomenon known as ``automation bias'' exists, where individuals place undue trust in computer-generated solutions~\cite{10.1136/amiajnl-2011-000089}. 
The predisposition to accept something once it is written out~\cite{gero_2022} could lead writers to inadvertently adopt outdated or biased conventions when influenced by LLMs. 
This reflects the broader issue where machine-learning models, trained on pre-existing data, can amplify entrenched biases, such as gender-related~\cite{zhao-etal-2017-men} or nationality biases~\cite{venkit2023nationality}. 
Like other technologies, LLMs have the potential to disproportionately benefit those who are already powerful.

%----------------------- dead kitten ----------------

\begin{comment}



Second, the deeper issue is that LLMs could reinforce the outdated voice of a discourse community and suppress the newly emerged voice. For example, P001 was writing a queer story, but the ideas suggested by the AI-based func- tions were always about heterosexual relationships. There were also gender bias in the suggestions.

\kenneth{----------------------KENNETH IS WORKING HERE----------------------}
\bigskip

%\kenneth{Basically say the confirmation and validation behavior can not be very well interpreted by cognitive process model of writing, so we look for \soc theories of writing. \Soc theories could better point to potential risks of using LLMs in writing.}

%\kenneth{Point to the LGBT authors' comments, saying the power issue in \soc views.}

%\kenneth{Then probably eventually bridge to Avon's writing, saying this kind of thought is in fact relevant to HCI community.-- Avon, I moved your writing to here.}



In this subsection, we explore users' ``norm-aligning'' behavior when engaging with \system through the lens of \soc theories of writing.\kenneth{Is ``norm-setting'' a good word here? Or should we call it norm-seeking? Norm-following?...}\smb{i might suggest "norm-aligning" behavior. the section here is focused on how participants demonstrated evidence of using Inspo to "validate" their thoughts. the data excerpts, to me, demonstrate that writers already had an expectation of the way their writing might fit into the anticipated genre \& discourse community they wanted to be a part of (eg., using language that suggests "right" and "wrong" writing alternatives). this suggests to me that writers, as they are professionals, already have a working conceptual apparatus of what the discourse community expects and/or how to participate in the discourse community and Inspo was able to validate their alignment with that discourse community. }
While this behavior was not a main theme in our analysis, we believe it provides key insights into writers' interactions with LLMs.

During our study, we observed that participants, despite knowing their intent, sometimes used \system to validate their thoughts.
The following are two examples:

%occasionally knew what they intended to write but still sought ideas from \system to ``double-check'' their thoughts. 
%The participants 
%used \system to ``double check'' their writing plans.
%That is, participants already had concrete writing plans in mind, but they were not sure what the audience thought about their ideas. 
%if the idea would make sense to their target audience. 
%Via \system, the writers tried to probe readers' expectations of the following part, people's thoughts about various story directions, and if readers could understand the current snippet. 
%\myquote{P4}{With a human, I think it was fun to play around with the directions and be like, so what do you think? Like, I want this to be X, Y, Z, \textbf{where should I go now?}}
%\myquote{P14}{Sometimes I needed to see how [sic] what I'd written had come across before I moved on to the next part, ... essentially to see if what I was saying made sense to them or \textbf{what they were thinking was happening}.}


%After having an idea about how readers thoughts, the writers would then consider whether they wanted to adopt the readers opinions or not. When the feedback is not appealing enough, the writers might not buy in the ideas.
\myquote{\participant{5}}{I asked, should she confess the lie to her brother? Or should she insist that there is a boyfriend? 
And \textbf{it (\system) actually got right on what I was going to do} anyhow...
%So I liked the thought that yeah, 
Sometimes this could be either \textbf{confirmation of what I was going to do} or kind of lead me in another direction.
%What I didn't like was it lacked the detail to tell me why I would go in another direction, because it was just very vague.
}
%
\myquote{\participant{15}}{I want to see what things, like \textbf{where they (\system) think this story is going and then see whether or not that validates where I have it going in mind.} Or if there's a shift, or if, this is not yet enough content to get an understanding of these characters and where things are happening.}


%A subtler version of this behavior is when writers asked \system to choose from a set of follow-up plots:
%A subtler instance of this behavior occurred when writers asked \system to choose from a set of follow-up plots.
%probe readers' expectations of the following part, people's thoughts about various story directions, and if readers could understand the current snippet. 
%\myquote{P4}{With a human, I think it was fun to play around with the directions and be like, so what do you think? Like, I want this to be X, Y, Z, where \textbf{should} I go now?}

%\myquote{P14}{Sometimes I needed to see how [sic] what I'd written had come across before I moved on to the next part, ... essentially to see if what I was saying made sense to them or \textbf{what they were thinking was happening}.}


%(see Section~\ref{}.)\kenneth{Maybe add an explicit reference to here. Which section we're talking about?}
In collaboration with writing researchers from the English department, one of whom became a co-author, we found that the discourse community theory in \soc studies of writing provided a valuable lens for understanding this behavior (Section~\ref{sec:dc-and-llm}). With this discourse community theory lens, we can recognize how participants’ writing behaviors are part of a broader pattern of regular interaction with \system and their intended audiences~\cite{bizzell2003cognition}.\kenneth{Maybe cite some more papers?}
This perspective also proved useful in interpreting another observation from our study (Section~\ref{sec:dc-and-llm-risk}).

%\kenneth{I removed the historical debate of the cog vs. \soc camps, which is interesting story, but probably not very relevant to this paper.}

\subsubsection{Listening to the voice of a discourse community via LLMs\label{sec:dc-and-llm}}
Discourse Community (DC) is a \soc concept that views a genre of writing as a constantly negotiated, evolving, and shared form of communication for a group of individuals who share personal or professional values, interests, or goals~\cite{killingsworth1992}.
Professional writers align their work to the implicit and explicit expectations of their discourse community which give a genre its recognizable features—that is, a science fiction discourse community is recognizable because of its elements of technology and the future while a horror fiction discourse community is characterized by frightening themes and suspense. What is considered a rule or appropriate to a genre discourse community is not static, however, because audiences and writers participate across various discourse communities~\cite{porter1986} and their import-export practices negotiate--or ``broker''~\cite{Wenger2000}--content, style, and themes between discourse communities (see \Cref{sec:dc-and-llm-risk}).
\kenneth{Need to add a few words here to explain to a broader/AI audience what ``negotiation'' means here.}
\citet{swales2017concept} then expanded the definition of a discourse community to reflect that a community's membership is fluid and that the intercommunication among community members could be more distributed.\kenneth{This might need to be more direct, e.g., what was not good about the original version of DC? How does this expanded version better connect to our current world?}
\smb{In the interest of keeping this section concise, I’ll offer an idea that could go here (but I do think that the point is made between these two sentences so maybe this isn’t necessary?):
%
The expanded version of DC better connects to the distributed reality of our digital interactions. In other words, now sociocultural linguists and compositionists understand the various scales of communicative interaction. For example, our collaborative authorship is indicative of the tensions (productive and limiting) of distributed discourse communities: While we both operate in the broader scale of academic/higher education discourse community (which is distinct from primary education or trade discourse communities), I operate much more local scale of rhetoric and linguistics and you operate in your local HCI discourse community. We are bringing these discourse communities—as well as the distributed nature of our multilingualness—to this collaborative authorship, too.}
Swales also recognized that a discourse community develops an understanding of unspoken rules and expectations, referred to as ``silential relations,''~\cite{becker2000beyond} which need not be explicitly stated or written down.
Our findings can be understood as that the writers sometimes used \system's generated texts for double-checking their ideas with those ``silential relations.'' 
%To elaborate, the participants used \system to seek people's thoughts, expectations, and understandings about the various story directions.
%They also thought LLM's feedback could be treated as a human reader's.
%After having either human or AI readers' feedback from \system, writers considered the feedback either as a confirmation that the current story makes sense or a lead to other story directions.\kenneth{what does ``a lead to...'' mean here?}
DC theory underscores that true the most valuable knowledge of a discourse community can only be learned by actually participating in-- and becoming a member of-- the community; static artifacts like books, articles, and tutorials cannot substitute for this interaction with community members.
%understanding of a discourse community comes from active participation, and static artifacts like books, articles, and tutorials cannot substitute for this interaction with community members.
%Although static artifacts such as books, articles, tutorials, and written instructions can help people learn the historical context of the community, \soc theories emphasize that the most valuable knowledge of a discourse community can only be learned by actually participating in-- and becoming a member of-- the community~\cite{samimy2011participative}.
Given that LLMs now allow for rich and nuanced interaction, we suggest that writers may familiarize and adapt to the conventions or ``voice''~\cite{matsuda2001voice} of their chosen discourse community by observing what LLMs produce in different contexts.
%Drawing on the theory of discourse community, we argue that writers sometimes learn and negotiate the conventions or ``voice''~\cite{matsuda2001voice} of their chosen discourse community by seeing what LLMs generate in various scenarios.\kenneth{``argue'' might be too strong here.}
\kenneth{We should elaborate a little here about what DC theories says about how people interact with the convention of a DC? A few sentences and references that connect back to our example should be fine.}
\smb{Do you think we need more? I’m wondering about the organization because in order to address the question above about negotiation, I indicate that discussion continues in 9.1.2. if you do think we need more here, could you confirm if this is what you’re referring to:
%
When I read this, I interpreted it as saying maybe make a comment here about how with DC, we can see the participants searching for validation from the LLM of their proper participation in the ``voice'' of the discourse community—is that correct?
%
If so, I think that connects to what I was writing above in a comment about “norm-aligning.” 
%
Here’s a suggestion, if I’m correct in my interpretation of your comment:
}
In the cases of \participant{5} and \participant{15} above, both note an expectation of either validation of their thinking about a story's next steps, or a ``direction'' change. Because both participants explain the possibility of a ``shift'' or change in ``direction'' for the story prompting their use of \system in these moments, we can understand how participants already have some conceptual understanding of an appropriate style or voice for their intended discourse community participation. Participants' recognition of a possible need to change the direction of their stories exemplifies how both writers and audiences participate in adaptations to a discourse community convention or norm.

\subsubsection{Risks of using LLMs as voice\label{sec:dc-and-llm-risk}}
The \soc lens explicates the risks and concerns of using LLMs' outputs to learn and negotiate the convention of a community.

First, the most obvious issue is the social-technical gap~\cite{ackerman2000intellectual} between what writers want LLMs to provide and what LLMs can provide.
LLMs' outputs, at their best, can only be described as a rough representation of the community's convention captured in the LLMs' training data.
Due to the technical limitations of LLMs, the authenticity and level of detail in such representations are likely distant from what the community convention actually is.
%\kenneth{Need a sentence here to wrap up.}
%Learning the convention of a community solely from LLMs 
%LLMs are known to generate inaccurate content~\cite{ji2022survey}; %writers sometimes found LLMs fail to capture the nuance of their writing %style~\cite{10.1145/3490099.3511105}.
%WHY: 2
%Second, 
A genre is constantly negotiated and updated by all discourse community members~\cite{Wenger2000}.
%\kenneth{Is the second and the first potentially the same thing? First says technical limitation; second says even it's technically capable, it's inherited the limitation.}
Such fluidity contrasts with the static, frozen data used to train LLMs, which could not accurately reflect the current conventions of the community.
%
%LLMs, like many technologies, can be used as a proxy of reality in order to provide support in human tasks.
%The risks, like many technologies, lie in the potential neglection of the gaps between the proxy and reality.
LLMs, like other technologies, can be used as a stand-in for reality to provide support in human tasks.
However, like other technologies, there is a risk of overlooking the differences between the stand-in and actual reality.

Second, the deeper issue is that LLMs could reinforce the outdated voice of a discourse community and suppress the newly emerged voice.
%These biases are not significantly harmful and mostly affect the quality of the generated inspirations. 
%However, participants also noted potentially problematic biases. 
For example, P001 was writing a queer story, but the ideas suggested by the AI-based functions were always about heterosexual relationships. There were also gender bias in the suggestions.
\myquote{\participant{1}}{I could imagine some people if they're writing like \textbf{queer story}. I think \textbf{all the suggestion that gave me was heterosexual relationship}.}
\myquote{\participant{1}}{[AI Plot Generation] ... gave me something like `she blushed when she realized people were looking at her naked body.' It's a bit like what I just described previously, like women are dispensable.}
%
Such bias could convey problematic values to users and require more attention.
Participants in Dramatron (\cite{mirowski2022co}, Section 5.3) also found that LLMs sometimes generated predictable outputs and occasionally gave responses with problematic stereotypes.

One could argue that writers, with their unique agency, would not easily succumb to biases present in machine-generated texts.
However, a well-documented phenomenon known as automation bias exists, where individuals place undue trust in computer-generated solutions.
Dr. Katy Gero captured the essence of this in writing: ``...once something is on the page, it's just a little bit harder to imagine anything else''~\cite{gero_2022}.
This predisposition could lead writers to adopt outdated or biased conventions when influenced by LLMs inadvertently.
This reflects the broader issue where machine-learning models, trained on pre-existing data, can amplify entrenched biases, such as gender-related~\cite{zhao-etal-2017-men} or nationality biases.
The initial motivation for many automation efforts was to provide increased accessibility for marginalized groups who lack resources, like with automated tutors or therapy chatbots.
However, similar to other technologies, LLMs have the potential to disproportionately benefit those who are already powerful.\kenneth{This is spicy hahaha} \smb{Yes, it is! But I like it…it’s very true. }

\end{comment}



==> sections/9-discussion.tex <==
%\subsection{Design Implications}
%\kenneth{TODO HCOMP: (1) Keep three key points and make them inline instead of bullet points. (2) Echo LLM is better than human narratives; cite Steven's CHI paper.}
%\input{sections/8-design-recommendations}


\paragraph{Humans in the Loop in the Era of LLMs.}
In the Introduction, we noted that humans generally excel over state-of-the-art LLMs like GPT-4 in creative writing~\cite{bellemare2024divergent}.
However, in our study, even though we used the older and less capable GPT-3, many participants still increasingly favored AI assistance over \crowd for writing.
This suggests that for human-in-the-loop systems to remain valuable, human components must be highly skilled, handling tasks beyond the capabilities of LLMs. 
For instance, participants in our study recommended enhancing the \system's \crowd function with more skilled contributors, such as writers or editors---a suggestion less common in the user study of earlier writing assistants relied only on crowds before LLMs were available, such as Heteroglossia~\cite{heteroglossia-huang-2020} 
%This contrasts with earlier studies on crowd-powered writing assistants like Heteroglossia~\cite{heteroglossia-huang-2020}, which relied solely on crowds before the advent of LLMs. 
Ensuring high-quality human involvement in these systems poses a significant research challenge for the human computation community.







%\paragraph{Limitations.}
%We recognize several limitations in our study.
%First, \system was based on GPT-3 and inherited its drawbacks, such as lack of transparency and being less advanced than GPT-3.5/GPT-4. 
%Second, choosing a deployment study over an in-lab study improved scalability but compromised the depth of data, particularly in understanding participants' intent at specific times.
%Thirdly, \system included a credit system to reflect the financial cost of each request, and participants were informed that using the \crowd option would cost more credits.
%Although we consider this a minor factor---since participants used far fewer credits than allocated, %(typically only 1 out of 100), 
%and we offered more credits if needed---it may still have slightly influenced their willingness to use the \crowd option.
%Finally, our study was brief. 
%A longer observation period could reveal more about how participants adapt to and utilize the system over time.











\subsection{A \Soc View of Writing}
\input{sections/9-1-soc-view}












\begin{comment}
Lastly, using a \soc view of writing introduces inherent limitations.
For instance, various parallel \soc views of writing exist under the broader umbrella, often disagreeing on specific topics. 
While we recognize writing communities by their unique styles in this work, some scholars advocate for more detailed classifications based on location~\cite{swales2017concept}. 
Others view these communities as part of larger ``landscapes of practice,'' complex systems shaping unpredictable human activities~\cite{wenger2010communities}.
Some particularly emphasize community boundaries and the challenges of belonging to conflicting groups~\cite{wenger2010communities,samimy2011participative,mccook2016literacy}.
Further research is needed to understand how writers' use of LLMs is perceived across these varied \soc perspectives.
\end{comment}




%-------------- dead kitten -------------
\begin{comment}





%On the surface, online crowd work has inherent technical limitations, including longer latency and high costs to control quality.
A higher-level implication is that with the readily available, low-cost, and decent LLM option for assistance, human components in human-in-the-loop systems must now be more capable, handling tasks that LLMs cannot yet manage.
%This enhancement in human input will demand greater effort and attention from both system builders and human workers.
%As supporting evidence, 
Participants in our study suggested that \system's crowd function could benefit from more skilled individuals, like writers or editors---a suggestion less common in the user study of earlier writing assistants relied only on crowds before LLMs were available, such as Heteroglossia~\cite{heteroglossia-huang-2020}

%\kenneth{TODO HCOMP: Ackonwledge that the study is too old :(}
We acknowledge several limitations in our work. 
Firstly, \system used on GPT-3 and inherited its limitations, such as being a closed model lacking transparency and being weaker than GPT-3.5 and GPT-4.
Secondly, opting for a deployment study over an in-lab study prioritized scalability but resulted in a trade-off: 
% as discussed in Related Work (Section~\ref{subsec:related-work-in2writing}),  --> don't have this anymore
while analyzing writing logs allowed us to observe behavior, it led to a lack of nuanced data on participants' intent at each timestamp.
Thirdly, our study of most participants lasted only one week; observing them for longer, like months or years, could yield more interesting findings as they become proficient with \system.
%\kenneth{For HCOMP, I removed the }

The panel also displays the user's remaining credits and the cost of each task, calculated based on task type, snippet length, and specific parameters.\kenneth{TODO HCOMP: We should add here to say that we have a credit system, initially intended to understand the trade-offs BUT we gave a lot more credit than people used so we don't believe this is very important to the study results.}



%\kenneth{In the era where LLMs can give you really really fast and NOT so bad results; it's extremely easy to fall for automation bias and go with it. So the human involvements need to be good. And often enough it's not (!!!!)}

%\kenneth{Say we know the trade-offs.-- This needs some more work and rearrange.}
%\cy{The user study is conducted with GPT-3 (before ChatGPT era).}
%\cy{The elephant paper. We can do fully remote study for days but we can not do think aloud. But compared to Wordcraft, the writing logs can still provide some insights similar to think aloud (probably).}

%Despite this work's interesting findings and contribution, 
We are aware of some limitations of our work.
\kenneth{First, \system used GPT-3 and therefore inherited many of its limitations, e.g., being a close model that lacks transparency, weaker than GPT-3/GPT4, etc. Second, as mentioned in Related Work (Section 2.1), we chose a deployment study over an in-lab study, prioritizing scalability regarding the number of writing hours and participants we could recruit. While we could analyze participants' writing logs to observe behavior, the trade-off was a lack of nuanced data on participants' intent at each timestamp. Third, we only studied most of our participants for one week. As participants were learning to use \system, observing them for longer, such as months or years, might result in more interesting findings. Finally, we used a \soc view of writing to examine some of our observations, which inevitably inherited the limitations of such views.
For example, a set of parallel \soc views of writing exist.
Although the views all fall under the broader umbrella, they often disagree on specific topics. 
In this work, we recognize writing communities by their unique styles, but some scholars seek more detailed classifications based on location~\cite{swales2017concept}.
Others view these communities as part of larger ``landscapes of practice,'' which are complex systems shaping unpredictable human activities~\cite{wenger2010communities}.
Some particularly emphasize community boundaries and the challenges of belonging to several conflicting groups~\cite{wenger2010communities,samimy2011participative,mccook2016literacy}.
More research is needed to grasp how writers' use of LLMs is perceived across these varied \soc perspectives.
}

\begin{itemize}
    \item 
%First, this project only focuses on a particular version of LLM, i.e., GPT-3, which inherently has a set of limitations: it is a close LLM instead of open models such as GPT-2 or Lamma, so we do not know its training data and detailed models setups; it was released before its strong successors such as GPT-3.5/GPT-4, so some of the issues we observed in the study could have been mitigated.
First, this project exclusively targets GPT-3 and acknowledges its inherent limitations. GPT-3, being a closed language model, lacks transparency regarding its training data and detailed model setups, distinguishing it from open models like LLaMA. 
Additionally, since GPT-3 predates its robust successors like GPT-3.5/GPT-4, some of the issues identified in the study might have been addressed in the newer versions.




\item
%Second, we decided to conduct a deployment study instead of an in-lab study, which intentionally traded the data types we could collect for scalability.
%Although we could observe participants' writing behavior by analyzing their writing logs, we did not have nuanced data on participants' intent at each timestamp, which in-lab studies like think-aloud studies could otherwise capture.
Secondly, we chose a deployment study over an in-lab study, prioritizing scalability regarding the number of writing hours and participants we could recruit. While we could analyze participants' writing logs to observe behavior, the trade-off was a lack of nuanced data on participants' intent at each timestamp, details that in-lab studies like think-aloud studies could capture.



\item
%Third, even though one participant used \system for one month, our work primarily studied writers for no more than a week.
%As people likely develop strategies to incorporate new technologies over time, some interesting use cases or interactions might emerge if we observe users for months or years.
Thirdly, while one participant utilized the system for a month, our study focused on writers for no more than a week. Observing users over more extended periods, such as months or years, could reveal interesting use cases or interactions, as individuals develop strategies for incorporating new technologies over time.



\item
Finally, we used a \soc view of writing to examine some of our observations, which inevitably inherited the limitations of such views.
For example, a set of parallel \soc views of writing exist.
Although the views all fall under the broader umbrella, they often disagree on specific topics. 
In this work, we recognize writing communities by their unique styles, but some scholars seek more detailed classifications based on location~\cite{swales2017concept}.
Others view these communities as part of larger ``landscapes of practice,'' which are complex systems shaping unpredictable human activities~\cite{wenger2010communities}.
Some particularly emphasize community boundaries and the challenges of belonging to several conflicting groups~\cite{wenger2010communities,samimy2011participative,mccook2016literacy}.
More research is needed to grasp how writers' use of LLMs is perceived across these varied \soc perspectives.


\end{itemize}

\bigskip

Finally, we used a \soc view of writing to examine some of our observations, which inevitably inherited the limitations of such views.
\kenneth{Theories can disagree with each other; compared with cognitive view, it's harder to model.}

\bigskip


We are aware of some limitations of our work. 
First, this research is motivated and driven by the \soc views of writing, which inevitably inherits the limitations of such views.
For example, a discourse community's historical, social, and cultural contexts are often complex and fluid, making it challenging to isolate specific \soc behaviors and build tools to support them.
Furthermore, a set of parallel \soc views of writing exist. 
Although these views all fall under the broader umbrella, they often disagree with each other on specific topics.
In the follow-up subsection, we will overview these differences briefly.
Second, while we are confident that the high-level takeaways will remain valid, this project only focused on a particular version of LLM.
Some of the issues, such as the flaws of GPT-3, will likely be mitigated to some degree in the future.
Finally, even though one participant used \system for one month, our work primarily studied writers for no more than a week.
Like other new technologies, people develop strategies to incorporate them over time.
Some interesting use cases or interactions might emerge if we observe users for months or years.

%Originally, the drive for automation aimed to amplify accessibility, particularly for marginalized groups, evidenced by innovations like automated tutors or therapy chatbots for quitting drugs. Yet, there's a looming risk: technologies, including LLMs, might primarily benefit those already in positions of power, reinforcing existing imbalances.







%\kenneth{Add the LGBT thingy here, NOT just biases, but voices.}
People are known to exhibit automation bias, where they excessively trust and rely on computer-generated solutions.
In the domain of writing, Dr. Katy Gero's article summarized it the best: ``...once something is on the page, it's just a little bit harder to imagine anything else.''~\cite{gero_2022}
As a subtle consequence, LLMs could make it easier for writers to fall back to an older, outdated version of the convention of a community.
\kenneth{I'd probably argue that LLms will be more annoying than predicting next token etc}
This is a symptom of a common effect that machine-learning models learn from existing data and amplify existing biases, \eg, gender biases~\cite{zhao-etal-2017-men} or nationality biases.\kenneth{Cite my paper}
The initial motivation for automation was to provide increased accessibility for marginalized groups who lack resources.
However, similar to other technologies, LLMs have the potential to disproportionately benefit those who are already powerful.\kenneth{This is spicy hahaha}

\kenneth{Kenneth is writing here}




\subsubsection{LLM as a proxy of a discourse community}
We think \system could serve as a writers' discourse community. 
\overview{Introduction/Definition of discourse community}
%edited by MB
%We analyzed interview transcripts and writing logs through the lens of the \textbf{\em discourse community}, a \soc concept that views a genre as the result of the latest negotiation between all members of a community.
%edited by Shannon
The \textbf{\em discourse community} is a \soc concept that views a genre of writing as a constantly negotiated, evolving, and shared form of communication for a group of individuals who share any number of personal or professional values, interests, or goals. %edited by MB
\citet{swales2017concept} then expanded the definition of a discourse community to reflect the reality that a community's membership is fluid and that the intercommunication among community members could be more distributed. 
%edited by Shannon
Swales also recognized that a discourse community develops an understanding of unspoken rules and expectations, referred to as ``silential relations,''~\cite{becker2000beyond} which need not be explicitly stated or written down.

\overview{The reason why the system is a discourse community}
This concept is particularly interesting to us because the back-and-forth interactions between writers and LLMs can be characterized as an act of negotiation in the service of a writer's participation in a particular discourse community. 
\overview{Instance: Summary of CSCW 7.3: Using LLMs to Learn and Negotiate with Conventions}
For example, we found writers sometimes used \system's generated texts to double-check their ideas with those ``silential relations.'' 
To elaborate, our participants used \system to seek people's thoughts, expectations, and understandings about the various story directions. %P4, P14
They also thought LLM's feedback could be treated as a human reader's. %P15, P5
After having either human or AI readers' feedback from \system, writers considered the feedback either as a confirmation that the current story makes sense or a lead to other story directions. %P5
Drawing on the theory of discourse community, we argue that writers learn and negotiate the conventions or ``voice''~\cite{matsuda2001voice} of their chosen discourse community by seeing what LLMs generate in various scenarios.

\overview{Compare with related work: cognitive view v.s. sociocultural view}
In contradiction to the \textit{inner-directed} cognitive view of writing, which focuses on writers' internal assembling processes (e.g., planning, transcribing ideas to text, and reviewing~\cite{flower1981cognitive}), the \textit{outer-directed} sociocultural perspective considers writing as a social technique shaped and mediated by social situations~\cite{bizzell2003cognition}.
Most existing writing assistants are driven by the cognitive camp (e.g., Grammarly), 
%even though \soc theories are the dominant paradigm in today’s writing research~\cite{prior2006sociocultural} (an outcome of the theoretical debates between the two camps in the 1980s). 
even though empirical research on writing and language has increasingly turned to \soc theories as a result of intense theoretical debates in composition pedagogy and writing studies in the 1980s~\cite{prior2006sociocultural}.
% 
The theory of discourse communities offers writing-support researchers a \soc analytical lens that sees a writer's language and writing habits as part of a broader pattern of regular interaction with audiences~\cite{bizzell2003cognition}.
% While there are many ways to think about the sociality of writing, here we focus on the influences and implications that writers' perceived discourse communities have on their writing-- for instance, typified language use and writing patterns (genres) recognizable to and accepted by their audiences. 
% We believe the idea of a discourse community-- regardless of how dispersed or abstract they are across space and time-- more holistically addresses the decisions writers make as they write. 
% Writers do not write ``as isolated individuals but as members of communities... [their] aims and intentions in writing are not merely personal, idiosyncratic, but reflective of the communities to which [they] belong'' (\cite{harris1989idea}, p. 749).
We make use of a theory of discourse communities to understand how [semi-]professional writers interact with and negotiate \system given their complex social and abstract discourse communities of authorial peers and audience members.




\overview{Connect with related work: creative writing support}
\avon{Address collaborative writing if having space.}
\avon{I feel that some previous creative writing support tools can be viewed as discourse communities. But, which ones?}
-CreativeHelp: Generate follow-up sentence

-InkWell: Imitate the writer's personality to provide stylistic variations

-Metaphoria: Create metaphors by connecting concepts

-Heteroglossia: Elicit story plot ideas from online crowd workers

-Clark: take turns coauthoring the story with writers

-Generating story continuations~\cite{roemmele2015creative}, predicting plots~\cite{huang-huang-2021-semantic}, or modeling story arcs~\cite{chung2022talebrush}.

\overview{Design implications that facilitate writers to engage in their discourse community}
We further demonstrate the explanatory power of the discourse community theory by using it to interpret what writers might expect from LLMs and the apparent risks of using LLMs to learn a community's voice. 
\avon{Add design implications here.}
\avon{In CSCW paper, we claim only LLM as a discourse community. In CHI, do we wanna claim both AI and human discourse communities?}
\avon{Can existing collaborative writing tools as an inspiration for design implications?}
Our core contribution is to offer a new perspective on the interactions between writers and LLMs, informing the design of future writing assistants that prioritize text generation.

Lessons learned from blog muse: audience-based inspiration for bloggers
We have designed and implemented a novel system -- called Blog Muse -- whose goal is to inspire potential blog writers by connecting them with their audience through a topic-suggestion system.
→ suggest writers what readers want!

BunCho: AI Supported Story Co-Creation via Unsupervised Multitask Learning to Increase Writers’ Creativity in Japanese
Crowd workers (readers) support the revision of the synopsis.
→ The difference in the use of crowd workers

“It’s Complicated”: Negotiating Accessibility and (Mis)Representation in Image Descriptions of Race, Gender, and Disability (CHI’21)
Content creators are concerned about how to write appearances to not lead to misrepresentation of image descriptions.
→  Writer Reader co-writing



\subsubsection{Common Use Cases}
\avon{What are the other findings in CSCW writing that are related to the discourse community? I feel like some common use cases, and concerns (in CSCW paper) could be included!}
\paragraph{Getting Language Suggestions.}
\label{sec:use-case-language-use}
% \cy{Google: 6.2 - Wordcraft as a Fellow Writer}
Similar to Wordcraft's fellow writer (\cite{ippolito2022creative}, Section 6.2) where participants used LLMs to rewrite or continue the story and picked the desired sentences, 
one major use case is to learn certain words or language from \system. Some users found the suggestions matched their expectation or were even higher quality. This is particularly useful for writers because Auto-Completion can mimic the writer's voice. 
\cy{Say something about DC?}%
\cy{This part can probably be explained by DC as writers are carefully picking up the desired language for a certain genre.}%
\myquote{P1}{What helps me is sometimes \textbf{I learn new ways to say something}... It's more like the \textbf{language level inspiration}. Not the plot idea level, but for that it's still helping me.}
%
P5, P14, and P15 mentioned that some wording suggestions from \system were so good and aligned so well with their writing that they used the suggestions in their story.
\myquote{P5}{If I didn't copy all of it, \textbf{I would copy parts of it} because I liked, you know, \textbf{the style of the sentence} and everything.}
\myquote{P14}{I didn't copy and paste, but \textbf{I grabbed certain words}. Yeah. So never a full sentence, but maybe like a few [words] in a row.}
\myquote{P15}{Sometimes it would just be a word and I'd just be like, you know what? \textbf{That is a really good transition word, I'm going to use it} and just sort of little things like that.}




\paragraph{Exploring Possibilities by Querying Multiple Suggestions}
% \cy{Deepmind: 5.1.2 - seed-based generation. }
% \cy{Google: 6.5 - Theme and Variations}
% Use the ``Get Another Plot'' function to get multiple suggestions. 
% (1) People use this to give INSPO another chance to see if it can generate a better suggestion.
% (2) People use this to generate all the possible outcomes.
% This one is probably related to the negotiation behavior (Users negotiates with the AI) 
% \cy{Which paper can we cite to explain the negotiation behavior?}
\system's ``Get Another Plot'' button allows users to ask for multiple suggestions for the same text. 
We found that some participants developed strategies to use this feature: 
some participants gave \system another chance to see if another plot better aligned with their need, 
while others requested a lot of suggestions to see all the possible outcomes of story paths or language uses. 
Similar behaviors were also found in both WordCraft (\cite{ippolito2022creative}, Section 6.5) and Dramatron (\cite{mirowski2022co}, Section 5.1.2) where LLMs were used to generate multiple responses.
We argue that such behavior can be seen as writer trying to negotiate with \system to find a path that both the writer and the target discourse community can accept.

% \myquote{P2}{Now I know \textbf{I can just click generate more ideas or I need to pick more text}. It's still AI. It's not my brain. ... It isn't that good yet.}
% \myquote{P10}{When you plot something and \textbf{it doesn't appeal to you and generate another plot}, it gives you a good plot that you can definitely put it.}
\myquote{P14}{Decide if it works with my story or if it gives me any other ideas. And if it did, I would write that next part.\textbf{ If not, I would try and either get a new idea from the generator}.}
%
% P2 and P15 also shared how they asked \system to generate a lot of ideas and browsed all the possible ways to continue the story or describe things:
% \myquote{P2-\nanowrimo}{I think I got into the habit of asking for three ideas. So the first little bit I was like, I'll just see what the first idea is and then ask for a third one or second one. And I think when I started, then I just got in the habit of like, \textbf{I'm just going to ask it to give me three or four different ideas immediately}.}
\myquote{P15}{\textbf{I would generate a couple of those} sometimes too just to be like, \textbf{what language is it using? What sort of things is [it] putting in here?}}
\myquote{P15}{I think there was one that I had seven plot ideas on. Cause I was just like, \textbf{what else do you get for me}? And it wasn't that they were bad or anything. It was that the interaction was cheap and it was a quick response. \textbf{And it gave me the most sort of ideas} in that short period of time.}


\paragraph{Getting Inspirations for Story Development}
% \cy{Deepmind: 5.2.1 - Inspiration for the Writer. (helping writer's block)}
% \cy{Google: 6.1 Idea Generation and Brainstorming}
% Users get a better picture of what they are going to write or something to think about.
% => Using the concept.
% \cy{Basically to see what other people would do in the community.}
Participants used \system to brainstorm world building and plot planning or when stuck in their writing. 
Although some ideas were not adopted into the story, they helped writers think creatively about what might happen.
Again, both WordCraft (\cite{ippolito2022creative}, Section 6.1) and Dramatron (\cite{mirowski2022co}, Section 5.2.1) reported a similar use case where LLMs were used for brainstorming.
\cy{Can we explain anything using DC here?}%
For example, P1 asked \system to come up with some ideas of how magic works for building the worlds in the story:
\myquote{P1}{Please give me some spells, how does the magic work? And then this one is okay. There is one of the bots, tell me this, which is not bad. It's quite good. Magic works by drawing on the power of nature. The more in tune with nature the caster, is the more powerful their spells will be. This one is pretty good in terms of like, \textbf{it does help in terms of giving me inspiration}.}
%
\myquote{P4}{So the function was helpful for \textbf{figuring out how to map out a plot}. I didn't really start with a plot in mind when I was writing this story.}
\myquote{P14}{\textbf{If I'm having writers block} and I can't figure out what to say next, \textbf{I would definitely use [Inspo] to see if I had any ideas from it.}}
%
% P2 used Inspo to add drama to characters' lives.
% \myquote{P2}{I guess another hard part is I don't like to make them suffer too much. Then it's what they have to because that's what drama is. \textbf{[Inspo] gave me ideas for ways to make them suffer}.}


% \kenneth{I guess all the concerns about agency, ownership, etc, are also part of the echoing prior work?}

\subsubsection{Common Concerns}

\paragraph{LLMs' Bias}
% \cy{Deepmind: 5.3.1 - The system outputs are too literal and predictable.}
% \cy{Deepmind: 5.3.2 - The system outputs can be problematic, stereotypical and biased.}
Participants noticed that \system's LLM-generated inspirations had a few tendencies they found unhelpful. 
For example, P1 felt the AI-based function always provided something really dramatic.
\myquote{P1}{The emotion is \textbf{always very dramatic} in these like AI things.}
P4 mentioned that some ideas were formulaic and stuck to a certain genre.
\myquote{P4}{What I saw from the other ones was a little bit more \textbf{formulaic} or like they all \textbf{tended to drift toward the same outcome} or kind of like... they hugged the genre closer.}
\myquote{P5}{I know when I'm asking something, it's pretty much like, how can we keep this story going? Not necessarily to resolve it. But \textbf{it's almost like they're trying to find a way to resolve the story}.}
%
These biases are not significantly harmful and mostly affect the quality of the generated inspirations. 
However, participants also noted potentially problematic biases. 
For example, P1 was writing a queer story, but the ideas suggested by the AI-based functions were always about heterosexual relationships. There were also gender bias in the suggestions.
\myquote{P1}{I could imagine some people if they're writing like \textbf{queer story}. I think \textbf{all the suggestion that gave me was heterosexual relationship}.}
\myquote{P1}{[AI Plot Generation] ... gave me something like `she blushed when she realized people were looking at her naked body.' It's a bit like what I just described previously, like women are dispensable.}
%
Such bias could convey problematic values to users and require more attention.
Participants in Dramatron (\cite{mirowski2022co}, Section 5.3) also found that LLMs sometimes generated predictable outputs and occasionally gave responses with problematic stereotypes.



\paragraph{Authorship and Plagiarism Issues}
% \cy{Deepmind: 7.4 - Using a Tool or Participating in a Co-Creative System. Many participants felt they did not own the final output.}
% \cy{Deepmind: 7.3 Ethical Questions and Risks Posed by AI Writing Tools (copyright issues)}
% \cy{Google: 7.6 Concerns about the Origin of Wordcraft's Suggestions}
Writers are concerned about authorship when using \system, especially the Auto-Completion function.
\myquote{P1}{\textbf{I'd prefer to complete my own paragraph}.}
\myquote{P11}{[Auto-Completion] makes you feel \textbf{you have not quite done the writing}.}
%
P2 and P4 had concerns about claiming authorship after using \system.
\myquote{P2}{I think that though the autocomplete function was the most useful, \textbf{I might have some qualms about claiming authorship}... What kind of copyright protections would be in place? I.e., is something that an AI wrote property of the person who wrote the code for the AI, or would the human’s input be more important in determining the ownership of that? \textbf{Assuming that the human author would retain rights, then I would use it in the future to assist with generating ideas}.}
\myquote{P4}{I think that the one thing that I would be worried about that I think a lot of writers would like really, \textbf{really worry about who owns [the writing]}.}
Similarly, in Dramatron's post-interview surveys, most of the participants felt difficulty in claiming authorship after co-wrote with LLMs (\cite{mirowski2022co}, Section 7.4).
%
On the other hand, P11 was also concerned whether the LLMs might provide texts from existing resources: plagiarism. P11 believed that one of their generated suggestions was from a book.
\myquote{Idea}{... June and Calvin’s Interracial Relationship was viewed as a taboo within the African American community. This view was evident in \underline{\smash{Episode 8}}, when Calvin’s uncle visits ...}
P11 may have perceived plagiarism due to the words ``Episode 8'' in the suggestion, as we did not find this identical text online. 
However, as many prior works have shown that LLMs have ability to remember training data, relieving user's concerns about plagiarism is an important issue (\cite{10.1145/3532106.3533533}, Section 6.2.4 and \cite{carlini2021extracting}).
%\cy{citation}
Both WordCraft (\cite{ippolito2022creative}, Section 7.6) and Dramatron (\cite{mirowski2022co}, Section 7.3) discussed the users' concerns about the origin of the generated texts and the risks of using copyrighted contents unintentionally.



\subsubsection{Using LLMs to Learn and Negotiate with Conventions}
\overview{summary of finding about discourse community}
-Gauge actual human, LLM, or readers' thoughts, expectations, and understandings about the various story directions.
-Then they can decide what to do next. (Confirmation or lead to other directions)
-LLM is an aggregated reader that knows patterns and is a valid reader that picks up patterns.

The participants used Inspo to confirm potential readers\avon{reader or writer?}’ thoughts of their writing plans – participants already had concrete writing plans in mind, but they were not sure what the audience thought about their ideas. Via Inspo, the writers tried to probe readers’ expectations of the following part, people’s thoughts about various story directions, and if readers could understand the current snippet.
\begin{quote}
    \textit{``With a human, I think it was fun to play around with the directions and be
like, so what do you think? Like, I want this to be X, Y, Z, where should I go now?''} -- P4
\end{quote}
\begin{quote}
    \textit{``.. I was able to get a response back from an actual person. Like an actual
reader, essentially to see if what I was saying made sense to them or what they
were thinking was happening.''} -- P14
\end{quote}

After having an idea about how readers thoughts, the writers would then consider whether
they wanted to adopt the readers opinions or not. When the feedback is not appealing enough, the
writers might not buy in the ideas.
\begin{quote}
    \textit{`` asked, should she confess the lie to her brother? Or should she insist that
there is a boyfriend? Sometimes this could be either confirmation of what I was
going to do or kind of lead me in another direction.''} -- P5
\end{quote}

Some of the participants (P4, P14) preferred feedback from real humans as it resembled the ex-
perience of asking real readers; while others (P5, P15) chose AI’s feedback. One reason that our
participants chose AI’s feedback was that the LLMs have learned the “patterns” from the corpus. If
a writer’s writing patterns could be recognized by the AI, our writers thought that meant the idea
made sense.
\begin{quote}
    \textit{``I would almost treat the AI also as a reader of, where do they think this is
going, in a similar way [I treated] the human. And seeing if there are patterns
in my writing that an algorithm can pick up. Because obviously I am writing based
on everything I’ve read. There are patterns this computer has been trained on things,
and so is my writing in a way that other people are going to be able to pick up on
those patterns too?''} -- P15
\end{quote}


    
\end{comment}




==> tables/inspiration-stastistic.tex <==
%TC:ignore
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
%\addtolength{\tabcolsep}{-0.7mm}
\small
\centering
\begin{tabular}{@{}l@{}c@{}ccccc|cccc@{}}
\toprule
 &  &  & \multicolumn{4}{c}{\textbf{\#Task}} & \multicolumn{4}{c}{\textbf{\#Suggestion}} \\ \cmidrule(lr){4-7}\cmidrule(lr){8-11}
 & \multicolumn{1}{@{}l@{}}{\textbf{Days}} & \multicolumn{1}{l}{\textbf{\#Word}} & \multicolumn{1}{c}{\textbf{C}} & \multicolumn{1}{c}{\textbf{S}} & \multicolumn{1}{c}{\textbf{GP}} & \multicolumn{1}{c}{\textbf{GC}} & \multicolumn{1}{c}{\textbf{C}} & \multicolumn{1}{c}{\textbf{S}} & \multicolumn{1}{c}{\textbf{GP}} & \multicolumn{1}{c@{}}{\textbf{GC}} \\ \midrule
\textbf{\textbf{\participant{1}}} & 3 & 1,376 & \underline{1} & \textbf{3} & \textbf{3} & \textbf{3} & 1 & \underline{3} & \textbf{6} & \underline{3} \\
\textbf{\textbf{\participant{2}}} & 3 & 1,352 & 3 & \underline{4} & 2 & \textbf{5} & 5 & \underline{6} & 2 & \textbf{8} \\
\textbf{\textbf{\participant{4}}} & 7 & 2,376 & \underline{6} & \underline{6} & \underline{6} & \textbf{12} & \underline{6} & \underline{6} & \underline{6} & \textbf{12} \\
\textbf{\textbf{\participant{5}}} & 7 & 10,289 & \underline{6} & \textbf{11} & \underline{6} & \underline{6} & \textbf{12} & \underline{11} & 7 & 7 \\
\textbf{\textbf{\participant{10}}} & 7 & 1,773 & 1 & \underline{2} & 1 & \textbf{5} & \underline{2} & \underline{2} & \underline{2} & \textbf{9} \\
\textbf{\textbf{\participant{11}}} & 7 & 2,317 & 2 & 4 & \textbf{7} & \underline{5} & 2 & 6 & \textbf{9} & \underline{8} \\
\textbf{\textbf{\participant{14}}} & 7 & 2,715 & 5 & \underline{6} & 5 & \textbf{15} & \underline{11} & 10 & 8 & \textbf{16} \\
\textbf{\textbf{\participant{15}}} & 7 & 2,759 & 6 & \underline{9} & 7 & \textbf{10} & \underline{16} & \textbf{19} & 14 & \textbf{19} \\
\textbf{\textbf{\participant{2}}$_{na}$} & 30 & - & 7 & \textbf{23} & 2 & \underline{13} & \underline{22} & \textbf{23} & 2 & 13 \\ \midrule
\textbf{Total} & - & - & 37 & \underline{68} & 39 & \textbf{74} & 77 & \underline{86} & 56 & \textbf{95} \\ \bottomrule
\end{tabular}
%\vspace{-2mm}
%\addtolength{\tabcolsep}{+0.7mm}
\caption{The number of tasks and suggestions retrieved by all the participants (RQ1). C, S, GP, GC stand for \crowd, \plot, \gptplot, \gptc, respectively. \participant{2}$_{na}$ represent \participant{2}'s NaNoWriMo study. Participants used \gptc most frequently. The highest and second highest usage are \textbf{bold} and \underline{underlined}.}
\label{tab:inspiration-stastistic}
\end{table}




% \begin{table*}[]
% \centering
% \small
% \addtolength{\tabcolsep}{-0.3mm}
% \begin{tabular}{llrrrrrrrrrr}
% \toprule
%  &  & \textbf{\participant{1}} & \textbf{\participant{2}} & \textbf{\participant{4}} & \textbf{\participant{5}} & \textbf{\participant{10}} & \textbf{\participant{11}} & \textbf{\participant{14}} & \textbf{\participant{15}} & \textbf{\participant{2}}$_{na}$ & \textbf{Total} \\ \midrule
%  \multicolumn{2}{l}{\textbf{Days of Study}} & 3 & 3 & 7 & 7 & 7 & 7 & 7 & 7 & 30 & - \\
%  \multicolumn{2}{l}{\textbf{Word Counts}} & 1,376 & 1,352 & 2,376 & 10,289 & 1,773 & 2,317 & 2,715 & 2,759 & - & - \\ \midrule
% \multirow{4}{*}{\textbf{\# task}}
%  & \textbf{\crowd}   & \underline{1} & 3 & \underline{6} & \underline{6} & 1 & 2 & 5 & 6    & 7     & 37 \\
%  & \textbf{\plot}    & \textbf{3} & \underline{4} & \underline{6} & \textbf{11} & \underline{2} & 4 & \underline{6} & \underline{9}   & \textbf{23}   & \underline{68} \\
%  & \textbf{\gptplot} & \textbf{3} & 2 & \underline{6} & \underline{6} & 1 & \textbf{7} & 5 & 7    & 2     & 39 \\
%  & \textbf{\gptc}    & \textbf{3} & \textbf{5} & \textbf{12} & \underline{6} & \textbf{5} & \underline{5} & \textbf{15} & \textbf{10} & \underline{13} & \textbf{74} \\ \midrule
% \multirow{4}{*}{\textbf{\# Inspiration}}
%  & \textbf{\crowd} & 1 & 5 & \underline{6} & \textbf{12} & \underline{2}  & 2 & \underline{11} & \underline{16} & \underline{22} & 77 \\
%  & \textbf{\plot} & \underline{3} & \underline{6} & \underline{6} & \underline{11} & \underline{2}   & 6 & 10 & \textbf{19} & \textbf{23} & \underline{86} \\
%  & \textbf{\gptplot} & \textbf{6} & 2 & \underline{6} & 7 & \underline{2}  & \textbf{9} & 8 & 14 & 2 & 56 \\
%  & \textbf{\gptc} & \underline{3} & \textbf{8} & \textbf{12} & 7 & \textbf{9}    & \underline{8} & \textbf{16} & \textbf{19} & 13 & \textbf{95} \\ \bottomrule
% \end{tabular}
% \addtolength{\tabcolsep}{0.3mm}
% \caption{The number of tasks and inspirations retrieved by all the participants. \participant{2}$_{na}$ represent \participant{2}'s NaNoWriMo study. Participants used \gptc most frequently. The highest and second highest usage are \textbf{bold} and \underline{underlined}.}
% \label{tab:inspiration-stastistic}
% \end{table*}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{clrrrrrrr}
% \toprule
% \multicolumn{2}{c}{\textbf{Task Type}} & \textbf{P1} & \textbf{P2} & \textbf{P3} & \textbf{P4} & \textbf{P5} & \textbf{P6} & \textbf{Total} \\ \midrule
% \multirow{2}{*}{\textbf{Information}} & \textbf{Length of Study (Days)} & 3 & 3 & 7 & 7 & 7 & 7 & - \\
%  & \textbf{Final Word Counts} & 1,376 & 1,351 & 2,373 & 10,287 & 2,713 & 2,758 & - \\ \midrule
% \multirow{4}{*}{\textbf{\# task}} & \textbf{Crowd Plot Generation} & 1 & 3 & 6 & 6 & 5 & 6 & 27 \\
%  & \textbf{AI Plot Generation} & 3 & 4 & 6 & 11 & 6 & 9 & 39 \\
%  & \textbf{AI Plot Generation + Guidance} & 3 & 2 & 6 & 6 & 5 & 7 & 29 \\
%  & \textbf{Auto-Completion} & 3 & 5 & 12 & 6 & 15 & 10 & \textbf{51} \\ \midrule
% \multirow{4}{*}{\textbf{\# inspirations}} & \textbf{Crowd Plot Generation} & 1 & 5 & 6 & 12 & 11 & 16 & 51 \\
%  & \textbf{AI Plot Generation} & 3 & 6 & 6 & 11 & 10 & 19 & 55 \\
%  & \textbf{AI Plot Generation + Guidance} & 6 & 2 & 6 & 7 & 8 & 14 & 43 \\
%  & \textbf{Auto-Completion} & 3 & 8 & 12 & 7 & 16 & 19 & \textbf{65} \\
%  \bottomrule
% \end{tabular}
% \caption{The number of tasks and inspirations retrieved by all the participants. Participants used Auto-Completion most frequently.\kenneth{This needs to be update}}
% \label{tab:inspiration-stastistic}
% \end{table}

%TC:endignore

==> tables/inspiration-tasks.tex <==
%TC:ignore
\begin{table*}[t]
    \centering 
    \small
    \begin{tabular}{lcccc}
        \toprule
        \multicolumn{1}{c}{\textbf{Task Name}} & \textbf{Computation} & \textbf{Instruction} & \textbf{Inspiration Type} & \textbf{Cost} \\ \midrule 
        \textbf{Crowd Plot Generation} & Human & Allowed & Story Plot & High \\
        \textbf{AI Plot Generation} & Machine & Not Allowed & Story Plot & Lowest \\
        \textbf{AI Plot Generation with Guidance} & Machine & Allowed & Story Plot & Low \\
        \textbf{Auto-completion} & Machine & Not Allowed & Content & Low \\
        \bottomrule
    \end{tabular}
    \caption{\system provides four inspiration tasks. Each of them behaves differently.}
    \label{tab:inspiration-task}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}

\item Crowd Plot Generation;
\item AI Plot Generation;
\item AI Plot Generation with Guidance;
\item Auto-completion;
    
    
\end{comment}

%TC:endignore

==> tables/latency-table.tex <==
%TC:ignore


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\small
\centering
\addtolength{\tabcolsep}{-0.5mm}
\begin{tabular}{@{}cccccc@{}}
\toprule
\multicolumn{2}{c}{\textbf{Task Type}} & \textbf{C} & \textbf{S} & \textbf{GP} & \textbf{GC} \\ \midrule
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}System\\ Latency\end{tabular}}} & \textbf{\#Samples} & 30 & 45 & 37 & 61 \\
 & \textbf{25\%} & 1,753 & 7 & 7 & 9 \\
 & \textbf{50\%} & 3,449 & 8 & 8 & 9 \\
 & \textbf{75\%} & 8,160 & 10 & 9 & 10 \\ \midrule
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Reading\\ Latency\end{tabular}}} & \textbf{\#Samples} & 19 & 36 & 32 & 51 \\
 & \textbf{25\%} & 21,881 & 15 & 8 & 4 \\
 & \textbf{50\%} & 34,429 & 115 & 20 & 13 \\
 & \textbf{75\%} & 73,652 & 538 & 74 & 84 \\ \midrule
\multicolumn{2}{c}{\textbf{Not Reading}} & 36.67\% & 20.00\% & 13.51\% & 16.39\% \\ \bottomrule
\end{tabular}
%\vspace{-2mm}
\addtolength{\tabcolsep}{0.5mm}
\caption{
    System and reading latency (in seconds) for four different tasks (RQ1).
    C: \crowd, S: \plot, GP: \gptplot, and GC: \gptc.
    Note that \participant{2}$_{na}$ is excluded. For \crowd, half took up to 60 minutes for an initial response, and users typically read the response hours later. A higher rate of not reading is also observed.
}
\label{tab:latency-distribution}
%\vspace{-3mm}
\end{table}

% \begin{table*}[t]
% \centering \small
% \begin{tabular}{@{}lccccccccc@{}}
%     \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Task Type}}} & \multicolumn{4}{c}{\textbf{System Latency}} & \multicolumn{4}{c}{\textbf{Reading Latency}} & \multirow{2}{*}{\textbf{Not Reading}} \\ \cmidrule(lr){2-9}
%     \multicolumn{1}{c}{} & \textbf{\# Samples} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} & \textbf{\# Samples} & \textbf{25\%} & \textbf{50\%} & \textbf{75\%} & \\ \midrule
%     \textbf{\crowd} & 30 & 1,753 & 3,449 & 8,160 & 19 & 21,881 & 34,429 & 73,652 & 36.67\% \\
%     \textbf{\plot} & 45 & 7 & 8 & 10 & 36 & 15 & 115 & 538 & 20.00\% \\
%     \textbf{\gptplot} & 37 & 7 & 8 & 9 & 32 & 8 & 20 & 74 & 13.51\% \\
%     \textbf{\gptc} & 61 & 9 & 9 & 10 & 51 & 4 & 13 & 84 & 16.39\% \\ \bottomrule
% \end{tabular}
% \caption{
%     System and reading latency (in seconds) for four different tasks. Note that \participant{2}$_{na}$ is excluded. In the case of the \crowd option, half took up to 60 minutes for an initial response, and users typically read the response hours later. Additionally, there is a higher possibility of results not being read.\kenneth{Update the table to say System Latency and Reading Latency. See the paper content.}
% }
% \label{tab:latency-distribution}
% \end{table*}


%TC:endignore



==> tables/participants-table.tex <==
%TC:ignore
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% \newcommand{\sy}{P1\xspace}
% \newcommand{\kat}{P2\xspace}
% \newcommand{\bunny}{P3\xspace}
% \newcommand{\trisha}{P4\xspace}
% \newcommand{\chris}{P5\xspace}
% \newcommand{\mikhai}{P6\xspace}

\begin{table}[t]
\centering \small
    \begin{tabular}{@{}lll@{}}
    \toprule
    \textbf{Participant} & \textbf{Writing Exp.} & \textbf{Publishing Experience} \\ \midrule
    \participant{1} & $\leq$ 1 Year & Online forums, blogs, websites \\
    \participant{2} & 5-10 Years & Online forums, blogs, websites \\ \midrule
    \participant{4} & 5-10 Years & Published books \\
    \participant{5} & $\geq$ 10 Years & Published books \\
    \participant{10} & 5-10 Years & Online forums, blogs, websites \\
    \participant{11} & 3-5 Years & Online forums, blogs, websites \\
    \participant{14} & $\geq$ 10 Years & Online forums, blogs, websites \\
    \participant{15} & $\geq$ 10 Years & Online forums, blogs, websites \\
    \bottomrule
    \end{tabular}
    %\vspace{-2mm}
\caption{Participants were selected based on writing experience and publishing experience. \participant{1} and \participant{2} joined the pilot study; the rest of the participants joined the formal user study. \participant{2} further participated in the NaNoWriMo study.\kenneth{Maybe merge Table 1 and 2?}
}
\label{tab:participant-information}
\vspace{-2mm}
\end{table}


% \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{llll}
% \toprule
% \multicolumn{1}{c}{\textbf{Participant}} & \textbf{Writing Experience} & \textbf{Publishing Experience} & \textbf{Writing Style} \\ \midrule
% \participant{1} & Less than 1 Year & Published in online forums, blogs, or websites & Outliner \\
% \participant{2} & 5 Years - 10 Years & Published in online forums, blogs, or websites & Mix of both \\ \midrule
% % P3 & 3 Years - 5 Years & Published books & Discovery Writer \\
% \participant{4} & 5 Years - 10 Years & Published books & Discovery Writer \\
% \participant{5} & More than 10 Years & Published books & Discovery Writer \\
% % P6 & 5 Years - 10 Years & Self-published books & Discovery Writer \\
% % P7 & 5 Years - 10 Years & Self-published books & Discovery Writer \\
% % P8 & 5 Years - 10 Years & Self-published books & Discovery Writer \\
% % P9 & More than 10 Years & Self-published books & Discovery Writer \\
% \participant{10} & 5 Years - 10 Years & Published in online forums, blogs, or websites & Outliner \\
% \participant{11} & 3 Years - 5 Years & Published in online forums, blogs, or websites & Outliner \\ % Not sure if we want this one
% % P12 & 1 Year - 3 Years & Published in online forums, blogs, or websites & Outliner \\
% % P13 & 1 Year - 3 Years & Published in online forums, blogs, or websites & Outliner \\
% \participant{14} & More than 10 Years & Published in online forums, blogs, or websites & Mix of both \\
% \participant{15} & More than 10 Years & Published in online forums, blogs, or websites & Mix of both \\ 
%  \bottomrule
% \end{tabular}
% \caption{Participants were selected based on writing experience, publishing experience, and writing strategy (\ie, outliner, discovery writer, and mix of both). \participant{1} and \participant{2} joined the pilot study; the rest of the participants joined the formal user study. \participant{2} further participated in the NaNoWriMo study.\kenneth{HCOMP TODO: Remove the Writing Style column and make it fit in single-columnn}
% % (We originally recruited 15 participants and half of them dropped during the study. We kept the original participant index.)
% }
% \label{tab:participant-information}
% \end{table*}
% %TC:endignore
